All polytopes are coset geometries: characterizing automorphism groups of k-orbit abstract polytopes

Abstract polytopes generalize the classical notion of convex polytopes to more general combinatorial structures. The most studied ones are regular and chiral polytopes, as it is well-known, they can be constructed as coset geometries from their automorphism groups. This is also known to be true for 2- and 3- orbit 3-polytopes. In this paper we show that every abstract $n$-polytope can be constructed as a coset geometry. This construction is done by giving a characterization, in terms of generators, relations and intersection conditions, of the automorphism group of a $k$-orbit polytope with given symmetry type graph. Furthermore, we use these results to show that for all $k\neq 2$, there exist $k$-orbit $n$-polytopes with Boolean automorphism groups, for all $n\geq 3$.

==> AbstractPolytopes.tex <==
\section{Abstract polytopes and maniplexes}\label{sec:Polytopes-and-maniplexes}

In this section we shall give the basic definitions and properties of abstract polytopes and maniplexes, and some relations between them. For more details, we refer the reader to \cite{PolyMani}, \cite{ARP} and \cite{Maniplexes}. 

A partially ordered set is said to be {\em flagged} if it has
a (unique) least and a (unique) greatest
element and each maximal chain, called {\em a flag}, has the same
finite cardinality. 
As all flags have the same cardinality, say $n+2$, flagged posets naturally admit an order-preserving
function, the {\em rank function},  from the poset to the set $\{-1,0,1,\ldots,n\}$. 
The rank function allows us to talk about flag-adjacencies: given two flags $\Phi$ and $\Psi$ of a flagged poset, they are said to be $i$-adjacent if they to differ only in the element of rank $i$.


An {\em (abstract) $n$-polytope} (also called an {\em (abstract)
  polytope of rank 
  $n$}) is a flagged poset $\p$ in which the following 
conditions hold:
\begin{itemize}
\item {\em Diamond condition:} for each flag $\Phi$ of $\p$ and each $i \in \{0,1,\dots, n-1\}$, there exists a unique $i$-adjacent flag to $\Phi$. %if $F<G$ and $\rk(G)-\rk(F)=2$ then  there exist exactly two different elements $H_1,H_2\in  \p$ such that   $F<H_i<G$.
  \item {\em Strong flag connectedness:} for any two flags $\Phi$ and
    $\Psi$ of $\p$, %intersect on the elements of ranks on a set $K\subset
            %\{-1,\ldots,n\}$, then 
    there exists a sequence of adjacent flags connecting $\Phi$ to $\Psi$,
    such that all the flags in the sequence contain $\Phi \cap \Psi$ as a subset. 
\end{itemize}



%Note that the diamond condition is equivalent to say that if $F$ and $G$ are two elements of $\p$ such that $F<G$ and $\rk(G)-\rk(F)=2$, then there exist exactly two different elements $H_1,H_2\in  \p$ such that $F<H_i<G$.


The elements of a polytope are called {\em faces}, and faces of rank $i$ are called {\em $i$-faces}. 
Given a flag $\Phi$, we often denote its $i$-face as
$\Phi_i$, and by $\Phi^i$ its (unique!)
$i$-adjacent flag. 
Recursively, if $w$ is a word on
$\{0,\ldots,n-1\}$ we denote by $\Phi^{wi}$ the flag $(\Phi^{w})^i$.
It is straightforward to see that $(\Phi^i)^i=\Phi$, and that $(\Phi^i)_j=\Phi_j$ if and only if $i\neq j$.

Given a flagged poset $\p$ one can define its {\em flag graph}
as the graph $\G(\p)$ whose vertices are the flags of $\p$ and two
flags $\Phi$ and $\Psi$ are connected by an edge of color
$i\in\{0,1,\ldots,n-1\}$ if and only if they are $i$-adjacent. 
The flag graph of an $n$-polytope is an {\em $n$-maniplex}, that is,
an $n$-regular connected simple graph with a proper edge coloring with colors
$\{0,\ldots,n-1\}$ such that if $i$ and $j$ are two colors satisfying that
$|i-j|>1$, then the graph induced by edges
of colors $i$ and $j$ is a disjoint union of 4-cycles.
However, not every maniplex is the flag graph of a polytope.

While abstract polytopes generalize classical polytopes to combinatorial structures,
maniplexes (introduced by Steve Wilson in 2012 \cite{Maniplexes}) generalize flag graphs of a polytope as well as of the flag graphs of maps on surfaces (that is, 2-cellular
embeddings of connected graphs on surfaces). 
In order to unify our notation of abstract polytopes and maniplexes, when dealing with maniplexes we shall call its vertices {\em flags}, and say that two of flags are $i$-adjacent if they are the vertices of an edge of color $i$.



It follows from the definition of a maniplex that each flag is incident to exactly
one edge of each color. 
Then, for each $i\in\{0,1,\ldots,n-1\}$ one
can define $r_i$ as the permutation of the set of flags that maps
each flag to its $i$-adjacent one.
In other words $\Phi r_i=\Psi$ if and only if $\Phi$ and $\Psi$
are $i$-adjacent.

The permutations $r_i$, with $i\in \{0,1,\ldots,n-1\}$, are all
involutions with no fixed points and, by connectivity, they generate a group of permutations on the flags which acts
transitively on them. 
Furthermore, if $|i-j|>1$ then $r_ir_j$ is also an involution with no
fixed points; thus, $r_i$ and $r_j$
commute.



%One may use the action of this permutation group generated by 
%involutions as an alternative definition of a maniplex. That is, %a
%maniplex may equivalently be defined as a set $\F$ whose elements are called
%{\em flags}, and an indexed set of permutations $\{r_i\}_{i=0}^{n-1}$
%of $\F$ satisfying:
%\begin{itemize}
%\item for every $i$ the involution $r_i$ has no fixed points,
%\item if $\Phi r_i=\Phi r_j$ for some flag $\Phi$, then $i=j$,
%\item the group $\gen{r_i:i=0,\ldots,n-1}$ acts transitively on $\F$,
%\item if $|i-j|>1$ then $r_ir_j$ is an involution.
%\end{itemize}
%Note that these conditions imply that the involutions $r_ir_j$ have no fixed points.


Since $\Phi r_i$ is the flag $i$-adjacent to $\Phi$, it is convenient to
denote it by $\Phi^i$ and to follow the same recursive notation as before: $\Phi^{wi}=(\Phi^w)^i$ where $w$ is a word on
$\{0,1,\ldots,n-1\}$.
%Thus, if $\omega \in \langle r_0, r_1, dots, r_{n-1} \ranlge$, 

The group $\gen{r_0, r_1\ldots,r_{n-1}}$ is called the {\em monodromy} or
{\em connection} group of the maniplex $\M$, it shall be denoted by
$Mon(\M)$ and we shall call each of its elements a {\em
  monodromy}. 
  If $w$ is a word on the
alphabet $\{0,1,\ldots,n-1\}$ we identify $w$ with the monodromy
$x\mapsto x^w$, that is, the word $a_1a_2\ldots a_k$ is identified
with the monodromy $r_{a_1}r_{a_2}\ldots r_{a_k}$.

A {\em maniplex homomorphism} is a graph homomorphism that preserves the color of the edges. 
Using the connectedness of maniplexes one can see that every maniplex homomorphism is determined by the image of one flag and that they are all surjective.
The notions of {\em isomorphism} and {\em automorphism} follow naturally.

 As with polytopes, we denote the automorphism group of a maniplex $\M$ by $\Gamma(\M)$. 
 By definition, if $\gamma \in \Gamma(\M)$, then $(\Phi r_i)\gamma = (\Phi^i)\gamma = (\Phi\gamma)^i = (\Phi\gamma)r_i$, for all $i\in \{0,1, \dots, n-1\}$, implying that $\omega\gamma = \gamma \omega$ for all $\omega \in Mon(\M)$.

Note further that, since the action of $Mon(\M)$ is transitive, the action of $\Gamma(\M)$ is free (or semi-regular). 
Of course, this is true for both  polytopes and maniplexes.

%Thus, given maniplexes $\M$ and $\M'$, then
% $\gamma:\M \to \M'$ is a maniplex
%homomorphism if and only if  $(\Phi^i)\gamma = (\Phi\gamma)^i$ for all flags $\Phi$ and $i\in \{0,1,\ldots,n-1\}$.
%Therefore if $\M=\M'$, then $(\Phi r_i)\gamma = (\Phi^i)\gamma = (\Phi\gamma)^i = (\Phi\gamma)r_i$, implying that $\omega\gamma = \gamma \omega$ for all
%$\omega \in Mon(\M)$.


% We will see later that the automorphism
%group of $\p$ as a polytope coincides with that of $\G(\p)$ as a
%maniplex, that is $\Gamma(\p) = \Gamma(\G(\p))$.

%If $\Phi$ is a flag of a maniplex $\M$ and $\Psi$ is any other flag, there
%exists a monodromy $w$ such that $\Psi=\Phi^w$. Then, if $\gamma:\M\to
%\M'$ is a maniplex homomorphism, we have that $\Psi\gamma =
%(\Phi^w)\gamma = (\Phi\gamma)^w$. This means that $\gamma$ is
%completely determined by its action on only one flag ($\Phi$, for
%example). In particular, the automorphism group of a maniplex acts {\em
%  freely} on its flags. Of course, this is also true for polytopes.

%\elias{creo que no vamos a usar dualidad.} A maniplex $\M$ also has a {\em dual} maniplex $\M^*$ which is obtained
%simply by replacing each color $i$ by $n-1-i$. If $\M$ is the flag
%graph of a polytope $\p$ is easy to see that $\M^*$ is the flag graph
%of $\p^*$.

%Just as with polytopes, the dual of a maniplex has the same
%automorphism group as the original maniplex. A maniplex isomorphic to
%its dual is called {\em self-dual}.

Let $\M$ be an $n$-maniplex. If $I\subset \{0,1,\ldots,n-1\}$, we
define $\M_I$ as the subgraph of $\M$ induced by the edges of colors
in $I$. If $i\in\{0,1,\ldots,n-1\}$, we use the symbol $\ol{i}$ to
denote the set $\{0,1,\ldots,n-1\}\setminus\{i\}$, and more generally,
if $K\subset \{0,1,\ldots,n-1\}$, we denote its complement by
$\ol{K}$. In particular $\M_{\ol{i}}$ is the subgraph of $\M$ obtained
by removing the edges of color $i$. We will use this notation also for
any graph with a coloring of its edges even if it is not a maniplex.

In \cite{PolyMani} Garza-Vargas and Hubard describe how to recover a polytope $\p$ from its flag graph: 
%
%Given the flag graph of a polytope $\p$, one may use the strong flag connectedness to recover $\p$ from it. To do this, note that if two flags $\Phi$ and $\Psi$ share the same $i$-face there should be a path in the flag graph from $\Phi$ to $\Psi$ that does not use darts of color $i$.
%Conversely, if there is such a path between $\Phi$ and $\Psi$, since after traveling one dart one arrives to a flag with the same faces except for the one with rank equal to the color of the dart, then $\Phi$ and $\Psi$ (and every flag along the way) must have the same $i$-face. 
%This means that the set of flags with the same $i$-face $F$ as $\Phi$ are the flags in the same connected component of the subgraph obtained by erasing the edges of color $i$, that is $\M_{\ol{i}}(\Phi)$. 
%One may identify this connected component with the $i$-face $F$.
%
%Moreover, if an $i$-face $F$ and a $j$-face $G$ are incident, there
%should be a flag $\Phi$ containing both of them. So the subgraphs
%corresponding to $F$ and $G$ should have $\Phi$ in their
%intersection. Conversely, if the subgraphs corresponding to $F$ and
%$G$ have non-empty intersection, the flags in the intersection have
%both $F$ and $G$ as elements, implying that $F$ and $G$ are incident.
%One may use this to get a ranked poset $\p(\M)$ from any maniplex $\M$. 
the elements of rank $i$ of $\p$ are the connected
components of $\M_{\ol{i}}$; the order is given as follows: given connected components  $F$ and $G$ of $\M_{\ol{i}}$ and $\M_{\ol{j}}$, respectively, we set $F<G$ if and only if $i<j$ and $F\cap G \neq \emptyset$.

Moreover, starting with $\M$ one can construct the set
of $i$-faces as the connected components of $\M_{\ol{i}}$ 
and define the relation $F<G$ for $F\in \M_{\ol{i}}$ and 
$G\in \M_{\ol{j}}$ if and only if $i<j$ and 
$F\cap G \neq \emptyset$.
The set of all $i$-faces, with $i\in\{0,\dots, n-1\}$ together with $''<''$ is denoted by $\p(\M)$.
%then defined by the rule
%$F<G$ if and only if $F\cap G \neq \emptyset$ and $\rk(F)<\rk(G)$,
%where $\rk$ is the {\em rank} function of $\p$.
In \cite{PolyMani} it is proved that if $\M$ is any maniplex, then
$\p(\M)$ is a flagged poset.

It is not difficult to see (\cite{PolyMani}) that $\p$ and $\p'$ are isomorphic polytopes if and only if their flag graphs $\G(\p)$ and $\G(\p')$ are isomorphic. This fact implies the following theorem, which can be interpreted as saying that all the information of the
polytope $\p$ is encoded in its flag graph.
%Let $\p$ and $\p'$ be two isomorphic polytopes, let $\Phi$ be a flag
%of $\p$ and let $\gamma:\p \to \p'$ be an
%isomorphism. Then for every $i\in \{0,1,\ldots,n-1\}$, $\Phi\gamma$
%and $(\Phi^i)\gamma$
%should be $i$-adjacent flags of $\p'$, since they must have the same $j$-faces
%for $j \neq i$ (since there pre-images do), and they must have a
%different $i$-face (for the same reason). This means that $\gamma$
%induces a maniplex homomorphism between the flag graphs of $\p$ and $\p'$.
%On the other hand, a maniplex homomorphism between $\G(\p)$ and
%$\G(\p')$ would induce a homomorphism of polytopes between the faces
%of $\p$ and $\p'$ which is defined by looking at the $i$-faces of $\p$
%and $\p'$ as connected components of $\G(\p)_{\ol{i}}$ and
%$\G(\p')_{\ol{i}}$ respectively.

%We have sketched a proof of the following theorem (which appears in
%\cite{PolyMani}).

\begin{teo}\cite{PolyMani}\label{t:GrafBand}
  Let $\p$ be a polytope and let $\M=\G(\p)$ be its flag graph. Then
  $\p$ is isomorphic (as a poset) to $\p(\M)$ and $\Gamma(\p) \cong
  \Gamma(\M)$.
\end{teo}

%\elias{sí queremos este ejemplo en este artículo?}As an example one may look at Figure~\ref{f:GrafPrisma} and note
%that in fact when we erase the edges of color 0 (blue) we get one connected
%component around each vertex of the triangular prism; when we erase the
%edges of color 1 (red) we get a connected component around each edge of
%the triangular prism and that component will always be
%a 4-cycle of colors 0 and 2; and finally when we erase the edges of
%color 2 (green) we get a connected component inside each 2-face of the
%triangular prism.

%Theorem~\ref{t:GrafBand} means that all the information of the
%polytope $\p$ is encoded in its flag graph. %ISA SUGIERE IMPLIES EN
                                %VEZ DE MEANS

%\elias{igual, tal vez demasiado detalle para este artículo?}Before moving on, we want to show how in addition to the faces we can
%actually get every kind of chain of a polytope $\p$ from looking at
%subgraphs of the flag graph $\p$. Let $K$ be a subset of
%$\{0,1,\ldots,n-1\}$. A chain $c$ in $\p$ is of {\em type $K$} if it
%has exactly one element of each rank in $K$.

%Just as we noted that an $i$-face can be identified with a connected
%component of $\M_{\ol{i}}$, a chain
%of type $K$ may be identified with a connected component of
%$\M_{\ol{K}}$: Let $c$ be a chain of type $K$, and let $\Phi$ be a
%flag containing $c$. Due to the strong connectivity of $\p$, one can
%get from $\Phi$ to another flag $\Psi$ by a path that does not uses
%darts with colors in $K$ if and only if $\Psi$ also contains $c$.

%% In general, the converse of Theorem~\ref{t:GrafBand} is not true: a
%% maniplex $\M$ may not be isomorphic to the flag graph of its induced
%% poset $\p(\M)$. Moreover, this flag graph may not even be a
%% maniplex.

Theorem 5.3 of \cite{PolyMani} gives a characterization of {\em polytopal} maniplexes, that is, those maniplexes
that are isomorphic to the flag graph of some polytope.
Such characterization is given in terms of some path intersection properties of the maniplexes.

%In \cite{PolyMani} Garza-Vargas and Hubard prove some characterizations of {\em polytopal} maniplexes, i.e. those maniplexes that are isomorphic to the flag graph of some polytope. 
%These results will be summarized in Theorem~\ref{t:PolyMani}, which in a particular case states that the converse of Theorem~\ref{t:GrafBand} is also true. Before stating Theorem~\ref{t:PolyMani} we need some more definitions.

\begin{Def}\label{d:PIP}
  Let $\M$ be an $n$-maniplex. We say that $\M$ satisfies the {\em
    strong path intersection property} (or SPIP) if for every two
  subsets $I,J \subset \{0,1,\ldots,n-1\}$ and for any two flags $\Phi$ and
  $\Psi$, whenever there is a path $W$ from $\Phi$ to $\Psi$ using only edges of
  colors in $I$ and also a path $W'$ from $\Phi$ to $\Psi$ using only edges
  of colors in $J$, there also exists a path $W''$ from $\Phi$ to
  $\Psi$ that uses only edges of colors in $I \cap J$.

  We say that $\M$ satisfies the {\em weak path intersection property} (or WPIP)
  if for any two flags $\Phi$ and $\Psi$ and for all $k,m \in
  \{0,1,\ldots,n-1\}$, whenever there is a path $W$ from $\Phi$ to $\Psi$
  with only edges of colors in $[0,m]:=\{0,1,\ldots,m\}$ and a path $W'$
  from $\Phi$ to $\Psi$ with only edges of colors in
  $[k,n-1]:=\{k,k+1,\ldots,n-1\}$, then there is also a path $W''$
  from $\Phi$ to $\Psi$ with only edges of colors in $[k,m]:=\{k,k+1,\ldots,m\}$.
\end{Def}

\begin{teo}\label{t:PolyMani}
  \cite[Theorem 5.3]{PolyMani} Let $\M$ be a maniplex. Then the following conditions are all
  equivalent:
  \begin{itemize}
    \item $\M$ is polytopal.
  \item $\M$ satisfies the SPIP.
  \item $\M$ satisfies the WPIP.
  \end{itemize}

  In any of these cases $\p(\M)$ is a polytope whose flag graph is
  isomorphic to $\M$.
\end{teo}
%\elias{va a haber que agregar algo de voltajes antes de pasar a lo siguiente}

==> Basic.tex <==

\input{AbstractPolytopes}

\subsection{Premaniplexes and symmetry type graphs}\label{s:STG}
\input{STG}

\section{Voltage graphs}\label{sec:voltage}
\input{VoltageGraphs}

 
 \input{VoltMan}

==> Basic_Definitions.tex <==
\section{Basic notions}\label{ch:basic}

%In this chapter we introduce the main concepts we will be using
%in this thesis. We will study polytopes in a pure combinatorial
%manner: we will be interested in incidence between faces, edges and
%vertices but not in angles, distances and areas. To take this approach
%we use the concept of {\em abstract polytopes}, introduced by
%Egon Schulte in~\cite{EgonPhd}. The idea is to look at polytopes as
%partially ordered sets satisfying certain conditions that are always
%satisfied by, for example, convex polytopes.

%In Section~\ref{s:Polytopes} we will introduce the concept of abstract
%polytope, as well as some generalizations. We will also introduce the
%main concepts used when studying abstract polytopes, such as {\em
%  faces, flags, rank, isomorphisms and automorphisms} and {\em
%  duality}. In Section~\ref{s:Graphs} we will define the basic
%concepts of Graph Theory we will be using, such as the concept of {\em
%  graph} itself as well as {\em vertices, darts, edges} ({\em links,
%  loops} and {\em semi-edges}), {\em degree} of a vertex, {\em
%  simple graphs, subgraphs, $k$-valent} graphs, {\em paths}, and {\em
%  graph homomorphisms, isomorphisms} and {\em automorphisms}. Even if
%the reader is familiar with Graph Theory, we recommend reading
%Section~\ref{s:Graphs}, since notation and some concepts may be
%different than what the reader may be used to. In
%Section~\ref{s:Maniplexes} we introduce the concept of the {\em flag
%  graph} of a polytope and present the concept of a {\em maniplex} as
%its generalization. We also present some theorems that characterize
%which maniplexes are flag graphs of polytopes. In
%Section~\ref{s:STG} we introduce the concept of the {\em symmetry type
%  graph} of a polytope or a maniplex and introduce {\em
%  multi-maniplexes} as their generalization. Then we present the main
%questions motivating these thesis: Can we characterize when is a
%multi-maniplex the symmetry type graph of a polytope or a maniplex?
%And can we characterize the automorphism groups of a polytope with a
%given symmetry type graph? Finally in Section~\ref{s:Regular} we
%present an answer previously given in~\cite{EgonPhd} to the second
%question for the particular case of {\em regular} polytopes. We will
%use the ideas of this last section throughout this thesis.%

\section{Polytopes as posets}\label{s:Polytopes}

A {\em flagged} partially ordered set (poset) is one in which there is
a least and a greatest
element and each maximal chain, called {\em a flag}, has the same
finite cardinality. Flagged posets admit a unique order-preserving
{\em rank}
function $\rk:\p\to \{-1,0,1,\ldots,n\}$ where $n+2$ is the size of the
flags. The number $n$ is called the {\em rank of $\p$}.

If two flags $\Phi$ and $\Psi$ coincide in all but one of their
elements we say that they are {\em adjacent}. If the element they do
not have in common is of rank $i$ we say that they are {\em
  $i$-adjacent}.

%% Given a
%% flagged poset $\p$ one can define its {\em flag graph}
%% as the graph $\G(\p)$ whose vertices are the flags of $\p$ and two
%% flags $\Phi$ and $\Psi$ are connected by an edge of color
%% $i\in\{0,1,\ldots,n-1\}$ if and only if they differ only
%% on the element of rank $i$. In this case we say that $\Phi$ and
%% $\Psi$ are {\em $i$-adjacent}. VIENE MÁS ADELANTE

Flagged posets are often represented by their {\em Hasse diagram}. The
Hasse diagram of a ranked poset~\footnote{Hasse diagrams can be
  constructed also for non-ranked posets and even to dense posets, but
  we will only use the more simple ones.} $\p$ has its elements
represented by points on different {\em levels}, each level
corresponding to a rank. If two elements, $x,y$ have consecutive ranks
and are incident (i.e. $\rk(y)-\rk(x)=1$ and $x<y$), we draw a line segment
connecting them. In this way, an element $a$ is greater than an element
$b$ if and only if there is a strictly downwards path from $a$ to $b$
in the Hasse diagram.

Chains in a Hasse diagram look like a set of points connected on a
strictly downwards path. A maximal chain consists of all the points in
a maximal strictly downwards path. A ranked poset is a
flagged poset if and only if all its maximal chains go through all the
levels.
%% from the greatest element to the least element , or in other words, if
%% one can reach the highest and the lowest point of the diagram starting
%% at any point without ever changing direction (up or down).


In Figure~\ref{f:EjHasse} we see the Hasse diagram of the poset
$\p:=\{\emptyset,\allowbreak \{1\},\allowbreak \{2\},\allowbreak
\{3\},\allowbreak \{1,2\},\allowbreak \{2,3\},\allowbreak
\{1,2,3\},\allowbreak \{1,2,3,4\}\}$
ordered by contention. This is in fact an example of a flagged
poset. Highlighted in red is the flag
$\Phi=\{\emptyset,\allowbreak \{3\},\allowbreak \{2,3\},\allowbreak
\{1,2,3\},\allowbreak \{1,2,3,4\}\}$.

\begin{figure}
  \begin{center}
    \includegraphics[width=4cm]{Hasse1.pdf}
    \caption{\label{f:EjHasse} Example of the Hasse diagram of a flagged
      poset.}
  \end{center}
\end{figure}

An {\em (abstract) $n$-polytope} (also called an {\em (abstract)
  polytope of rank
  $n$}) is a flagged poset $\p$ of rank $n$ in which the following
conditions hold:
\begin{itemize}
\item {\em Diamond condition:} if $F<G$ and $\rk(G)-\rk(F)=2$ then
  there exist exactly two different elements $H_1,H_2\in
  \p$ such that
  $F<H_i<G$.

\item {\em Strong flag connectedness:} given two flags $\Phi$ and
  $\Psi$, %intersect on the elements of ranks on a set $K\subset
  %\{-1,\ldots,n\}$, then
  there is a sequence of adjacent flags connecting $\Phi$ to $\Psi$,
  such that all the flags in the sequence contain the faces of the
  intersection $\Phi \cap \Psi$.
  %doesn't use edges of colors in $K$.
\end{itemize}

In terms of the Hasse diagram, the diamond condition tells us that if
$\rk(G)-\rk(F)=2$ and $F<G$, the {\em section} $G/F:=\{H: F\leq H \leq
G\}$ looks precisely like a ``diamond'' (see
Figure~\ref{f:Diamante}). In
Figure~\ref{f:EjHasse} we see
that the diamond condition is satisfied for $F=\{2\}$ and
$G=\{1,2,3\}$, since there are exactly two elements between them
($\{1,2\}$ and $\{2,3\}$), but it is not satisfied if we take
$\F=\{3\}$ and $G=\{1,2,3\}$, thus the example given is not an
abstract polytope. The strong connectedness is a bit harder
to see; it says that given two flags, one can get from one to the
other by changing elements not in the intersection one at a time.

\begin{figure}
  \begin{center}
    \D{G}{H_1}{H_2}{F}
    \caption{\label{f:Diamante} A Hasse diagram showing the diamond
      condition.}
  \end{center}
\end{figure}

As their name suggests, the easier examples of abstract polytopes are
the incidence lattices of convex polytopes. In Figure~\ref{f:EjPoli}
we see the Hasse diagram of a tetrahedron. In Figure~\ref{f:Diamantes}
we see some examples of the diamond condition. By symmetry, it should
be clear that these examples are enough to show that the whole poset
satisfies the diamond condition. In Figure~\ref{f:ConexidadFuerte} we
see two highlighted flags (red and blue) with a vertex in common. One
can transform the red flag to the blue flag without ever touching the
vertex in common by changing the edge, then
the face of rank 2, and then the edge again. This is an example of
strong connectedness.

\begin{figure}
  \begin{subfigure}[b]{\columnwidth}
    \begin{center}
      \includegraphics[width=9cm]{Tetraedro.pdf}
      \caption{\label{f:bla} The Hasse diagram of a tetrahedron. This
        is an example of an abstract polytope of rank 3.}
    \end{center}
  \end{subfigure}
  \vspace{0.7cm}
  \begin{subfigure}[b]{\columnwidth}
    \begin{center}
      \includegraphics[width=9cm]{Diamantes.pdf}
      \caption{\label{f:Diamantes} Examples of the diamond condition.}
    \end{center}
  \end{subfigure}
  \vspace{0.7cm}
  \begin{subfigure}[b]{\columnwidth}
    \begin{center}
      \includegraphics[width=9cm]{StrongFC.pdf}
      \caption{\label{f:ConexidadFuerte} Example of strong flag
        connectedness. One can get from the red flag to the blue flag
        by changing the edge, then the 2-face, and then the edge
        again, as indicated by the green arrows.}
    \end{center}
  \end{subfigure}
  \caption{\label{f:EjPoli} The Hasse diagram of a tetrahedron. This
    is an example of an abstract polytope of rank 3.}
\end{figure}

A flagged poset satisfying only the diamond condition is called a {\em
  pre-polytope}.

As an example of a pre-polytope that is not a polytope we consider two
cubes glued by one of their vertices (see Figure~\ref{f:DosCubos}) and
take the face lattice of the result. If we let $\Phi$ be a flag on one
of the cubes containing the glued vertex and let $\Psi$ be one on the
{\em other} cube, there will be no way of getting from $\Phi$ to
$\Psi$ without changing the vertex (in fact we will not be able to get
from $\Phi$ to $\Psi$ by changing one face at a time). Another
example would be one cube in which we glue two opposite vertices. In
that case all flags would be connected, but there would be pairs of
flags sharing a vertex but such that one should change the vertex to
get from one to the other.

\begin{figure}
  \centering
  \includegraphics[width=6cm]{DosCubos.pdf}
  \caption{Two cubes glued by one of their vertices form an example of
    a pre-polytope that is not a polytope}
  \label{f:DosCubos}
\end{figure}

In this thesis, unless stated otherwise, by a polytope we mean an
abstract polytope and we use $n$ to denote its rank. The elements of
rank $i$ in a polytope are called {\em $i$-faces}, and $(n-1)$-faces
are often referred to as {\em facets}.  Given a flag
$\Phi$, we denote its $i$-face as $\Phi_i$, and we denote by
$\Phi^i$ the (unique) $i$-adjacent flag to $\Phi$. Recursively, if $w$
is a word on $\{0,\ldots,n-1\}$ we denote by $\Phi^{wi}$ the flag
$(\Phi^w)^i$.

To picture flags in convex (and some other) polytopes we use what is
called the {\em barycentric subdivision}. To do this for each flag
$\Phi$ we form a simplex whose vertices are the barycenters of each of
its faces. In the barycentric division, $i$-adjacent flags correspond
to simplices that share a facet, specifically the one that contains of
all of their vertices except the barycenter of the $i$-face. In
Figure~\ref{f:TetraedroSubdiv} we can see the
barycentric subdivision of a tetrahedron.

\begin{figure}
  \begin{center}
    \includegraphics[width=5cm]{TetraedroSubdiv.pdf}
    \caption{\label{f:TetraedroSubdiv} Barycentric subdivision of the
      tetrahedron.}
  \end{center}
\end{figure}



An {\em isomorphism} between two polytopes $\p$ and $\p'$ is simply an
isomorphism of posets, that is, a bijection $\gamma:\p \to \p'$
such that $A<B$ if and only if $A\gamma < B\gamma$. In this case we
say that $\p$ and $\p'$ are isomorphic and write $\p \cong \p'$.

As usual, the automorphisms of a polytope $\p$ (the isomorphisms
between $\p$ and itself) form a group. We denote this group by
$\Gamma(\p)$.

Given a poset $\p$ one can get a dual poset $\p^*$ just by reversing
the order $<$, or in terms of the Hasse diagram by ``flipping it
over''. In the case of polytopes, the dual $\p^*$ of a polytope
is still a polytope
and it is still called the {\em dual} polytope. The dual of a polytope
has exactly the same automorphism group as the polytope, that is
$\Gamma(\p) = \Gamma(\p*)$.

If a polytope is isomorphic to its dual it is called {\em self-dual}.

\section{Graphs}\label{s:Graphs}

We will work with lots of graphs in this thesis. In the literature several
definitions graph exist, and although for the most part they are
equivalent, in our case it is important which
one we are working with. We will be working with one of the more complete
ones, which includes graphs with multiple edges, loops and semi-edges
(which as we shall see, should be distinguished from one another).

In this thesis, a {\em graph} is a 4-tuple $X=(V,D,(\cdot)^{-1}, I)$ where:
\begin{itemize}
\item $V$ is a non-empty set whose elements are called {\em vertices}.
\item $D$ is a set whose elements are called {\em darts}.
\item $(\cdot)^{-1}:D\to D$ is an involution called the {\em
  inverse}. %Usually we denote the image of a dart $x$ under $\lambda$
  % by $x^{-1}$ instead of $\lambda(x)$.
\item $I:D\to V$ is a function that maps each dart to a vertex called
  its {\em initial} vertex or {\em start-point}.
\end{itemize}

Given a dart $d$, its {\em end-point} or {\em terminal} vertex is
simply $T(d):=I(d^{-1})$.

The {\em edges} of a graph $X$ are the orbits of $D$ under the action
of the group generated by $(\cdot)^{-1}$ (i.e., pairs $\{d,d^{-1}\}$) and
we denote the set of edges of $X$ by $E(X)$ or just $E$ when the
underlying graph is implicit. The {\em end-points} of an edge are the
end-points (or start-points) of its darts.

An edge with just one dart is called a {\em semi-edge}, and it consists
of a dart $d$ satisfying $d=d^{-1}$. We will often refer to the only
dart of a semi-edge as a semi-edge itself, it should be clear from
context if we are referring to the dart $d$ or the edge $\{d\}$.

If an edge consist of two different darts but they both have the same
starting point, we call it a {\em loop}. A dart in a loop has the same
starting and terminal vertex, but in contrast to a semi-edge it can be
``traveled backwards''.

Edges that are not semi-edges or loops are called {\em links}.

We say that an edge $e$ is {\em incident} to the vertices that are
start-points of at least one of its darts.

As usual, we will think of a graph as a drawing where vertices
are represented by points and edges are represented by line segments
joining their end-points. Loops will be represented by a closed curve
based on the point representing their end-point, while semi-edges will
be represented as line segments that having one end-point on the
vertex they are incident to, leaving the other end-point
``hanging''. For an example, see Figure~\ref{f:EjGrafica}.

\begin{figure}
  \begin{center}
    \includegraphics[width=5cm]{graph.pdf}
    \caption{\label{f:EjGrafica}Example of a graph with all possible
      kinds of edges.}
  \end{center}
\end{figure}

The {\em valency} or {\em degree} of a vertex $v$, denoted by
$deg(v)$ is the cardinality of the set of darts whose starting vertex
is $v$. Note that this means that each loop adds 2 to the degree of
a vertex, while links and semi-edges adds 1. In other words, the
valency of a vertex $v$ is the sum of the number of links and
semi-edges incident to it plus twice the number of loops incident to
it.

A graph is called {\em simple} if it has no loops or semi-edges, and
no two edges are incident to the same vertices (such pairs of edges
are called {\em multiple edges} or {\em parallel edges}).

Given a graph $X$, its {\em subgraphs} are those graphs whose sets of
vertices and darts are subsets of the sets of vertices and darts of
$X$ respectively, and the start-points and inverses of darts are the
same as in $X$. A {\em spanning} subgraph is a subgraph with all the
vertices of $X$.

If $U$ is a subset of the vertex set of a graph $X$ the {\em subgraph
  induced by $U$} is the subgraph whose vertex set is $U$ and its
darts are all the edges of $X$ with both endpoints in $U$. If $A$ is a
set of edges of a graph $X$ the {\em subgraph induced by $A$} is the
subgraph whose vertex set are all the endpoints of edges in $A$ and its
set of darts are the darts of edges in $A$.

A graph in which every vertex has valency $k$ is called a {\em
  $k$-valent}~\footnote{Most texts use the term {\em $k$-regular}
  graph, but we reserve the word {\em regular} for concepts that are
  more related to symmetry and regular actions.}  graph.

A {\em path} in a graph $X$ is a finite sequence of darts
$W=x_1x_2\ldots, x_k$ such that the end-point of each dart is the
start-point of the next one. The number $k$ is called the {\em length}
of $W$ and it is denoted by $\ell(W)$. The {\em start-point} or {\em
  initial vertex of $W$} is the start-point of $x_1$ and the {\em
  end-point} or {\em terminal vertex of $W$} is the end-point of
$x_k$. If a path $W$ starts at a vertex $u$
and ends at a vertex $v$, we say that $W$ goes from $u$ to $v$ and
write $W:u\to v$, and we also say that it {\em connects} $u$ to
$v$. If we talk about the {\em end-points} (in plural) of a path, we
mean both its end-point and its start-point. The {\em inner} vertices
of a path are the start-points of the darts except the first one, that
is, ``all the vertices along the way'' from the start-point to the
end-point.

The empty sequence is not considered a path of length 0, but each
vertex is. When thought of as a path, $W=u$ is a path of length 0 that
goes from $u$ to $u$.

A graph $X$ is {\em connected} if for every two vertices $u$ and $v$
there is a path going from $u$ to $v$. The {\em connected components}
of a graph are its maximal connected subgraphs. We denote by $X(u)$
the connected component of $X$ containing the vertex $u$.

A path is {\em closed} if its end-point is the same as its
start-point. A path is a{\em cycle} if its closed and it visits each
inner vertex exactly once. We will often identify a cycle with the
subgraph it induces and with any other cycle that induces the same
subgraph, so in terms of subgraphs a cycle is just a finite connected
2-valent subgraph.

A connected graph
without cycles is called a {\em tree}. It is
important to mention that every connected graph has at least one
spanning subgraph which is a tree, this is called a {\em spanning
  tree}. If $X$ is any graph, a {\em spanning forest} is a spanning
subgraph consisting of a spanning tree on each connected component.

Given two graphs $X=(V(X),D(X),(\cdot)^{-1}_X,I_X)$ and
$Y=(V(Y),D(Y),(\cdot)^{-1}_Y,I_Y)$, a {\em homomorphism} from $X$ to $Y$ is
a pair of functions $f=(f_1,f_2)$ (acting on the right) such that:
\begin{itemize}
\item $f_1:V(X)\to V(Y)$ and $f_2:D(X)\to D(Y)$.
\item For all $x\in D(X)$ we have that $I_Y(xf_2)=(I_X(x))f_1$ and
  $(xf_2)^{-1}_Y = (x^{-1}_X)f_2$.
\end{itemize}

We usually write $vf$ (for a vertex $v$) and $xf$ (for a dart $x$)
instead of $vf_1$ and $xf_2$ respectively. We also write $f:X\to
Y$, when $f$ is a homomorphism from $X$ to $Y$.

Note that the image of a link under a homomorphism can be any type of
edge, while the image of a loop cannot be a link and the image of a
semi-edge should always be a semi-edge.

The image of a connected graph under a homomorphism must also be
connected, since the image of a path is a path connecting the images
of its end-points.

If both parts of a homomorphism $f=(f_1,f_2):X \to Y$ are invertible
and $f^{-1}:=(f_1^{-1},f_2^{-1})$ is also a homomorphism, we say that
$f$ (and $f^{-1}$) is an {\em isomorphism}. Also, we say that $X$ and
$Y$ are {\em isomorphic} and write $X\cong Y$. The concept of {\em
  automorphism} is now intuitive.

%% A {\em coloring} of the vertices (resp. edges) of a graph $X$ is just a
%% function $c$ with the vertices (edges) of $X$ as its domain. If $x$ is
%% a vertex (resp. edge) and $c$ is a coloriing, the calue $c(x)$ is
%% referred to as the {\em color of $x$}. We will always think that the
%% darts of an edge have the same color as the edge. A coloring of
%% vertices (resp. edges) is {\em proper} if there are no
%% two adjacent vertices (resp. edges sharing an end-point) with the same
%% color.

\section{Flag graphs and maniplexes}\label{s:Maniplexes}

Given a flagged poset $\p$ of rank $n$, one can define a graph $\G(\p)$
associated to it, together with a $\{0,1,\ldots,n-1\}$ coloring of its
edges (that is, a function that assigns one of these numbers to each
edge). This graph is called the {\em flag graph} of $\p$. The vertices
of $\G(\p)$ are the flags of $\p$ and if two flags
are $i$-adjacent we draw a link of color $i$ between them.

In the case of a pre-polytope, each flag is $i$-adjacent to exactly
one other flag, which means that its flag graph is $n$-valent and the
coloring is {\em proper}, that is, no two darts of the same color start
at the same vertex. In this case, we can be more formal and
say that a dart of $\G(\p)$ is a pair $(\Phi,i)$ where $\Phi$ is a
flag and $i \in \{0,1,\ldots,n-1\}$. Then $I(\Phi,i):=\Phi$ and
$(\Phi,i)^{-1} := (\Phi^i,i)$ (recall that $\Phi^i$ is the only
$i$-adjacent flag to $\Phi$).

Let $i,j \in \{0,1,\ldots,n-1\}$ be such that $|i-j|>1$. Then, any
flag $\Phi$ of a pre-polytope $\p$ and its $i$-adjacent flag $\Phi^i$
have the same $j-1, j$ and $j+1$-faces. So their $j$-adjacent flags
should have the same $j$-face. In fact they have the same faces in
each rank except for $i$. In other words, $\Phi^{ij}$ is equal to
$\Phi^{ji}$ whenever $|i-j|>1$. In terms of the flag graph, this means
that the connected
components of the subgraph induced by the edges of colors $i$ and $j$
are a bunch of disjoint 4-cycles (whenever $|i-j|>1$).

In Figure~\ref{f:GrafPrisma} we see a triangular prism (in
stereographic projection)
transposed with its flag graph.

\begin{figure}
  \begin{center}
    \includegraphics[width=9cm]{GrafPrisma.pdf}
    \caption{\label{f:GrafPrisma} Flag graph of the triangular prism.}
  \end{center}
\end{figure}

%The following fact will not be used in the rest of this thesis, but
It is interesting to note that if $\p$ was only a flagged poset but
not a pre-polytope, something similar happens: given a flag $\Phi$ and
{\em one} of its $i$-adjacent flags $\Psi$, if for some $j$ with
$|i-j|>1$ one changes simultaneously the $j$-face of $\Phi$ and
$\Psi$ one would get $i$-adjacent flags $\Phi'$ and $\Psi'$. But in
this case the 4-cycle that these four flags form in the flag graph
would not necessarily be a connected component of the graph induced by
the edges of colors $i$ and $j$ as each vertex might be incident to
more than one edge of each color. %% However it would remain a fact
%% that if $W=x_1x_2$ is a path starting at a flag $\Phi$ and the colors
%% of $x_1$ and $x_2$ are $i$ and $j$ respectevely, then there are darts
%% $x_3$ and $x_4$ of colors $i$ and $j$ such that $W'=x_1x_2x_3x_4$ is a
%% closed path. NO ME ENCANTA ESTA REDACCIÓN!OBSOBS
That is, in the flag graph of a flagged poset every path consisting of
two edges of colors $i$ and $j$ with $|i-j|>1$ can be extended to a
4-cycle with alternating colors $i$ and $j$.

In the case of an abstract polytope $\p$, we can see that the
strong connectivity of $\p$ implies that its
flag graph is also connected. The flag graph of a polytope has
properties in common with the flag graph of a map (a 2-cellular
embedding of a connected graph on a surface). This is why Steve Wilson
\cite{Maniplexes} has introduced the concept of a {\em maniplex}
which generalizes both of these ideas.

There are lots of equivalent definitions of what a maniplex is. Here
we use the following one: an {\em $n$-maniplex} is a simple, connected
$n$-valent graph $\M$ together with a proper coloring of its edges
with colors $\{0,1,\ldots,n-1\}$ satisfying that if $|i-j|>1$, then
the connected components of the graph induced by the edges of colors
$i$ and $j$ are 4-cycles. The vertices of a maniplex are called {\em
  flags}. We will prefer Greek letters $\Phi$ and $\Psi$ for names of
flags.

It follows from the definition that each flag is incident to exactly
one edge of each color. Then, for each $i\in\{0,1,\ldots,n-1\}$ one
can define an involution $r_i$ on the flags of the maniplex that maps
each flag to the other end of the edge of color $i$ which is incident
to it. In other words $\Phi r_i=\Psi$ if and only if $\Phi$ and $\Psi$
are connected by an edge of color $i$ (in which case we say they are {\em
  $i$-adjacent}).

The permutations $r_i$ with $i\in \{0,1,\ldots,n-1\}$ are all
involutions with no fixed points and generate a group which acts
transitively on the flags of $\M$, since $\M$ is connected. They also
satisfy that if $|i-j|>1$ then $r_ir_j$ is also an involution with no
fixed points, or in other words, $r_i$ and $r_j$
commute~\footnote{This kind of ``far commutativity'' is pretty common
  in Mathematics (and in day to day life): the order of the factors
  does not affect the product as long as the factors are far enough
  from each other so that one does not affect what the other does. You
  can put on a shoe and a sock in any order and get the same result,
  as long as they are not on the same foot.}. One may use these
involutions also as an alternative definition of a maniplex, i.e. a
maniplex may also be defined as a set $\F$ whose elements are called
{\em flags}, and an indexed set of involutions $\{r_i\}_{i=0}^{n-1}$
of $\F$ satisfying:
\begin{itemize}
\item For every $i$ the involution $r_i$ has no fixed points.
\item If $\Phi r_i=\Phi r_j$ for some flag $\Phi$, then $i=j$.
\item The group $\gen{r_i:i=0,\ldots,n-1}$ acts transitively on $\F$.
\item If $|i-j|>1$ then $r_ir_j$ is an involution.
\end{itemize}
Note that these conditions imply that the involutions $r_ir_j$ have no
fixed points.

Since $\Phi r_i$ is the flag $i$-adjacent to $\Phi$ it is convenient to
denote it by $\Phi^i$ and to follow the same recursive notation as in
polytopes to define $\Phi^w$ where $w$ is a word on
$\{0,1,\ldots,n-1\}$.

The group $\gen{r_i:i=0,\ldots,n-1}$ is called the {\em monodromy} or
{\em connection} group of $\M$. In this thesis we will denote it by
$Mon(\M)$ and we will call each of its elements a {\em
  monodromy}. If $w$ is a word on the
alphabet $\{0,1,\ldots,n-1\}$ we identify $w$ with the monodromy
$x\mapsto x^w$, that is , we identify the word $=a_1a_2\ldots a_k$
with the monodromy $r_{a_1}r_{a_2}\ldots r_{a_k}$.

A {\em maniplex homomorphism} is a graph homomorphism that preserves
the color of the edges. The image of a dart under a  maniplex
homomorphism is completely determined by the image of its starting
point, so we may think of a maniplex homomorphism by considering only
its action on the flags. In other words, it is more convenient to
think of a maniplex homomorphism as a mapping between flags that
preserves $i$-adjacencies for all $i\in \{0,1,\ldots,n-1\}$.

In terms of the monodromy group, a function $\gamma:\M \to \M'$ is a
homomorphism if and only if it commutes with the monodromies,
i.e. $(\Phi^i)\gamma = (\Phi\gamma)^i$ for all $i\in
\{0,1,\ldots,n-1\}$ and $\Phi \in \F$ (which could be written as
$r_i\gamma = \gamma r_i$ for all $i \in \{0,1,\ldots,n-1\}$), or
equivalently $(\Phi^w)\gamma = (\Phi\gamma)^w$ for every monodromy $w$
(which could be written as $\omega\gamma = \gamma \omega$ for all
$\omega \in Mon(\M)$).

The notions of {\em isomorphism} and {\em automorphism} follow
naturally. As with polytopes, we denote the automorphism group of a
maniplex $\M$ by $\Gamma(\M)$. We will see later that the automorphism
group of $\p$ as a polytope coincides with that of $\G(\p)$ as a
maniplex, that is $\Gamma(\p) = \Gamma(\G(\p))$.

If $\Phi$ is a flag of a maniplex $\M$ and $\Psi$ is any other flag, there
exists a monodromy $w$ such that $\Psi=\Phi^w$. Then, if $\gamma:\M\to
\M'$ is a maniplex homomorphism, we have that $\Psi\gamma =
(\Phi^w)\gamma = (\Phi\gamma)^w$. This means that $\gamma$ is
completely determined by its action on only one flag ($\Phi$, for
example). In particular, the automorphism group of a maniplex acts {\em
  freely} on its flags. Of course, this is also true for polytopes.

A maniplex $\M$ also has a {\em dual} maniplex $\M^*$ which is obtained
simply by replacing each color $i$ by $n-1-i$. If $\M$ is the flag
graph of a polytope $\p$ is easy to see that $\M^*$ is the flag graph
of $\p^*$.

Just as with polytopes, the dual of a maniplex has the same
automorphism group as the original maniplex. A maniplex isomorphic to
its dual is called {\em self-dual}.

Let $\M$ be an $n$-maniplex. If $I\subset \{0,1,\ldots,n-1\}$, we
define $\M_I$ as the subgraph of $\M$ induced by the edges of colors
in $I$. If $i\in\{0,1,\ldots,n-1\}$, we use the symbol $\ol{i}$ to
denote the set $\{0,1,\ldots,n-1\}\setminus\{i\}$, and more generally,
if $K\subset \{0,1,\ldots,n-1\}$, we denote its complement by
$\ol{K}$. In particular $\M_{\ol{i}}$ is the subgraph of $\M$ obtained
by removing the edges of color $i$. We will use this notation also for
any graph with a coloring of its edges even if its not a maniplex.

Given the flag graph of a polytope $\p$, one may use the strong flag
connectedness to recover $\p$ from it. To do this, note that if two
flags $\Phi$ and $\Psi$ share the same $i$-face there should be a path
in the flag graph from $\Phi$ to $\Psi$ that does not use darts of
color $i$. Conversely, if there is such a path between $\Phi$ and
$\Psi$, since after traveling one dart one arrives to a flag with the
same faces except for the one with rank equal to the color of the dart,
then $\Phi$ and $\Psi$ (and every flag along the way) must have the
same $i$-face. This means that the set of flags with the same $i$-face
$F$ as $\Phi$ are the flags in the same connected component of the
subgraph obtained by erasing the edges of color $i$, that is
$\M_{\ol{i}}(\Phi)$. One may identify this connected component with
the $i$-face $F$.

Moreover, if an $i$-face $F$ and a $j$-face $G$ are incident, there
should be a flag $\Phi$ containing both of them. So the subgraphs
corresponding to $F$ and $G$ should have $\Phi$ in their
intersection. Conversely, if the subgraphs corresponding to $F$ and
$G$ have non-empty intersection, the flags in the intersection have
both $F$ and $G$ as elements, implying that $F$ and $G$ are
incident.

One may use this to get a ranked poset $\p(\M)$ from any maniplex
$\M$. The elements of rank $i$ of  the poset would be the connected
components of $\M_{\ol{i}}$. The order is then defined by the rule
$F<G$ if and only if $F\cap G \neq \emptyset$ and $\rk(F)<\rk(G)$,
where $\rk$ is the {\em rank} function of $\p$.

In \cite{PolyMani} it is proved that if $\M$ is any maniplex then
$\p(\M)$ is in fact a poset (actually it is a flagged poset).

Let $\p$ and $\p'$ be two isomorphic polytopes, let $\Phi$ be a flag
of $\p$ and let $\gamma:\p \to \p'$ be an
isomorphism. Then for every $i\in \{0,1,\ldots,n-1\}$, $\Phi\gamma$
and $(\Phi^i)\gamma$
should be $i$-adjacent flags of $\p'$, since they must have the same $j$-faces
for $j \neq i$ (since there pre-images do), and they must have a
different $i$-face (for the same reason). This means that $\gamma$
induces a maniplex homomorphism between the flag graphs of $\p$ and
$\p'$.

On the other hand, a maniplex homomorphism between $\G(\p)$ and
$\G(\p')$ would induce a homomorphism of polytopes between the faces
of $\p$ and $\p'$ which is defined by looking at the $i$-faces of $\p$
and $\p'$ as connected components of $\G(\p)_{\ol{i}}$ and
$\G(\p')_{\ol{i}}$ respectively.

We have sketched a proof of the following theorem (which appears in
\cite{PolyMani}).

\begin{teo}\label{t:GrafBand}
  Let $\p$ be a polytope and let $\M=\G(\p)$ be its flag graph. Then
  $\p$ is isomorphic (as a poset) to $\p(\M)$ and $\Gamma(\p) =
  \Gamma(\M)$.
\end{teo}

As an example one may look at Figure~\ref{f:GrafPrisma} and note
that in fact when we erase the edges of color 0 (blue) we get one connected
component around each vertex of the triangular prism; when we erase the
edges of color 1 (red) we get a connected component around each edge of
the triangular prism and that component will always be
a 4-cycle of colors 0 and 2; and finally when we erase the edges of
color 2 (green) we get a connected component inside each 2-face of the
triangular prism.

Theorem~\ref{t:GrafBand} means that all the information of the
polytope $\p$ is encoded in its flag graph. %ISA SUGIERE IMPLIES EN
                                %VEZ DE MEANS

Before moving on, we want to show how in addition to the faces we can
actually get every kind of chain of a polytope $\p$ from looking at
subgraphs of the flag graph $\p$. Let $K$ be a subset of
$\{0,1,\ldots,n-1\}$. A chain $c$ in $\p$ is of {\em type $K$} if it
has exactly one element of each rank in $K$.

Just as we noted that an $i$-face can be identified with a connected
component of $\M_{\ol{i}}$, a chain
of type $K$ may be identified with a connected component of
$\M_{\ol{K}}$: Let $c$ be a chain of type $K$, and let $\Phi$ be a
flag containing $c$. Due to the strong connectivity of $\p$, one can
get from $\Phi$ to another flag $\Psi$ by a path that does not uses
darts with colors in $K$ if and only if $\Psi$ also contains $c$.

%% In general, the converse of Theorem~\ref{t:GrafBand} is not true: a
%% maniplex $\M$ may not be isomorphic to the flag graph of its induced
%% poset $\p(\M)$. Moreover, this flag graph may not even be a
%% maniplex.

In \cite{PolyMani} Garza-Vargas and Hubard prove some
characterizations of {\em polytopal} maniplexes, i.e. those maniplexes
that are isomorphic to the flag graph of some polytope. These results
will be
summarized in Theorem~\ref{t:PolyMani}, which in a particular case
states that the converse
of Theorem~\ref{t:GrafBand} is also true. Before stating
Theorem~\ref{t:PolyMani} we need some more definitions.

\begin{Def}\label{d:PIP}
  Let $\M$ be an $n$-maniplex. We say that $\M$ satisfies the {\em
    strong path intersection property}  (or SPIP) if for every two
  subsets $I,J \subset \{0,1,\ldots,n-1\}$ and for any two flags $\Phi$ and
  $\Psi$, if there is a path $W$ from $\Phi$ to $\Psi$ using only darts of
  colors in $I$ and also a path $W'$ from $\Phi$ to $\Psi$ using only darts
  of colors in $J$, then there also exists a path $W''$ from $\Phi$ to
  $\Psi$ that uses only darts of colors in $I \cap J$.

  We say that $\M$ satisfies the {\em weak path intersection property}
  if for any two flags $\Phi$ and $\Psi$ and for all $k,m \in
  \{0,1,\ldots,n-1\}$, whenever there is a path $W$ from $\Phi$ to $\Psi$
  with only darts of color in $[0,m]:=\{0,1,\ldots,m\}$ and a path $W'$
  from $\Phi$ to $\Psi$ with only darts of colors in
  $[k,n-1]:=\{k,k+1,\ldots,n-1\}$, then there is also a path $W''$
  from $\Phi$ to $\Psi$ with only darts of colors in $[k,m]:=\{k,k+1,\ldots,m\}$.
\end{Def}

\begin{teo}\label{t:PolyMani}
  \cite{PolyMani} Let $\M$ be a maniplex. Then the following conditions are all
  equivalent:
  \begin{itemize}
  \item $\M$ satisfies the SPIP.
  \item $\M$ satisfies the WPIP.
  \item $\M$ is polytopal.
  \end{itemize}

  In any of these cases $\p(\M)$ is a polytope whose flag graph is
  isomorphic to $\M$.
\end{teo}



\section{Symmetry type graphs and Multi-maniplexes}\label{s:STG}

An important kind of homomorphisms are {\em covering
  homomorphisms}. We say that $p:X\to Y$ is a {\em covering
  homomorphism} (or a {\em covering} for short) if it is surjective and
for every vertex $v$ in $X$, the restriction of $p$ to the darts
starting in $x$ is a bijection with the darts starting on $xp$. In
particular, covering automorphisms preserve the valency of
vertices. In this case we also say that $X$ {\em covers} $Y$ or that
it is a {\em cover} of it.

% Given an equivalence relation $\sim$ on the vertices and darts of a
% graph $X$ (in which a vertex may not be equivalent to a dart), we may
% define a {\em quotient graph} $X/\sim$ in which the vertices and darts
% are the equivalence clases of vertices of $X$ and darts of $X$
% respectevely. If a dart $d$ starts at a vertex $x$, we define the
% starting point of the dart $[d]$ in $X/\sim$ to be $[x]$ and define
% the inverse of $[d]$ to be $[d^{-1}]$. This is a good definition in
% the sense that it does not depend on the representative chosen. One
% can see that the natural
% projection $\pi:x\mapsto [x],\; d\mapsto [d]$ is in fact a
% covering OBSOBS NOSIERTO. In fact the opposite is also true: if $p:X\to X'$ is a covering, then $X'$ is isomorphic to $X/\sim$ for some equivalence
% relation $\sim$. This equivalence relation is given by $x\sim y$ if
% and only if $xp = yp$ (whether $x$ and $y$ are vertices or darts). In
% conclusion, the graphs covered by a graph $X$ are exactly its
% quotients.

% OBSOBS: HABLAR DE ESTE PÁRRAFO CON ISA: UNA RELACIÓN ENTRE DARDOS
% INDUCE UNA RELACIÓN ENTRE VÉRTICES PERO NO VICEVERSA :/

A {\em covering transformation of $X$ with respect to a covering
  homomorphism $p$} is an automorphism of $X$ that leaves invariant
the {\em fibers} (pre-images of single points) of
$p$, that is, $fp=p$. These transformations also form a group, which we
denote by $CT(p)$. We say that $p$ is a {\em regular} covering if
$CT(p)$ acts regularly on each fiber of vertices, that is, if for any
vertices $v$ and $u$ in $X$ with $up=vp$ there is a (unique) covering
transformation $f$ such that $uf=v$. %(later we will see that when $X$
                                %is connected the uniqueness is
                                %implied).

Regular coverings are intimately related with the quotients of graphs
by subgroups of its automorphism group. %% If $\Gamma$
%% is the automorphisms group of a graph $X$ and $G\leq \Gamma$,
If $G$ acts on $X$ by automorphisms, then the
quotient graph $Y=X/G$ is defined as follows:
\begin{itemize}
\item The vertices of $Y$ are the orbits of vertices of $X$ under the
  action of $G$.
\item The darts of $Y$ are the orbits of the darts of $X$ under the
  action of $G$.
\item The starting point $I_Y(dG)$ of a dart $dG$ in $Y$ is $I_X(d)G$,
  where $I_X(d)$ is the starting point of $d$ in $X$.
\item The inverse dart of $dG$ is $d^{-1}G$ where $d^{-1}$ is the
  inverse dart of $d$ in $X$.
\end{itemize}
%In other words, the quotient graph $X/G$ is the quotient $X/{\sim_G}$
%where $x\sim_G y$ if there exists $\alpha \in G$ such that $x\alpha = y$.

One can verify that $X/G$ is well defined and
that the natural projection $\pi:X\to X/G$ is a regular covering with
covering transformations group $CT(\pi)=G$.

Conversely, if $p:X\to Y$ is a regular covering, then $Y$ is
isomorphic to $X/CT(p)$(see~\cite{TopAlg2}, for example).

Let $p:X\to Y$ be a covering and let $u$ and $v$ be vertices on $X$
and $Y$ respectively, such that $p(u)=v$. Let $W = y_1y_2\ldots y_k$
be a path on $Y$ starting in $v$. Since $p$ is a covering, there is a
unique dart $x_1$
starting in $u$ which is mapped to $y_1$. There is also a unique dart
$x_2$ starting at the end of $x_1$ which is mapped to $y_2$. In this
way, following a simple induction we get a unique path $\os{W}$
starting at $u$ and such that $\os{W}p=W$. This path $\os{W}$ is
called the {\em lift of $W$ starting at $u$}.

Let $X$ be a connected graph, let $p:X\to Y$ be a covering and let
$\alpha \in CT(p)$. Suppose $\alpha$
has a fixed point $x$, and let $x'$ be any other vertex in $X$. Let
$\os{W}$ be a path from $x$ to $x'$ and let $W:=\os{W}p$. Then
$W=\os{W}\alpha p$, which means that $\os{W}\alpha$ is a lift of $W$
starting at $x$, but since $\os{W}$ is the only lift of $W$ starting
at $x$, we get $\os{W}\alpha=\os{W}$, in particular $x'\alpha =
x'$. This proves $\alpha$ must be the identity, in other words,
$CT(p)$ acts freely on each fiber. In particular we have shown that to
prove that $p$ is regular we only have to prove that $CT(p)$ acts
transitively on each fiber (the uniqueness is given). Moreover, if we
know the action of $CT(p)$ on any fiber, we know its action on any
other fiber (using the connectedness as we just did), so it is enough
to prove that it acts transitively on {\em one} fiber.

\begin{lema}
  If $\varphi:\M \to \M'$ is a maniplex homomorphism then it is in
  fact a covering.
\end{lema}
\begin{dem}
  Recall that by the definition of a maniplex homomorphism, if $e$ is
  an edge in $\M$ of color $i$, then the edge $e\varphi$ of $\M'$ also
  has color $i$. Let $x$ be any flag in the image of $\varphi$. Let
  $y$ be any other
  flag in $\M'$. Then there is a path $W$ from $x$ to $y$. Let
  $\os{x}$ be a flag in $\M$ such that $\os{x} \varphi = x$. Let $\os{W}$
  be the path that starts in $\os{x}$ and follows exactly the same
  colors as $W$  (in fact, $\os{W}$ will be the lift of $W$) and let
  $\os{y}$ be its end flag. Since $\varphi$ is
  a maniplex homomorphism it must satisfy that $\os{W}\varphi = W$,
  which implies that $\os{y}\varphi = y$. This proves that $\varphi$
  is surjective.

  Now let $\os{z}$ be any vertex in $\M$ and let
  $z:=\os{z}\varphi$. Let $\os{d}$ be a dart starting at $\os{z}$. Then
  $\os{d}\varphi$ must be a dart starting at $z$ and having the same color
  as $\os{d}$. We know that there is exactly one such
  dart. Conversely, if $d$ is a dart starting at $z$, there is exactly
  one dart starting at $\os{z}$ with that same color. This proves that
  $\varphi$ is locally a bijection. \qed
\end{dem}

Given a maniplex $\M$ and a group $G\leq \Gamma(\M)$, the {\em
  symmetry type graph (STG) of $\M$ with respect to $G$}, denoted by
$\T(\M,G)$ is simply the quotient $\M/G$ where the color of the orbit
of each dart is the color of the dart itself. When $G = \Gamma(\M)$ we
omit it and call $\T(\M):=\T(\M,\Gamma(\M))$ the {\em symmetry type
  graph (STG) of $\M$}. We say that $\M$ is a {\em $k$-orbit} maniplex
if its STG $\T(\M)$ has exactly $k$-vertices. A {\em regular} maniplex
is a 1-orbit maniplex, that is, one in which the automorphism group
acts regularly on its flags. %% We denote the symmetry
%% type graph $\M$ with respect to its full automorphisms group simply by
%% $\T(\M)$ and we call it simply its {\em symmetry type graph (STG)}.

\begin{lema}\label{l:STGcubre}
  If $H$ is a subgroup of $G$ then $\T(\M,G)$ is covered by
  $\T(\M,H)$.
\end{lema}
\begin{dem}
  Let $\varphi:\T(\M,H) \to \T(\M,G)$ be defined by $(xH)\varphi :=
  xG$. This is in fact well defined, because $xH = yH \Rightarrow
  x^{-1}y \in H \subset G \Rightarrow  xG = yG$. Now recall that
  the monodromies and automorphisms of a maniplex commute, and thus,
  $(xH)^i = (x^i)H$. By applying $\varphi$ we get that  $(xH)^i\varphi
  (x^i)H\varphi = (x^i)G = (xG)^i$. This proves that $\varphi$ is a
  color preserving homomorphism. By the same logic that maniplex
  homomorphisms are coverings we may prove that this color preserving
  homomorphism is also a covering. \qed
\end{dem}

%% Let $H$ be a subrgoup of the full automorphism group of a maniplex
%% $\M$. Let $x$ and $y$ be vertices of $\T(\M,H)$. We will say that $x$
%% is {\em equivalent} to $y$ if they have the same image under the natural
%% homomorphism $\varphi:\T(\M,H) \to \T(\M)$ and we write $x\sim y$. It
%% is easy to see that $\sim$ is in fact an equivalence relation.

The {\em symmetry type graph of a \bf polytope} (with respect to a
group) is just the symmetry type of its flag graph (with respect to
the same group). A {\em $k$-orbit polytope} is one with a $k$-orbit
flag graph, that is, one with a STG with exactly $k$-vertices. {\em
  Regular} polytopes are just 1-orbit polytopes.

In Figure~\ref{f:STGPrisma} we see once again the flag
graph of a triangular prism, this time together with its symmetry type
graph. The vertices of the flag graph have been colored to show to
what orbit do they correspond on the symmetry type graph.

\begin{figure}
  \begin{center}
    \includegraphics[width=9cm]{STGPrisma.pdf}
    \caption{\label{f:STGPrisma} Flag graph of the triangular prism
      together with its symmetry type graph. The color of the vertices
      on the flag graph
      corresponds to the color of their orbit on the symmetry type graph.}
  \end{center}
\end{figure}

In Section~\ref{s:Maniplexes} we discussed that there is a natural
correspondence between the $i$-faces of a polytope $\p$ and the
connected components of its flag graph $\G(\p)_{\ol{i}}$. Let $G$ be a
group of automorphisms of $\p$ and let
$p:\G(\p)\to \T(\p,G)$ be the natural projection. Let $F$ be an
$i$-face of $\p$ and let $\Phi$ and
$\Psi$ be two flags through $F$. Then $\Phi$ and $\Psi$ are connected
by a path $W$ that does not use the color $i$. After applying $p$ we
get that $\Phi p$ and $\Psi p$ are connected by the path $W p$ which
does not use the color $i$. We have thus proven that the orbits of the
flags that share a particular $i$-face are in the same connected
component of $\T(\p,G)_{\ol{i}}$.

Now let $F'$ be another $i$-face in the same $G$-orbit as $F$. Let
$\gamma \in G$ be such that $F'\gamma = F$. Let $\Phi'$ be flag
through $F'$. Then $\Phi'\gamma$ is a flag through $F$. By
construction, $\Phi' p = (\Phi'\gamma) p$, which means that $\Phi' p$
is in the same connected component of $\T(\p,G)_{\ol{i}}$ as $\Phi
p$.

Conversely, if two flags $\Phi$ and $\Phi'$ are such that $\Phi p$ and
$\Phi' p$ are connected by a path $W$ that does not use the color $i$,
then there is a lift $\os(W)$ of this path connecting $\Phi$ to a flag
$\Psi$ in the same orbit as $\Phi'$. Then there exists $\gamma\in G$
such that $\Psi = \Phi' \gamma$. By taking the $i$-face of both sides
we get $\Psi_i = \Phi'_i \gamma$, but $\Psi_i = \Phi_i$, since they
are connected by a path that does not use the color $i$. We conclude
then that the $i$-faces $Phi_i$ and $\Phi'_i$ are on the same
$G$-orbit.

We have proved proposition~\ref{p:iCompsSTG}:

\begin{prop}\label{p:iCompsSTG}
  Let $\p$ be an $n$-polytope and let $G$ be a group of automorphisms
  of $\p$. Let $i\in \{0,1,\ldots, n-1\}$. Then the connected
  components of $\T(\p,G)_{\ol{i}}$ correspond to the $G$-orbits of
  $i$-faces of $\p$,
  i.e., two flags have $i$-faces in the same $G$-orbit if and only if
  their orbits are in the same connected component of
  $\T(\p,G)_{\ol{i}}$.
\end{prop}

Just as we did for the flag graph, this result can be generalized when
we consider many colors instead of just one:

\begin{prop}\label{p:CompsSTG}
    Let $\p$ be an $n$-polytope and let $G$ be a group of automorphisms
  of $\p$. Let $K\subset \{0,1,\ldots, n-1\}$. Then the connected
  components of $\T(\p,G)_{\ol{K}}$ correspond to the $G$-orbits of
  chains of type
  $K$ of $\p$, i.e., two flags have subchains of type $K$ in the same
  $G$-orbit if and only if
  their orbits are in the same connected component of
  $\T(\p,G)_{\ol{K}}$.
\end{prop}

In Figure~\ref{f:STGcaras} we see how after removing the edges of color
2 from the STG of the triangular prism we get one connected component
per 2-face orbit. The square 2-faces are in cyan and brown flags, while
triangular 2-faces are only in magenta flags. In
Figure~\ref{f:STGcaras-aristas} we see that if we remove edges of colors
1 and 2 from the STG of the triangular prism we get one connected
component per orbit of chains of type $\{1,2\}$, that is, incident
pairs of the form $C=\{e,F\}$ where $e$ is an edge and $F$ a 2-face. If
$F$ is a triangle, $C$ is contained only in magenta flags, if $e$ is
in a triangle but $F$ is a square all flags containing $F$ are cyan,
and if $e$ is shared by two squares all flags containing $C$ are
brown.

\begin{figure}
  \centering
  \includegraphics[width=9cm]{STGcaras.pdf}
  \caption{When we remove edges of color 2 from the STG of the prism
    we get one component for each 2-face orbit.}
  \label{f:STGcaras}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=9cm]{STGcaras-aristas.pdf}
  \caption{When we remove edges of colors 1 and 2 from the STG of the
    prism we get one component for each orbit of chains of type
    $\{1,2\}$.}
  \label{f:STGcaras-aristas}
\end{figure}

Let $\M$ be a maniplex, $G$ a group of automorphisms of
$\M$, and $p:\M\to \T(\M,G)$ the natural covering
homomorphism. Since $\M$ is connected and $p$ is a homomorphism,
$\T(\M,G)$ is also connected. Since each flag of $\M$ is incident to
exactly one edge of each color in $\{0,1,\ldots,n-1\}$ and $p$ is a
covering, the same must be true for $\T(\M,G)$, even though
$\T(\M,G)$ might not be simple. And finally, if $|i-j|>1$ then a path
of length 4 that alternates the colors of its darts between $i$ and
$j$ must end at the point where it started, (i.e. it must be {\em
  closed}), and since $p$ is a covering, the same must be true for
$T(\M,G)$, but in this case it might visit each vertex more
than once, i.e. it might be any quotient of a 4-cycle (see
Figure~\ref{f:ijComponentes}). These necessary properties determine
what we will call in this thesis a {\em multi-maniplex}~\footnote{In
  previous works, like~\cite{k-orb} what we call {\em
    multi-maniplexes} has been called {\em allowable graphs}. The
  author of this thesis thinks that the name {\em allowable graph} is
  too generic and prefers the name {\em multi-maniplex} that compares
  to {\em maniplex} in the same way that {\em multi-graph} compares to
  {\em graph}.}.

\begin{figure}
  \begin{center}
    \includegraphics[width=6cm]{ijComponentes.pdf}
    \caption{\label{f:ijComponentes} In the STG of a maniplex and any
      multi-maniplex, if $|i-j|>1$ the possible connected components of
      the graph induced by edges of colors $i$ and $j$ are any of the
      ones shown in this figure. These are the quotients of a
      4-cycle.}
  \end{center}
\end{figure}

\begin{Def}
  A {\em multi-maniplex} of rank $n$ is a connected $n$-valent graph
  $X$ together with a coloring of its edges $c:D(X)\to
  \{0,1,\ldots,n-1\}$ satisfying that each vertex is incident to
  exactly one edge of each color and that paths of length 4 that
  alternate between darts of two non-consecutive colors are closed.
\end{Def}

A {\em homomorphism} $h:X\to Y$ between multi-maniplexes is just a
graph homomorphism that preserves the color of the edges. The notions
of {\em isomorphism} and {\em automorphism} follow in a natural
way. We may also talk about {\em coverings} in multi-maniplexes, but
just as in maniplexes they happen to be the same as homomorphisms.

A multi-maniplex may also be defined by its {\em monodromy group},
that is, the group generated by the permutations $r_i$ which map each
vertex to the end-point of the dart of color $i$ starting at that
vertex. Just as in the case of maniplexes, these permutations are
involutions and commute when their indices are far apart. More
precisely, for all $i,j\in \{0,1,\ldots,n-1\}$ it is satisfied that
$r_i^2=1$ and $r_ir_j=r_jr_i$ whenever $|i-j|>1$. Because of the
connectivity we have that $Mon(X):=\gen{r_i\mid 0\leq i \leq n-1}$ acts
transitively on the vertices of $X$. On contrast with maniplexes,
since multi-maniplexes are not necessarily simple, we cannot assure
that $xr_i\neq x$ for a vertex $x$ or that $xr_i=xr_j$ implies $i=j$.

A multi-maniplex $X$ also has a {\em dual} multi-maniplex $X^*$ which
is obtained (just as with maniplexes) by replacing each color $i$ with
$n-1-i$. Once again, the dual of a multi-maniplex has the same
automorphism group as the multi-maniplex. As suspected, it is easy to
see that if $X$ is the STG of a maniplex $\M$ (or a polytope $\p$)
with respect to some group, then $X^*$ is the STG of $\M^*$ with
respect to the same group.


A multi-maniplex isomorphic to its dual is called {\em self-dual}.

%\section{Our main problems}

%% The present thesis focuses on two main questions. The first task is to
%% characterize symmetry type graphs of polytopes and maniplexes. We know
%% that they are multi-maniplexes, but what are other necessary
%% conditions (if any)?.

When studying polytopes  and maniplexes together with their STGs, the
following two questions occur naturally.

\begin{preg}\label{preg:EsSTG}
  Given a multi-maniplex $X$ how do we know if there exists a polytope
  (or a maniplex) whose STG is isomorphic to $X$?
\end{preg}

\begin{preg}\label{preg:EsAut}
  Given a multi-maniplex $X$ and a group $G$, how do we know if there is
  a polytope $\p$ (or a maniplex $\M$) such that $STG(\p,G) \cong X$ (or
  $STG(\M,G) \cong X$)? How do we know if $G$ is the full automorphism
  group of $\p$ (or $\M$) or just a subgroup?
\end{preg}

These two questions are the motivation for this thesis. The second
part of Question~\ref{preg:EsAut} emphasizes why
Question~\ref{preg:EsSTG} is not as trivial as it may initially look
like.

In this thesis we will give some advances in answering these questions.

\section{Regular polytopes}\label{s:Regular}

Question~\ref{preg:EsAut} has been answered for regular polytopes
\cite{ARP} and also
2-orbit polytopes \cite{2OrbPol1}. In this section we will outline the
method used for regular polytopes so that in further chapters we can
use similar techniques.

%We should explore the meaning of Theorem~\ref{t:Regulares}.
Let $\p$ be a regular polytope and let $\Phi$ be any flag of
$\p$. Then for every $i$ there is an automorphism that maps $\Phi$ to
its $i$-adjacent flag $\Phi^i$. We denote such an automorphism by
$\rho_i$. By applying $\rho_i$ twice we notice that $\Phi\rho_i^2 =
(\Phi^i)\rho_i = (\Phi\rho_i)^i = \Phi$, and since the action of the
automorphisms is free, we have that $\rho_i$ must be an involution.

Now consider some other flag $\Psi$. Since $\p$ is regular there
is an automorphism $\gamma \in \Gamma(\p)$ such that
$\Psi=\Phi\gamma$. Let $w=i_1i_2\ldots i_k$ be a word in $\{0,1,\ldots,n-1\}$
such that $\Psi=\Phi^w$. Now let
$\sigma=\rho_{i_k}\rho_{i_{k-1}}\ldots \rho_{i_1}$. Then one can
verify with a simple induction that $\Phi\sigma = \Phi^w = \Psi =
\Phi\gamma$, and since the action is free this implies that $\sigma =
\gamma$. We have actually proved that the set
$\{\rho_0,\rho_1,\ldots,\rho_{n-1}\}$ generates the whole automorphism
group of $\p$. The automorphisms $\rho_0,\rho_1,\ldots,\rho_{n-1}$ are
called the {\em distinguished generators of $\Gamma(\p)$ with respect
  to $\Phi$}.

Moreover, we can notice that for any set $I \subset
\{0,1,\ldots,n-1\}$, the orbit of $\Phi$ under the group
$\gen{\rho_i\mid i\in I}$ coincides with its orbit under the group
$\gen{r_i\mid i\in I}$ which consists of those flags that have the same
$j$-faces as $\Phi$ for  $j\notin I$. Note that this is not true for
an arbitrary flag $\Psi$, just for the flag with respect to which we
are taking these generators (and other flags in its orbit).

This actually has to do with the following proposition, which can be
found in \cite{ARP}.

\begin{prop}\label{p:anti-iso}
  Let $\p$ be a regular polytope with automorphism group $\Gamma(\p)$
  and monodromy group $Mon(\p)=\gen{r_0,r_1,\ldots,r_{n-1}}$. Let
  $\rho_0,\rho_1,\ldots,\rho_{n-1}$ be the distinguished generators of
  $\Gamma(\p)$ with respect to some flag $\Phi$. Then the map
  \[
  r_{i_1}r_{i_2}\ldots r_{i_{k-1}}r_{i_k} \mapsto
  \rho_{i_k}\rho_{i_{k-1}}\ldots \rho_{i_2}\rho_{i_1}
  \]

  is a group anti-isomorphism.
\end{prop}

Also as a consequence of Proposition~\ref{p:anti-iso} we have that if
$|i-j|>1$ then $\rho_i\rho_j$ must be an involution (since $r_jr_i$
is). Since the generators are also involutions one might write this
as $\rho_i\rho_j = \rho_j\rho_i$ whenever $|i-j|>1$.

For every $I \subset \{0,1,\ldots,n-1\}$ let $\Gamma_I$ be the
subgroup of $\Gamma$ generated by $\{r_i\mid i\in I\}$. For $I,J \subset
\{0,1,\ldots, n-1\}$ let consider an element $\gamma$ in the
intersection $\Gamma_I \cap \Gamma_J$. We noticed before that since
$\gamma$ is in $\Gamma_I$ we know that $\Phi\gamma$ has the same
$i$-faces as $\Phi$ for any $i$ not in $I$, but this is also true for
$i$ not in $J$. So if we denote the complement of $A$ in
$\{0,1,\ldots,n-1\}$ by $\ol{A}$ we have that $(\Phi\gamma)_i = \Phi_i$
for all $i$ in $\ol{I} \cup \ol{J}$, which by De Morgan's law is equal to
$\ol{I\cap J}$. This means that there is an element of $\Gamma_{I \cap
  J}$ that maps $\Phi$ to $\Phi\gamma$, but since the action is free,
this element should be $\gamma$ itself.

We have proved the following result:

\begin{prop}\label{p:IntPropReg}
  If $\Gamma$ is the automorphism group of a regular polytope and
  $\{\rho_0,\rho_1,\ldots,\rho_{n-1}\}$ are its distinguished generators
  with respect to some flag $\Phi$ then

  \begin{equation}\label{eq:IntPropReg}
    \forall I,J\subset \{0,1,\ldots,n-1\} \quad \gen{\rho_i\mid i\in I}
    \cap \gen{\rho_i\mid i\in J} = \gen{\rho_i\mid i\in I\cap J}.
  \end{equation}
\end{prop}

The property~\ref{eq:IntPropReg} is known as the {\em
  intersection property (for regular polytopes)}.

We have found two properties about the automorphism group of a regular
polytope: the intersection property and the far commutativity. In
\cite{EgonPhd} it is proved that these properties are in fact enough
to ensure that the group is the automorphism group of a regular
polytope:

\begin{teo}\label{t:Regulares}
  \cite{EgonPhd} Let $\Gamma$ be a group. Then there is a regular
  polytope $\p(\Gamma)$ having
  $\Gamma$ as its automorphism group if and only if $\Gamma$ is
  generated by a
  set of involutions $\{\rho_0,\rho_1,\ldots,\rho_{n-1}\}$ satisfying
  the intersection property~(\ref{eq:IntPropReg}) and that if
  $|i-j|>1$ then $\rho_i\rho_j$ is also an involution.
\end{teo}

A group generated by involutions satisfying the conditions of
Theorem~\ref{t:Regulares} is called a {\em string C-group}. The
canonical examples are the so called {\em string Coxeter groups},
which are groups $\Gamma$ with a presentation
\[
  \Gamma=\gen{\rho_0,\rho_1,\ldots,\rho_{n-1} |
    (\rho_i\rho_j)=(\rho_{i-1}\rho_i)^{p_i}=1\; (|i-j|>1)},
\]
where $p_i$ is either a positive integer or infinity\footnote{A
  relation $(\rho_{i-1}\rho_i)^\infty=1$ just means that the order of
  $(\rho_{i-1}\rho_i)$ is infinite. The relation may be ignored when
  constructing the group as a quotient of a free group by the
  normalizer of the elements of $R$.} for each
$i\in\{1,2,\ldots,n-1\}$. If $p_i=\infty$ for all $i$, $\Gamma$ is
called {\em the universal string Coxeter group}, and it is the
automorphism group of {\em the universal polytope of rank $n$}. It is
known~\cite{ARP} that if $\U$ is the universal polytope of rank $n$
and $\p$ is any other polytope there is a covering $p:\G(\U)\to\G(\p)$
(where $\G$ denotes the flag graph of its argument). Moreover, one can
see that for any multi-maniplex $X$ there is a covering
$p:\G(\U)\to X$. In particular this means that for every
multi-maniplex there exists some group $G$ such that $X=\T(\U,G)$,
giving a partial answer to Question~\ref{preg:EsSTG}, but only when
$X$ has only one vertex this is the actual symmetry type graph of
$\U$.

We have sketched a proof of one implication in
Theorem~\ref{t:Regulares}. For the other one we need to construct a
polytope starting from the group $\Gamma$ and its generators
$\{\rho_0,\rho_1,\ldots,\rho_{n-1}\}$. To do this we have to make some
observations about the case when we already know that $\Gamma$ is the
automorphism group of a polytope $\p$.

The first observation is that if we denote by $\ol{i}$ the set
$\{0,1,\ldots,n-1\}\setminus \{i\}$, we have that $\Gamma_{\ol{i}}$
should be the stabilizer of $\Phi_i$ (the $i$-face of the base
flag). This is because as we have noted, the elements of
$\Gamma_{\ol{i}}$ are precisely those that map $\Phi$ to a flag with the
same $i$-face.

Now consider any other $i$-face $F$. Since $\p$ is regular, there is
an element $\gamma \in \Gamma$ mapping $\Phi_i$ to $F$. Let $\sigma \in
\Gamma$ be any other element that maps $\Phi_i$ to $F$. Then
$\sigma\gamma^{-1}$ should stabilize $\Phi_i$, so $\sigma \in
\Gamma_{\ol{i}}\,\gamma$. So the coset $\Gamma_{\ol{i}}\gamma$
consists precisely of those automorphisms that map $\Phi_i$ to $F$. So
it is natural to associate this coset with the $i$-face $F$.

So to construct a polytope $\p(\Gamma)$ from a group $\Gamma$ first we
define its $i$-faces to be simply the right cosets of
$\Gamma_{\ol{i}}$.

Then we need to define the incidence relation. This is easy as well:
if $F<H$ there should be a flag $\Psi$ that includes both of them. Let
$\gamma \in \Gamma$ be such that $\Psi = \Phi\gamma$. If $F$ is
associate it with the coset $\Gamma_{\ol{i}}\,\sigma$ and $H$ is
associate it with $\Gamma_{\ol{j}}\, \tau$, then $\gamma \in
\Gamma_{\ol{i}}\,\sigma \cap \Gamma_{\ol{j}}\, \tau$.

So the obvious way to define the order relation in $\p(\Gamma)$ is the
following:

\[
\Gamma_{\ol{i}}\,\sigma <  \Gamma_{\ol{j}}\,\tau \quad {\rm if\; and\;
  only\; if} \quad \Gamma_{\ol{i}}\,\sigma \cap \Gamma_{\ol{j}}\, \tau
\neq \emptyset \quad {\rm and} \quad i<j.
\]

In \cite{ARP} and \cite{EgonPhd} it is proved that the poset
$(\p(\Gamma),<)$ is in fact a regular polytope and its automorphism
group is $\Gamma$. Analogous results have being found for 2-orbit
polyhedra (2-orbit polytopes of rank 3) \cite{2OrbPol1}, chiral
polytopes (a special kind of 2-orbit
polytopes)~\cite{QuiralesEgonAsia} and finally for all 2-orbit
polytopes \cite{2OrbPol2}.

In this thesis we will generalize these results for arbitrary
$k$-orbit polytopes. More concretely, in Chapter~\ref{ch:3Orb} we find
an analogous result for 3-orbit polyhedra and in
Chapter~\ref{ch:IntProp} we explore the results for 3-orbit polyhedra
to find a generalization for polytopes with any symmetry type graph.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Tesis_partida"
%%% End:


==> Caterpillars1.tex <==

\section{Example: Caterpillars}\label{s:Caterpillars}
%\isa{Vender m\'as caros los caterpillars}
If one wants to build polytopes from premaniplexes in the way we have described in this paper, it is natural to start with infinite families of premaniplexes. 
One could, of course, then start with premaniplexes with a fixed number $k$ of vertices. For example, one may want to construct 2-orbit polytopes (see \cite{IsaEgon2orbit}).
If, on the other hand, we do not want to limit the number of vertices of the premaniplexes in the family a first step could be to consider trees. However, since semi-edges are considered as cycles, there are no premaniplexes whose underlying graph (without colors) is a tree. Thus, we study the closest thing to them: premaniplexes that are trees with an unlimited number of semi-edges.
Hence, we define a {\em caterpillar} as a premaniplex in which every cycles contains at least one semi-edge.
In other words, a caterpillar is a premaniplex $X$ with a
unique spanning tree. 

In particular, a
caterpillar does not have pairs of parallel links (edges joining different vertices). If there are three
links  incident to one vertex, at
least two of them must have colors differing by more than 1, which
would imply that there is a 4-cycle. This implies that caterpillars
consist in fact of a single path $P$ (which we will call {\em the
  underlying path of $X$}) and lots of semi-edges. Of course, the
colors of two consecutive edges on the path must differ by exactly
one, otherwise there would be a 4-cycle.
We note here that the term {\em caterpillar} has been used in the graph theory literature for a very similar but slightly different concept.


Throughout this section, unless otherwise stated, $X$ will denote a finite caterpillar (that is, one with a finite number of vertices) with underlying path $P$, and its vertices will be labeled by $x_0, x_1,\ldots, x_k$, ordered as they are visited by $P$.
Furthermore, we denote by $(x_i,j)$ the dart of color $j$ at $x_i$ and by $c_i$ the color of the link connecting $x_{i-1}$ and $x_i$.


\begin{figure}
  \begin{center}
    \includegraphics[width=5cm]{caterpillar.pdf}
    \caption{\label{f:caterpillar} A finite caterpillar.}
  \end{center}
\end{figure}

We want to assign voltages to the semi-edges of $X$ in order to get the flag graph of a polytope as the derived maniplex.
To this end, we note that in caterpillars the conditions of Theorems~\ref{t:IntProp-w} and~\ref{t:IntProp} can be simplified, as stated in the following lemma:

\begin{lema}\label{l:IntPropCat}
  Let $X$ be a caterpillar and let $\xi:\Pi(X)\to\Gamma$ be a voltage
  assignment such that all the darts in the underlying path of $X$
  have trivial voltage. Then the following statements are equivalent.
  \begin{enumerate}
  \item $X^\xi$ is polytopal.
  \item For every vertex $x$ in $x$ and all sets
    $I,J\subset\{0,1,\ldots,n-1\}$ the equation
    \[
      \xi(\Pi_I^x(X))\cap \xi(\Pi_J^x(X)) = \xi(\Pi^x_{I\cap J}(X))
    \]
    holds.
    \item For every vertex $x$ in $X$ and all
      $k,m\in\{0,1,\ldots,n-1\}$ the equation
      \[
        \xi(\Pi_{[0,m]}^x(X))\cap \xi(\Pi_{[k,n-1]}^x(X)) =
        \xi(\Pi^x_{[k,m]}(X))
      \]
      holds.
  \end{enumerate}
\end{lema}

\begin{dem}
  To prove this we have to see that for every set of colors
  $I\subset \{0,1,\ldots, n-1\}$ the set $\xi(\Pi^{x,y}_I(X))$ is either
  $\xi(\Pi^x_I(X))$ or empty, depending on whether or not the segment of
  $P$ that goes from $x$ to $y$ (which we will denote $[x,y]$) uses or
  not only colors in $I$. In fact if $[x,y]$ uses only colors in
  $I$ then
  \[
    \xi(\Pi^{x,y}_I(X)) = \xi(\Pi^x_I(X) [x,y]) =
    \xi([x,y])\xi(\Pi^x_I(X)) = 1\cdot \xi(\Pi^x_I(X)) =
    \xi(\Pi^x_I(X)).
  \]

  Note also that $\xi(\Pi^{x,y}_I(X)) \cap \xi(\Pi^{x,y}_J(X))$
  is empty if and only if one of the factors is empty. These
  observations together with Theorems~\ref{t:IntProp-w} prove the
  equivalence between conditions 1 and 2, and with
  Theorem~\ref{t:IntProp} we prove the equivalence between conditions
  1 and 3, thus proving the lemma. \qed
  % So it is enough
  % to prove
  % that the intersection properties are satisfied for fundamental groups
  % based on each vertex, i.e. we have to prove that $\xi(\Pi^x_I) \cap
  % \xi(\Pi^x_J) = \xi(\Pi^x_{I \cap J})$ for each vertex $x$ and  $I,J
  % \subset \{0,\ldots,n-1\}$.
\end{dem}

Recall that a {\em Boolean group} (or an {\em elementary abelian $2$-group}) is a group in which every
non-trivial element has order exactly 2. Thus, all Boolean
groups are abelian, and finitely generated Boolean groups are
isomorphic to a direct product of cyclic groups of order 2.


\begin{prop}\label{p:Caterpillars1}
  Every caterpillar is the quotient of the flag graph of a polytope
  by a Boolean group.
\end{prop}

\begin{dem}
  Let $X$ be a caterpillar. 
  We shall find a Boolean group $B$ and a voltage assignment $\xi:\Pi(X)\to B$ such that $X^\xi$ is polytopal in the following way.
%  The simplest way to define this voltage assignment is to first  assign a different generator of a Boolean group to each semi-edge and then take the quotient by the subgroup generated by  4-paths with alternating far away colors.

%  A more algorithmic way to get the same result would be the following:

  First give the trivial voltage to all links of $P$ and a different voltage to each semi-edge incident to $x_0$. 
  We shall give voltage assignments to the semi-edges $(x_i,j)$, recursively on $i$. 
  To do so, define $\delta_i:=c_{i+1}-c_i$ for $i=1,\ldots,k-1$, and note that $\delta_i \in  \{-1,1\}$, as otherwise $X$ would have a $4$-cycle without semi-edges.
  There are two cases to consider to assign the voltage of $(x_i,j)$, for $i<k$:
  \begin{itemize}
      \item $j\neq c_i-\delta_i$. 
      In this case $(x_{i-1},j)$ is a semi-edge because $j$ differs from $c_i$ in more than $1$, and the links incident to $x_{i-1}$ have colors $c_i$ and  $c_{i-1}=c_i+\delta_{i-1}$.
      This implies that the path $(x_{i-1},c_i)(x_i,j)(x_i,c_i)(x_{i-1},j)$ must have trivial voltage.
      Hence, we assign to the semi-edge $(x_i,j)$ the same voltage as the one that $(x_{i-1},j)$ has.
      \item $j= c_i-\delta_i$. In this case, we assign a new generator of a Boolean group as the voltage of  $(x_i,j)$.
  \end{itemize}
  %  Now, recursively on $i$, if $(x_i,j)$ is a
 % semi-edge and $j \neq c_i-\delta_i$ assign to this semi-edge
  %the same voltage as the one from $(x_{i-1},j)$ (we know that
 % $(x_{i-1},j)$ is a semi-edge because $j$ differs from $c_i$ in more
 % than 1, and the links incident to $x_{i-1}$ have colors $c_i$ and
 % $c_{i-1}=c_i+\delta_{i-1}$). We do this because the
 % path $(x_{i-1},c_i)(x_i,j)(x_i,c_i)(x_{i-1},j)$ must have trivial
 % voltage. If $j=c_i-\delta_i$
 % assign a new generator of a Boolean group as the voltage of
%  $(x_i,j)$. 
  Finally, since $\delta_k$ is undefined, we assign new
  generators as the voltages of the darts $(x_k,c_k+1)$ and
  $(x_k,c_k-1)$
  (if they exist) and  for the other semi-edges on $x_k$ copy the
  voltage of the semi-edge of the same color on $x_{k-1}$. 
  
  Let us call
  the resulting voltage group $B$ and denote this
  voltage assignment by $\xi$. By Lemma~\ref{l:VoltMani}, $X^\xi$ is a maniplex.

  Note further that $\xi$ satisfies that if $i\in
  \{1,2,\ldots,k\}$; $r,s\in \{0,1,\ldots,n-1\}$ and $(x_{i-1},r)$ and
  $(x_i,s)$ are semi-edges, then $\xi(x_i,s) = \xi(x_{i-1},r)$ if and
  only if $r=s$ and $|r-c_i|\neq 1$. It also satisfies that if
  $i<\ell<j$ and $(x_i,r)$ and $(x_j,r)$ are semi-edges such that
  $\xi(x_i,r) = \xi(x_j,r) = \gamma$, then $(x_\ell,r)$ is also a
  semi-edge and $\xi(x_\ell,r) = \gamma$.

% This voltage assignment gives in fact a maniplex. 
  We claim that the second statement of Lemma~\ref{l:IntPropCat} is satisfied, and
  hence, $X^\xi$ is the flag graph of a polytope.
To show that this is the case, start by noticing that $\xi(\Pi^x_I)$ is the group generated by the voltages of the semi-edges on the component $X_I(x)$.

  Given $I, J \subseteq \{0,1, \dots, n-1\}$, suppose that for some vertex $x$ there is a semi-edge $e$ in
  $X_I(x)$ and a semi-edge $e'$ in $X_J(x)$ with
  $\xi(e) = \xi(e') = \gamma$ for some $\gamma \in \Gamma$. If $e=e'$
  then $e \in X_{I\cap J}(x)$. If $e\neq e'$ then we have that for
  some $i,j\in \{0,\ldots,k-1\}$ and some $r \in \{0,\ldots,n-1\}$
  occurs that $e=(x_i,r)$ and $e'=(x_j,r)$; in particular
  $r\in I\cap J$.
  % OBSOBS QUITO ESTO
  % and the segment $[x_i,x_j]$ does not use
  % the colors $r \pm 1$ (otherwise $\xi(e) \neq \xi(e')$ by
  % construction). Moreover $[x_i,x_j]$ uses only colors either greater
  % than $r+1$ or smaller than $r-1$. If $x\in [x_i,x_j]$, since $r\in I
  % \cap J$ we have that $(x,r) \in X_{I \cap J}(x)$ and its voltage is
  % $\gamma$.
  % FIN DE QUITO ESTO.
  If $x\in [x_i,x_j]$ then, as previously observed,
  $\xi(x,r) = \gamma$ (see Figure~\ref{f:IntPropCat_caso1}) and since
  $(x,r) \in X_{I \cap J}(x)$ this means $\gamma$ is a generator of
  $\xi(\Pi^x_{I\cap J})$. If $x\notin [x_i, x_j]$ consider without
  loss of generality that $x_i$ is further away from $x$ than $x_j$,
  in other words, that $x_j \in [x_i,x]$ (see Figure~\ref{f:IntPropCat_caso2}). Then
  $[x_i,x]$ uses only colors in $I$ and $[x_j,x] \subset [x_i,x]$ uses
  only colors in $J$. Then since $[x_j,x] \subset [x_i,x]$ we know
  that $[x_j,x]$ uses only colors in $I \cap J$, meaning that
  $e' \in X_{I \cap J}(x)$ and since its voltage is $\gamma$, this
  shows that $\gamma$ is always a generator of
  $\xi(\Pi^x_{I \cap J})$. Therefore, we have shown that if $\gamma$ is a
  generator of both $\xi(\Pi^x_I(X))$ and $\xi(\Pi^x_J(X))$, then it
  is also a generator of $\xi(\Pi^x_{I \cap J}(X))$.

  Now let $\sigma\in \xi(\Pi^x_I(X)) \cap \xi(\Pi^x_J(X))$ be
  arbitrary. Since the group $B$ is Boolean, $\sigma$ may be written
  as $\sigma=\gamma_1\gamma_2\ldots \gamma_s$ where the elements
  $\gamma_1, \gamma_2,\ldots, \gamma_s$ are different generators of
  $B$, and this decomposition is unique up to reordering of the
  factors. Since $\sigma \in \xi(\Pi^x_I(X))$, and because the voltage
  of a semi-edge is always a generator, each $\gamma_i$ is also in
  $\xi(\Pi^x_I(X))$, and since $\sigma \in \xi(\Pi^x_J(X))$ each
  $\gamma_i$ is also in $\xi(\Pi^x_J(X))$. But, this implies that each $\gamma_i$ is in
  $\xi(\Pi^x_{I\cap J}(X))$, implying that
  $\sigma \in \xi(\Pi^x_{I\cap J}(X))$. Therefore,
  $\xi(\Pi^x_I) \cap \xi(\Pi^x_J) = \xi(\Pi^x_{I \cap J})$. \qed
\end{dem}

\begin{figure}%[h]
  \centering
  \includegraphics[width=7.5cm]{IntPropCat_caso1.pdf}
  \caption{If $x\in[x_i,x_j]$ then $(x,r)$ has voltage
    $\gamma\in \xi(\Pi^x_{I\cap J}(X))$.}
  \label{f:IntPropCat_caso1}
\end{figure}

\begin{figure}%[h]
  \centering
  \includegraphics[width=7.5cm]{IntPropCat_caso2.pdf}
  \caption{If $x_j\in[x_i,x]$ then $e'=(x_j,r)$ is in
    $X_{I\cap J}(x)$ and has voltage $\gamma$.}
  \label{f:IntPropCat_caso2}
\end{figure}

Proposition~\ref{p:Caterpillars1} is still true for infinite
caterpillars. Even if our algorithmic way of assigning voltages may
not be doable, the voltage assignment is still well defined as a
quotient of the Boolean group with one generator assigned to each
semi-edge.

Note that Proposition~\ref{p:Caterpillars1} says that every caterpillar $X$ is a symmetry type graph of a polytope $\p$ with respect to some group $B\leq \Aut(\p)$. 
However need not happen that $X$ is the symmetry type graph of $\p$ with respect to the full automorphism group.
That is, $X^\xi$ might have ``extra'' symmetry.
%Now we are concerned with whether or not the group $B$ as constructed in the proof of Proposition~\ref{p:Caterpillars1} is the full automorphism of $X^\xi$. 
Thus, we would want to investigate what could be the
symmetry type of $X^\xi$ with respect to its full automorphism group.

Let us first introduce some concepts.

Given a caterpillar, let us call an {\em end-point} a vertex incident
to just one link (those are the end-points of the underlying
path). Note that a caterpillar is finite if and only if it has exactly
two end-points. Every symmetry must map end-points to end-points. If a
caterpillar is finite there is at most one non-trivial symmetry and
its action on the vertices $x_0,x_1,\ldots,x_k$ is given by
$x_j\mapsto x_{k-j}$. We will call a finite caterpillar {\em
  symmetric} if it has a non-trivial symmetry.

Recall that a {\em word} $w$ in $\{0,1,\ldots,n-1\}$ is simply a
finite sequence $w=a_1a_2\ldots a_t$, with $a_i\in \{0,1,\ldots,n-1\}$
for each $i=1,2,\ldots,t$. The {\em inverse} of a word $w$
is the word $w^{-1}$ that has the same colors as $w$ but written in
reverse order, that is, if $w=a_1a_2\ldots a_t$ then $w^{-1} =
a_ta_{t-1}\ldots a_1$. A word is {\em reduced} if it has no occurrence
of the same color twice in a row, that is $w=a_1a_2\ldots a_t$ is
reduced if and only if $a_{i+1}\neq a_i$ for all
$i=1,2,\ldots,t-1$. We will work with reduced words from now on. A
word $w=a_1a_2\ldots a_t$ is a {\em palindrome} if  $a_i = a_{t+1-i}$
for all $i\in \{1,2,\ldots,t\}$. A palindrome word of even length can
be written as $vv^{-1}$ for some word $v$ and is necessarily not
reduced. A palindrome word of odd length can always be written as
$w=vav^{-1}$ for some color $a$ and some word $v$.

Given a segment $[x,y]$ in a caterpillar, its {\em underlying word} is
the word $w$ consisting of the colors of the links in the path that
goes from $x$ to $y$. When we speak of the {\em underlying word} of a
caterpillar $X$ we are referring to the underlying word of its
underlying path in a fixed orientation.

Let us call a segment $[x,y]$ a {\em palindrome} if its underlying word
$v$ is a palindrome.

\begin{prop}\label{p:CubsCat}
  Let $X$ be a finite caterpillar and let $Y$ be a premaniplex not
  isomorphic to $X$ %with at least 2 vertices and
  such that there is a premaniplex homomorphism (or covering)
  $h:X\to Y$. Then $Y$ is a caterpillar. Moreover, if $Y$ has at least
  2 vertices and $S=c_1c_2\ldots c_k$ is the underlying word of $X$,
  then there is some $r<k$ such that $w=c_1c_2\ldots c_r$ is the
  underlying word of $Y$ and one of the following statements is true:
  \begin{enumerate}
  \item There exist colors $a_1,a_2,\ldots,a_t \in \{c_r+1,c_r-1\}$ and
    $b_1,b_2\ldots,b_{t-1} \in \{c_1+1,c_1-1\}$ such that
    $S=wa_1w^{-1}b_1wa_2w^{-1}b_2\ldots b_{t-1}wa_tw^{-1}$.
  \item There exist colors $a_1,a_2,\ldots,a_t\in \{c_r+1,c_r-1\}$ and
    $b_1,b_2\ldots,b_t \in \{c_1+1,c_1-1\}$ such that
    $S=wa_1w^{-1}b_1wa_2w^{-1}b_2\ldots b_{t-1}wa_tw^{-1}b_tw$.
  \end{enumerate}

  In any case, if $i \equiv j \md 2r+2$ then $h(x_i) = h(x_j)$. Also
  if $i \equiv -j-1 \md 2r+2$ % and $\floor{\frac{i}{r+1}} \not\equiv
  % \floor{\frac{j}{r+1}} \md 2$
  then $h(x_i) = h(x_j)$% (here
  % $\floor{x}$ denotes the integer part of $x$)
  .
\end{prop}

Before proving Proposition~\ref{p:CubsCat} let us remark that it
simply means that the quotients of a caterpillar $X$ are those
caterpillars $Y$ such that $X$ can be ``folded'' into $Y$. We
illustrate this concept in Figure~\ref{f:FoldedCat}: the semi-edges
are not drawn and the names of the vertices have been omitted, but the
idea is that $X$ must be ``folded'' into ``layers'' of $r+1$ vertices
and then each vertex will be projected to the vertex on $Y$ in the
same horizontal coordinate. The layer $\ell$ consists of the vertices
$x_i$ where $\floor{\frac{i}{r+1}}=\ell$ ($\floor{x}$ denotes the
integer part of $x$). Even layers go from left to right, while odd
layers go from right to left, hence the underlying word of even layers
is $w=c_1c_2\ldots c_r$ while the underlying word of odd layers is
$w^{-1}=c_rc_{r-1}\ldots c_1$.

\begin{figure}%[h!]
  \centering
  \begin{subfigure}[t]{0.45\linewidth}
    \includegraphics[width=6cm]{FoldCat1.pdf}
    \caption{Case 1}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.45\linewidth}
    \includegraphics[width=6cm]{FoldCat2.pdf}
    \caption{Case 2}
  \end{subfigure}
  \caption{The caterpillar $X$ covers the caterpillar $Y$ if and only
    if it ``folds'' into it.}
  \label{f:FoldedCat}
\end{figure}

Now let us proceed with the proof.

\begin{dem}
  Let us consider the equivalence relation $\sim_h$ on $X$ given by
  $x\sim_hy$ if and only if $h(x)=h(y)$. Recall that by the definition
  of a premaniplex homomorphism $x\sim_h y$ implies that $x^m\sim_h
  y^m$ for every monodromy $m$. We have actually showed that $Y$ is
  isomorphic to $X/\sim_h$.

  We already know that all premaniplex homomorphisms are surjective
  (see Section~\ref{s:STG}). By hypothesis $h$ is not an isomorphism,
  which implies it cannot be injective. Let $x$ and $y$ be two
  different vertices on $X$ such that $x\sim_h y$. Let
  $x_0,x_1,\ldots, x_k$ be the sequence of vertices in the underlying
  path of $X$. There is a monodromy $m$ such that $x^m=x_0$, and so
  $x_0\sim_h y^m$ and $y^m$ is different than $x_0$. Now let $q$ be
  the minimum positive number such that $x_q\sim x_0$. We know that
  $q$ exists because $x_0\sim_h y^m$. Note that if
  $q=1$ we would have that $x_0^i\sim_h x_0$ for all $i$, which would
  imply that the same is true for $x_1$ and in turn also for
  $x_2=x_1^{c_2}$ and so on. This would mean that all the vertices of
  $X$ are equivalent, meaning that $Y$ has only one vertex and the
  proposition follows. So we may assume that $q>1$.

  We know that $x_{q-1} = x_q^{c_q}$ is equivalent $x_0^{c_q}$. If
  $c_q \neq c_1$, we would have that $x_0^{c_q}=x_0$. This would imply
  that $x_{q-1}$ is equivalent to $x_0$, contradicting the minimality
  of $q$. So we have proven that $c_q = c_1$.

  Now note that if for some $\ell$ we have that $x_\ell\sim x_1$, then
  $x_\ell^{c_1}\sim x_1^{c_1}=x_0$. In particular this tells us that
  for $\ell<q-1$, $x_\ell$ cannot be equivalent to $x_1$. Now we can
  use the same argument we used to prove that $c_q=c_1$ to prove that
  $c_{q-1}=c_2$. Analogously we can prove that
  $c_3 = c_{q-2}, c_4=c_{q-3}$ and so on. In other words, $[x_0,x_q]$
  is a palindrome. Since for all $i$, $c_i$ and $c_{i+1}$ are
  different, then $q$ is odd, say $q=2r+1$. Let $v$ be the underlying
  word of the segment $[x_0,x_q]$. Then $v$ may be written as
  $v=wc_{r+1}w^{-1}$ for some word $w = c_1c_2\ldots c_r$. Let us call
  $a_1:=c_{r+1}$ and note that $a_1\in \{c_r+1,c_r-1\}$.

  For all $i=0,1,\ldots, k$, let us denote by $\widehat{i}$ the
  residue of dividing $i$ by $2r+2$. We will prove by induction on $i$
  that $x_i\sim_h x_{\widehat{i}}$ for all $i=0,1,\ldots, k$ and that
  $c_{i} = c_{\widehat{i}}$ when $i$ is not divisible by $r+1$,
  $c_i \in \{c_1+1,c_1-1\}$ if $i$ is an odd multiple of $r+1$ and
  $c_i= \{c_r+1,c_r-1\}$ when $i$ is an even multiple of $r+1$.

  Let our induction hypothesis be that $x_{\ell}\sim_h
  x_{\widehat{\ell}}$ for all $\ell<i$, and that
  $c_{\ell} = c_{\widehat{\ell}}$ if $\ell$ is not divisible by $r+1$.
  % This will prove
  % that  if $i\equiv j \md
  % 2r+2$ then $x_i\sim_h x_j$. Moreover, if $i \equiv -j-1 \md 2r+2$,
  % then $\widehat{i}= 2r+1 -\widehat{j}$. Note that since $v$ is
  % a palindrome, then $x_\ell\sim_h x_{2r+1-\ell}$ for
  % $\ell=0,1,\ldots,2r+1$, in particular $x_{\widehat{j}} \sim_h
  % x_{2r+1-\widehat{j}} = x_{\widehat{i}}$
  % and this
  % implies that if $i \equiv -j-1 \md 2r+2$ and
  % $\floor{\frac{i}{r+1}} \not\equiv \floor{\frac{j}{r+1}} \md 2$ then
  % $x_i\sim_h x_j$.

  % We will also
  % assume that $c_{i-1} = c_{\widehat{i-1}}$  but {\bf only}
  % when $\ell$ is not divisible by $r+1$. We will prove that
  % $c_i=c_{\,\widehat{i}}$ when $i$ is not divisible by $r+1$, that
  %  This would prove that $X$ has the structure suggested in the
  % statement of the theorem.

  Let us start with the case when $i\equiv 0 \md 2r+2$. In this case
  we want to prove that $x_i \sim_h x_{\widehat{i}}$ and that
  $c_i\in \{c_1+1,c_1-1\}$. By our induction hypothesis we know that
  $x_{i-1}\sim_hx_{2r+1} \sim_h x_0$ and $c_{i-1}=c_{2r+1}=c_1$. In
  particular $c_i\in \{c_1+1,c_1-1\}$.  This implies that
  $x_i=x_{i-1}^{c_i}\sim_h x_0^{c_i}=x_0=x_{\,\widehat{i}}$ (since
  $c_i\neq c_1$). Thus $i$ satisfies our claim.

  Now let us proceed with the case when $i$ is an odd multiple of
  $r+1$, that is $\widehat{i} = r+1$. In this case we want to prove
  that $x_i \sim_h x_{\widehat{i}}$ and that $c_i\in
  \{c_r+1,c_r-1\}$. Our induction hypothesis tells us that
  $x_{i-1}\sim_h x_r$ and that $c_{i-1}=c_r$. Hence
  $c_i \in \{c_r+1,c_r-1\}$. Note that one of the colors in
  $\{c_r+1,c_r-1\}$ is actually $c_{r+1}$, while the other is the
  color of a semi-edge incident to $x_r$. Since $x_{r+1}\sim_h x_r$ we
  have that
  $x_i=x_{i-1}^{c_i}\sim_h x_r^{c_i}\sim_h x_r\sim_h x_{r+1} =
  x_{\,\widehat{i}}$. Thus $i$ satisfies our claim.

  Finally let us prove our claim for the case when $i$ is not
  divisible by $r+1$. Our induction hypothesis tells us that
  $x_{i-1}\sim_h x_{\widehat{i-1}}$. Note that
  $\widehat{i} = \widehat{i-1}+1$. Since $i$ is not a multiple of
  $r+1$ we know that
  $x_{\,\widehat{i}}=x_{\widehat{i-1}}^{c_{\,\widehat{i}}}$ is not
  equivalent to $x_{\widehat{i-1}}$. This implies that
  $x_{i-1}^{c_{\,\widehat{i}}}$ is not equivalent to $x_{i-1}$, and
  since it is adjacent to $x_{i-1}$ it must be equal to either $x_i$
  or $x_{i-2}$. If $i\equiv 1 \md r+1$ then by induction hypothesis
  $x_{i-1}\sim_h x_0$, but recall that $x_0\sim_h x_{2r+1}=x_q$ by
  definition, and by induction hypothesis
  $x_{i-2}\sim_h x_{\widehat{i-2}} = x_{2r+1}$. This means that
  $x_{i-2}\sim_h x_{i-1}$, so $x_{i-1}^{c_{\,\widehat{i}}}$ must be
  $x_i$, implying that $ c_i=c_{\,\widehat{i}}$. If
  $i\not\equiv 1 \md r+1$ then our induction hypothesis tells us that
  $c_{i-1}=c_{\widehat{i-1}} \neq c_{\,\widehat{i}}$, and since
  $x_{i-2}=x_{i-1}^{c_{i-1}}=x_{i-1}^{c_{\widehat{i-1}}}$, so the only
  possibility is that $x_{i-1}^{c_{\,\widehat{i}}} = x_i$, implying that
  $c_i=c_{\,\widehat{i}}$ and that $x_i\sim_h x_{\,\widehat{i}}$. Thus,
  $i$ satisfies our claim. Note that we have also proven that if $i$
  is not divisible by $r+1$ then $x_{i-1}$ cannot be an end-point of
  $X$.

  We have proved that $x_i\sim_h x_{\,\widehat{i}}$ for all
  $i=0,1,\ldots, k$. This implies automatically that if $i\equiv j \md
  2r+2$ then $x_i\sim_h x_j$. Moreover, if $i\equiv -j-1 \md 2r+2$,
  then $\widehat{i} = 2r+1-\widehat{j}$. Now since $v$ is a
  palindrome, we know that $x_\ell \sim_h x_{2r+1-\ell}$ for all
  $\ell=0,1,\ldots, 2r+1$, in particular $x_{\,\widehat{i}} =
  x_{2r+1-\widehat{j}} \sim_h x_{\,\widehat{j}}$. This, together with the
  fact that $x_i \sim_h x_{\,\widehat{i}}$ and $x_j \sim_h
  x_{\,\widehat{j}}$, implies that $x_i \sim_h x_j$.

  We have already proved that $S=wa_1w^{-1}b_1wa_2w^{-1}\ldots$ and it
  ends after an occurrence of $w$ or $w^{-1}$. To end the prove note
  that since $h$ is surjective we already know exactly what
  premaniplex $Y$ is: It is a caterpillar with vertex sequence
  $h(x_0), h(x_1),\ldots, h(x_r)$. In fact, for $i=1,\ldots,r-1$ and
  $j=0,1,\ldots n-1$ we know that $h(x_i)$ is different from
  $h(x_i)^j=h(x_i^j)$ if and only if $j\in\{c_{i-1},c_i\}$; and if
  $i=0$ (resp. $r$) then $h(x_i)$ is different from $h(x_i)^j$ if and
  only if $j=c_1$ (resp. $c_r$). \qed


  % If $j=k$, that is, if $x_j$ is an end-point of $X$, there is nothing
  % left to prove. Otherwise, let $b_1:=c_{j+1}$ and note that since
  % $c_j=c_1$ we have that $b_1\in \{c_1+1,c_1-1\}$. Note that since
  % $x_j\sim_h x_0$ and $(x_0,c_{j+1})$ is a semi-edge, we know that
  % $x_{j+1}=x_j^{c_{j+1}}\sim x_0^{c_{j+1}} = x_0$. On the other hand,
  % $x_1 = x_0^{c_1}\nsim_h x_0$ (unless $Y$ has only one vertex, in
  % which case there is nothing left to prove), which means that
  % $x_{j+1}^{c_1}\nsim_h x_{j+1}$. Then $c_{j+2} = c_1$ and
  % $x_{j+2}\sim_h x_1$. Repeating this argument we get that $c_{j+3} =
  % c_2$ and $x_{j+3}\sim x_2$; $c_{j+4} = c_3$ and $x_{j+4}\sim x_3$,
  % and so on; until we get to $c_{j+r+1} = c_r$ and $x_{j+r+1}\sim
  % x_r$. Now, since $x_{r+1} = x_r^{c_{r+1}}\sim x_r$, then
  % $x_{j+r+1}^{c_{r+1}}\sim x_{j+r+1}$, so this {\em might} be an end
  % point. Otherwise, it will be $a_2$-adjacent to $x_{j+r+2}$ for some
  % $a_2 \in \{c_r+1,c_r-1\}$ (since $c_{j+r+2} = c_r$).
  % % can also be $c_{r+1}$-adjacent to $x_{j+r+2}$,
  % % or even $(2c_r-c_{r+1})$-adjacent to $x_{j+r+2}$. These are the only
  % % options, since $c_{j+r+3}$ must differ from $c_{j+r+2} = c_r$ by
  % % exactly 1.
  % If we continue, we get to another vertex
  % ($x_{j+2r+2} = x_{2j+1}$) which is equivalent to $x_0$. %Now, since $X$
  % % is not symmetric this is not an end point, so
  % This vertex may be $b_2$-adjacent to $x_{2j+2}$ for some $b_2\in
  % \{c_1+1,c_1-1\}$ (since $c_{2j+2}=c_1$).

  % Proceeding with this logic we  get to the desired result. OBSOBS NO
  % SÉ CÓMO HACER QUE LA DEMOSTRACIÓN SE ENTIENDA BIEN Y A LA VEZ SEA
  % FORMAL. \qed
\end{dem}

%   see that if $S$ is the sequence of
%   colors of the path $P$ starting by the first end-point, then $S$ must
%   be of the type $S = wa_1w^{-1}bwa_2w^{-1}bwa_3w^{-1}b\ldots$, where
%   $a_i = c_r\pm 1$ and $(c_1,b) \in \{(1,0),(n-2,n-1)\}$.

%   If $X$ is finite $S$ must end
% after an ocurrence of $w$ or $w^{-1}$. If $S$ ends after an
% occurrence of $w^{-1}$, say $S =
% wa_1w^{-1}bwa_2w^{-1}bwa_3w^{-1}b\ldots a_tw^{-1}$, then there must
% be at least one $i$ for which $a_i \neq a_{t+1-i}$, so that $S$ is not
% itself a palindrome (which would make the caterpillar symmetric). We
% should also consider that $S^{-1}$ must have the same structure, which
% is not automatic if $S$ ends after an occurence of $w$.

% In conclusion we get the following stronger theorem, which really
% restricts the structure of possible caterpillars that are not the STG
% of a polytope with a boolean automorphism group:

% \end{dem}

If we look closely at the proof of Proposition~\ref{p:CubsCat} we will
notice that we have not actually used the fact that $X$ is finite, but
only the fact that it has at least one end-point. So the proposition
may be generalized to the following one:

\begin{prop}\label{p:CubsCat1end}
  Let $X$ be a caterpillar with at least one end-point and let $Y$ be a premaniplex
  such that there is a premaniplex homomorphism (or covering) $h:X\to
  Y$. Then $Y$ is a caterpillar. Moreover, if $S=c_1c_2\ldots $ is
  the color sequence of $X$ starting at its end-point, there is some
  $r$ such that $w=c_1c_2\ldots c_r$ is the underlying word of $Y$
  and there exist colors $a_1,a_2,\ldots \in \{c_r+1,c_r-1\}$ and
    $b_1,b_2\ldots \in \{c_1+1,c_1-1\}$ such that
    $S=wa_1w^{-1}b_1wa_2w^{-1}b_2\ldots $. If $X$ is finite it ends
    after an occurrence of either $w$ or $w^{-1}$. If $i \equiv j \md
    2r+2$ then $h(x_i) = h(x_j)$. Also if $i \equiv -j \md 2r+1$ and
    $\floor{\frac{i}{r+1}} \not\equiv \floor{\frac{j}{r+1}} \md 2$
    then $h(x_i) = h(x_j)$.
\end{prop}

% OBSOBS  LOS GUSANOS SIN FINALES PARECEN COMPLICARSE POR LAS SIMETRÍAS
% DE TRASLACIÓN. ¿PONGO ALGO AL RESPECTO?

Let us look now at the degenerate cases. If $Y$ is only one vertex we
can think that the previous theorems still hold but with $w$ being the
empty word, and since $c_1$ and $c_r$ do not exist, we get rid of the
restrictions $a_i\in \{c_r+1,c_r-1\}$ and $b_i\in \{c_1+1,c_1-1\}$. In
Figure~\ref{f:FoldedCat} $X$ would have only one vertex and no links
per layer; essentially $X$ would be ``standing up'' instead of being
folded. If $Y$ is isomorphic to $X$ then $S=w$ and we do have no $a_i$
or $b_i$. In Figure~\ref{f:FoldedCat} $X$ would have only one layer.

Given a caterpillar, we have given a voltage assignment $\xi$ with a
Boolean voltage group $B$ such that $X^\xi$ is polytopal (see
Proposition~\ref{p:Caterpillars1}). Now we want to know when can we
claim that $B$ is the full automorphism group of $X^\xi$, or in other
words, when can we claim that $X$ is the STG of $X^\xi$.

Let $X$ be a finite caterpillar and let $\xi:\Pi(X)\to B$ be the
voltage assignment constructed in the proof of
Proposition~\ref{p:Caterpillars1}. If $X$ is symmetric, its
non-trivial symmetry induces an automorphism of $B$ which is just a
reordering of the generators, moreover, if the generators are given
the natural order, it induces the reverse order on the
generators. This implies that this symmetry always lifts (see
Theorem~\ref{t:Levanta}), so in this case the original caterpillar is
not the symmetry type of the derived polytope. But we will see in
Theorem~\ref{t:Caterpillars} that if this is not the case we can
almost be certain that the caterpillar is in fact the symmetry type
graph of the derived polytope by its full automorphism group. In this
case, by ``almost'' we mean that if this is not the case, the
caterpillar must have a very specific structure.

\begin{teo}\label{t:Caterpillars}
  Let $X$ be a finite caterpillar of length $k$ and rank $n$. Let
  $S=c_1c_2\ldots c_k$ be the underlying word of $X$. Then at
  least one of the following statements is true:
  \begin{enumerate}
  \item $X$ is symmetric.
  \item $X$ is the STG of a polytope with a Boolean automorphism
    group.
  \item $c_1$ is in $\{1,n-2\}$ and there exist $r\in
    \{1,2,\ldots,k-1\}$, and
    $a_1,a_2,\ldots,a_t \in \{0,1,\ldots,n-1\}$ where
    $t=(k+1)/(2r+2)$, such that
    $S=wa_1w^{-1}bwa_2w^{-1}b\ldots bwa_tw^{-1}$ where $w=c_1c_2\ldots
    c_r$ and %$(c_1,b) \in \{(1,0),(n-2,n-1)\}$.
    $b=0$ if $c_1=1$ and $b=n-1$ if $c_1=n-2$.
  \item There exist $r\in \{1,2,\ldots,k-1\}$ and
    $a,b \in \{0,n-1\}$ such that
    \[
      S=waw^{-1}bwaw^{-1}b\ldots bwaw^{-1}bw,
    \]
    where $w=c_1c_2\ldots c_r$. Also
    $(c_1,b), (c_r,a) \in \{(1,0),(n-2,n-1)\}$.
  \end{enumerate}
\end{teo}
\begin{dem}
  Suppose that $X$ is not symmetric and that it is not the STG of a
  polytope with a Boolean automorphism group. %% We want to prove that
  %% $(c_1,c_2)\in \{(1,0),(n-2,n-1)\}$ (for the pair $(c_k,c_{k-1})$ we
  %% would have a completely analogous proof).

  Consider the voltage
  assignment $\xi:\Pi(X)\to B$ previously discussed. We say that
  two vertices $x$ and $y$ of $X$ are equivalent ($x\sim y$) if there
  exist (or equivalently, for all) $\sigma,\tau \in B$ such that
  the flags $(x,\sigma)$ and $(y,\tau)$ of $X^\xi$ are in the same
  orbit under the action of the automorphism group of $X^\xi$. Then
  $\sim$ is an equivalence relation preserved by $i$-adjacency,
  that is $x\sim y \Rightarrow x^i\sim y^i$. Moreover,
  the natural function $h:X\to X/\sim$ is a premaniplex
  homomorphism, so by Proposition~\ref{p:CubsCat} there
  exists some $r$ such that the $S$ can be written
  as $wa_1w^{-1}b_1wa_2w^{-1}b_2\ldots $ ending after an occurrence of
  either $w$ or $w^{-1}$, where $w=c_1c_2\ldots c_r$, $a_i\in
  \{c_r+1,c_r-1\}$ and $b_i\in \{c_1+1,c_1-1\}$ (see
  Figure~\ref{f:FoldedCat}).

  %AHORITA VEMOS QUE ONDA CON ESTO  The proof that there is a palindrome
  %segment $[x_i,x_k]$ is completely analogous.

  Note that since $X$
  is not symmetric nor the STG of $X^\xi$ with respect to $B$, at
  least $b_1$ exists. Let $j\in\{0,1\ldots,k-1\}$ be a number such
  that the segment $[x_0,x_{j+1}]$ has the underlying word
  $wa_1w^{-1}b_1wa_2w^-1b_2\ldots w^{-1}b_i$ for some $i$. We know in
  particular that $b_i$ differs from $c_1$ in exactly 1. We want to
  prove that $(c_1,b_i) \in \{(1,0),(n-2,n-1)\}$. Let us assume this
  is not the case. We will get to a contradiction.

  Let $q$ be the {\em other} color that differs from
  $b_i$ in exactly 1 (that is $q = 2b_i - c_1$). Since $(c_1,b_i) \neq
  (1,0),(n-2,n-1)$ we know that $q\in \{0,1,\ldots,n-1\}$, and thus is
  the color of some edges of $X$. So there
  are semi-edges $e,e'$ incident
  to $x_0$ of colors $q$ and $b_i$ respectively. Let
  $\alpha:=\xi(e)$ and $\beta:=\xi(e')$. The voltage of the closed
  path $ee'ee'$ is $(\beta\alpha)^2 = 1$ because $B$ is Boolean. This
  means that its lift, (the path of length 4 that starts at $(x,1)$ in
  $X^\xi$ and  alternates colors between $q$ and $b_i$) must be closed.

  %Now let us check two cases:
  %
  % \noindent {\bf Case 1: The dart $(x_{j+1},r)$ is a link.} In
  % this case the path in $X$ of length 4 that alternates colors between
  % $r$ and $b_i$ and starts at  $x_j$ is not closed (after three steps
  % it is at $x_{j+2}$), so its lift cannot  be closed either.

  % \begin{figure}[h]
  %   \begin{center}
  %     \includegraphics[width=7cm]{CatCaso1.pdf}
  %     \caption{\label{f:CatCaso1} Case 1.}
  %   \end{center}
  % \end{figure}

  % \noindent {\bf Case 1: The dart $(x_{j+1},r)$ is a semi-edge.}
  By Theorem~\ref{p:CubsCat}, we know that $c_{j+1} = c_1 \neq q$, so
  we know that the darts $(x_{j+1},q)$ and $(x_j,q)$ are
  semi-edges. Let $\kappa := \xi(x_j,q)$ and
  $\lambda = \xi(x_{j+1},q)$. The path of length 4 that alternates
  colors between $r$ and $b_i$ and starts at $x_j$ is closed, and its
  voltage is $\lambda\kappa$. Note that since $|q-b_i|=1$ the
  construction of $\xi$ tells us that
  $\xi(x_j,q) \neq \xi(x_{j+1},q)$, that is $\lambda \neq \kappa$,
  which implies $\lambda\kappa \neq 1$. This means that the path of
  length 4 in $X^\xi$ starting at $(x_j,1)$ and alternating colors
  between $r$ and $b_i$ is not closed (it ends at
  $(x_j,\lambda\kappa)$.

    \begin{figure}%[h]
    \begin{center}
      \includegraphics[width=7cm]{CatCaso2.pdf}
      \caption{\label{f:CatCaso2} %Case2
        The voltage of the path that alternates colors between $r$ and
        $b_i$ starting at $x_j$ is $\lambda\kappa\neq 1$.}
    \end{center}
  \end{figure}

  % In both cases w
  We see that the path of length 4 in $X^\xi$ starting at $(x_j,1)$
  and alternating colors between $r$ and $c_{j+1}$ is not closed, but
  the one starting at $(x_0,1)$ is. This contradicts the fact that
  $(x_j,1)$ and $(x_0,1)$ are on the same orbit. The contradiction
  comes from the fact that there are edges of color
  $q = 2b_i -c_1 \in \{0,1,\ldots,n-1\}$, so to avoid this we must
  have that $(c_1,b_i) \in \{(1,0),(n-2,n-1)\}$. Since $c_1$ is fixed,
  every $b_i$ must be the same.

  % , so we have finished the proof.
  %The proof that $(c_k,c_i)\in\{(1,0),(n-2,n-1)\}$ is completely
  %analogous. \qed

  If the underlying word of $X$ ends after an occurrence of $w$ we
  may look at $X$ in the other direction. Then the previous result
  tells us that every $a_i$ is equal to some $a$ and that $(c_r,a)\in
  \{(1,0), (n-2,n-1)\}$. \qed
\end{dem}

 \begin{obs}
   If the third or fourth condition is the one holding in
   Theorem~\ref{t:Caterpillars}, the actual STG of $X^\xi$ is the
   finite caterpillar with underlying word $w$.
 \end{obs}

By doing exactly the same proof, we obtain the following analogous
result for infinite caterpillars with one end-point (this would
  look like a ray or half-straight line):

\begin{teo}\label{t:Caterpillars1end}
  Let $X$ be an infinite caterpillar with one end-point. Let $S$ be
  the sequence of colors of the underlying path of $X$ starting at its
  end-point. Then one of the following statements is true:
  \begin{enumerate}
  \item $X$ is the STG of a polytope with a Boolean automorphism
    group.
  \item There exist some number $r$ and colors
    $b,a_1,a_2,\ldots,a_t \in \{0,1,\ldots,n-1\}$ such that
    $S=wa_1w^{-1}bwa_2w^{-1}bwa_3w^{-1}\ldots$ where $w=c_1c_2\ldots
    c_r$ and $(c_1,b) \in \{(1,0),(n-2,n-1)\}$.
  \end{enumerate}
\end{teo}

% OBSOBS GUSANOS SIN FINALES?

% Let us examine more deeply the structure of a caterpillar that is
% neigther symmetric nor the STG of a polytope with boolean automorphism
% group.

% Let $X$ be a caterpillar with at least one end-point (finite or infinite) and
% suppose that it is neigther symmetric or the STG of a polytope with a
% boolean group. According to Theorems~\ref{t:Caterpillars}
% and~\ref{t:Caterpillars1end}, the underlying path of $X$  must start
% with a
% palindrome segment $[x_0,x_j]$. Let $v = c_1c_2\ldots c_j$ be the
% palindrome word describing the colors of this segment. Since $v$ is a
% palindrome and it may not have the same color twice in a row, $j$ must
% be odd, say $j=2r+1$. %% Let $c := c_{r+1}$ be the color exactly in the
% %% middle of $v$.

% \begin{teo}\label{t:Caterpillars_f}
%   Let $X$ be a caterpillar with at least one end-point $x_0$. Let $P$ be the
%   underlying (possibly infinite) path starting at $x_0$ and let $S$ be
%   the word describing its sequence of colors. Then at least one of the
%   following statements is true:
%   \begin{enumerate}
%   \item $X$ is finite and symmetric.
%   \item $X$ is the STG of a polytope with boolean automorphism group.
%   \item $S$ is of the form $S =
%     wa_1w^{-1}bwa_2w^{-1}bwa_3w^{-1}b\ldots$, where $w=c_1c_2\ldots
%     c_r$ is a word on $\{0,1,\ldots,n-1\}, \; a_i = c_r\pm 1$ for all
%     $i$, and $(c_1,b) \in \{(1,0),(n-2,n-1)\}$. If $X$ is finite, $S$
%     must end right after an occurence of $w$ or $w^{-1}$. If $S$ ends
%     right after the $t$-th occurence of $w^{-1}$, then there exists
%     $i$ such that $a_i \neq a_{t+1-i}$. The inverse word $S^{-1}$,
%     must also have this same structure.
%   \end{enumerate}
% \end{teo}

 \begin{obs}
   If the second condition is the one holding, the actual STG of
   $X^\xi$ is the finite caterpillar with underlying word $w$.
 \end{obs}



% We could have used a smaller boolean group to get a polytope: namely
% one with one generator for each color. The voltage of each
% semi-edge would be the generator corresponding to its color. This
% would not affect the proof of Proposition~\ref{p:Caterpillars1} (in
% fact it would have make it easier), but on
% Theorem~\ref{t:Caterpillars} We have used strongly the fact that some
% semi-edges of the same color have different voltages. It is a
% conjecture of the author of this thesis that if we use the smaller
% boolean group we would always get a polytope with extra symmetry,
% probably a regular one. OBSOBS CONJETURA LOCA, PENSAR MÁS

==> Caterpillars2.tex <==

\section{Example: Caterpillars}\label{s:Caterpillars}

If one wants to build polytopes from premaniplexes in the way we have described in this paper, it is natural to start with infinite families of premaniplexes. 
One could, of course, then start with premaniplexes with a fixed number $k$ of vertices. For example, one may want to construct 2-orbit polytopes (see \cite{IsaEgon2orbit}).
If, on the other hand, we do not want to limit the number of vertices of the premaniplexes in the family a first step could be to consider trees. However, since semi-edges are considered as cycles, there are no premaniplexes of rank $n\geq 3$ whose underlying graph (without colors) is a tree. Thus, we study the closest thing to them: premaniplexes that are trees with an unlimited number of semi-edges.
Hence, we define a {\em caterpillar} as a premaniplex in which every cycle  %contains at least one 
is a semi-edge.
In other words, a caterpillar is a premaniplex $X$ with a
unique spanning tree. 

In particular, a
caterpillar does not have pairs of parallel links (edges joining different vertices). If there are three
links  incident to one vertex, at
least two of them must have colors differing by more than 1, which
would imply that there is a 4-cycle. This implies that caterpillars
consist in fact of a single path $W$ (which we will call {\em the
  underlying path of $X$}) and lots of semi-edges. Of course, the
colors of two consecutive edges on the path must differ by exactly
one, otherwise there would be a 4-cycle.
We note here that the term {\em caterpillar} has been used in the graph theory literature for a very similar but slightly different concept.


Throughout this section, unless otherwise stated, $X$ will denote a finite caterpillar (that is, one with a finite number of vertices) with underlying path $W$, and its vertices will be labeled by $x_0, x_1,\ldots, x_k$, ordered as they are visited by $W$.
Furthermore, we denote by $(x_i,j)$ the dart of color $j$ at $x_i$ and by $c_i$ the color of the link connecting $x_{i-1}$ and $x_i$.


\begin{figure}
  \begin{center}
    \includegraphics[width=5cm]{caterpillar.pdf}
    \caption{\label{f:caterpillar} A finite caterpillar.}
  \end{center}
\end{figure}



\input{CoversCaterpillars}

\subsection{Caterpillars as STG of polytopes}

Given a caterpillar $X$, we want to assign voltages to the semi-edges of $X$ in order to get the flag graph of a polytope as the derived maniplex.
To this end, we note that in caterpillars the conditions of Theorems~\ref{t:IntProp-w} and~\ref{t:IntProp} can be simplified, as stated in the following lemma:

\begin{lema}\label{l:IntPropCat}
  Let $X$ be a caterpillar and let $\xi:\Pi(X)\to\Gamma$ be a voltage
  assignment such that all the darts in the underlying path of $X$
  have trivial voltage. Then the following statements are equivalent.
  \begin{enumerate}
  \item $X^\xi$ is polytopal.
  \item For every vertex $x$ in $X$ and all sets
    $I,J\subset\{0,1,\ldots,n-1\}$ the equation
    \[
      \xi(\Pi_I^x(X))\cap \xi(\Pi_J^x(X)) = \xi(\Pi^x_{I\cap J}(X))
    \]
    holds.
    \item For every vertex $x$ in $X$ and all
      $k,m\in\{0,1,\ldots,n-1\}$ the equation
      \[
        \xi(\Pi_{[0,m]}^x(X))\cap \xi(\Pi_{[k,n-1]}^x(X)) =
        \xi(\Pi^x_{[k,m]}(X))
      \]
      holds.
  \end{enumerate}
\end{lema}

\begin{dem}
  To prove this we have to see that for every set of colors
  $I\subset \{0,1,\ldots, n-1\}$ the set $\xi(\Pi^{x,y}_I(X))$ is either
  $\xi(\Pi^x_I(X))$ or empty, depending on whether or not the segment of
  $W$ that goes from $x$ to $y$ (which we will denote $[x,y]$) uses  only colors in $I$. In fact if $[x,y]$ uses only colors in
  $I$ then
  \[
    \xi(\Pi^{x,y}_I(X)) = \xi(\Pi^x_I(X) [x,y]) =
    \xi([x,y])\xi(\Pi^x_I(X)) = 1\cdot \xi(\Pi^x_I(X)) =
    \xi(\Pi^x_I(X)).
  \]

  Note also that $\xi(\Pi^{x,y}_I(X)) \cap \xi(\Pi^{x,y}_J(X))$
  is empty if and only if one of the factors is empty. These
  observations together with Theorems~\ref{t:IntProp-w} prove the
  equivalence between conditions 1 and 2, and with
  Theorem~\ref{t:IntProp} we prove the equivalence between conditions
  1 and 3, thus proving the lemma. \qed

\end{dem}

Recall that a {\em Boolean group} (or an {\em elementary Abelian $2$-group}) is a group in which every
non-trivial element has order exactly 2. Thus, all Boolean
groups are Abelian, and finitely generated Boolean groups are
isomorphic to a direct product of cyclic groups of order 2.


\begin{prop}\label{p:Caterpillars1}
  Every caterpillar is the quotient of the flag graph of a polytope
  by a Boolean group.
\end{prop}

\begin{dem}
  Let $X$ be a caterpillar. 
  We shall find a Boolean group $B$ and a voltage assignment $\xi:\Pi(X)\to B$ such that $X^\xi$ is polytopal in the following way.

  First assign trivial voltage to all links of $W$ and a different independent voltage to each semi-edge incident to $x_0$. 
  We shall give voltage assignments to the semi-edges $(x_i,j)$, recursively on $i$.
  If $|j-c_i|>1$ we assign the same voltage to $(x_i,j)$ as we did to $(x_{i-1},j)$.
  On the ohter hand, if $|j-c_i|=1$, we assign a new element as the voltage $(x_i,j)$ independent from all the voltages of previous darts.
  
  \if
  To do so, define $\delta_i:=c_{i+1}-c_i$ for $i=1,\ldots,k-1$, and note that $\delta_i \in  \{-1,1\}$%, as otherwise $X$ would have a $4$-cycle without semi-edges
  .
  There are two cases to consider to assign the voltage of $(x_i,j)$, for $i<k$:
  \begin{itemize}
      \item $j\neq c_i-\delta_i$. 
      In this case $(x_{i-1},j)$ is a semi-edge because $j$ differs from $c_i$ in more than $1$, and the links incident to $x_{i-1}$ have colors $c_i$ and  $c_{i-1}=c_i+\delta_{i-1}$.
      This implies that the path $(x_{i-1},c_i)(x_i,j)(x_i,c_i)(x_{i-1},j)$ must have trivial voltage.
      Hence, we assign to the semi-edge $(x_i,j)$ the same voltage as the one that $(x_{i-1},j)$ has.
      \item $j= c_i-\delta_i$. In this case, we assign a new generator of a Boolean group as the voltage of  $(x_i,j)$.
  \end{itemize}
  Finally, since $\delta_k$ is undefined, we assign new
  generators as the voltages of the darts $(x_k,c_k+1)$ and
  $(x_k,c_k-1)$
  (if they exist) and  for the other semi-edges on $x_k$ copy the
  voltage of the semi-edge of the same color on $x_{k-1}$. 
  \fi
  
  Let us call
  the resulting voltage group $B$ and denote this
  voltage assignment by $\xi$. By Lemma~\ref{l:VoltMani}, $X^\xi$ is a maniplex.

  Note further that $\xi$ satisfies that if $i\in
  \{1,2,\ldots,k\}$; $r,s\in \{0,1,\ldots,n-1\}$ and $(x_{i-1},r)$ and
  $(x_i,s)$ are semi-edges, then $\xi(x_i,s) = \xi(x_{i-1},r)$ if and
  only if $r=s$ and $|r-c_i|\neq 1$. It also satisfies that if
  $i<\ell<j$ and $(x_i,r)$ and $(x_j,r)$ are semi-edges such that
  $\xi(x_i,r) = \xi(x_j,r) = \gamma$, then $(x_\ell,r)$ is also a
  semi-edge and $\xi(x_\ell,r) = \gamma$.

  We claim that the second statement of Lemma~\ref{l:IntPropCat} is satisfied, and
  hence, $X^\xi$ is the flag graph of a polytope.
To show that this is the case, start by noticing that $\xi(\Pi^x_I)$ is the group generated by the voltages of the semi-edges on the component $X_I(x)$.

  Given $I, J \subseteq \{0,1, \dots, n-1\}$, suppose that for some vertex $x$ there is a semi-edge $e$ in
  $X_I(x)$ and a semi-edge $e'$ in $X_J(x)$ with
  $\xi(e) = \xi(e') = \gamma$ for some $\gamma \in \Gamma$. If $e=e'$
  then $e \in X_{I\cap J}(x)$. If $e\neq e'$, then $e=(x_i,r)$ and $e'=(x_j,r)$ for some $i,j\in \{0,\ldots,k-1\}$ and $r \in \{0,\ldots,n-1\}$; in particular
  $r\in I\cap J$.
  If $x\in [x_i,x_j]$ then, as previously observed,
  $\xi(x,r) = \gamma$ (see Figure~\ref{f:IntPropCat_caso1}) and since
  $(x,r) \in X_{I \cap J}(x)$ this means $\gamma$ is a generator of
  $\xi(\Pi^x_{I\cap J})$. If $x\notin [x_i, x_j]$ consider without
  loss of generality that $x_i$ is further away from $x$ than $x_j$,
  in other words, that $x_j \in [x_i,x]$ (see Figure~\ref{f:IntPropCat_caso2}). Then
  $[x_i,x]$ uses only colors in $I$ and $[x_j,x] \subset [x_i,x]$ uses
  only colors in $J$. Then since $[x_j,x] \subset [x_i,x]$ we know
  that $[x_j,x]$ uses only colors in $I \cap J$, meaning that
  $e' \in X_{I \cap J}(x)$ and since its voltage is $\gamma$, this
  shows that $\gamma$ is always a generator of
  $\xi(\Pi^x_{I \cap J})$. Therefore, we have shown that if $\gamma$ is a
  generator of both $\xi(\Pi^x_I(X))$ and $\xi(\Pi^x_J(X))$, then it
  is also a generator of $\xi(\Pi^x_{I \cap J}(X))$.

  Now let $\sigma\in \xi(\Pi^x_I(X)) \cap \xi(\Pi^x_J(X))$ be
  arbitrary. Since the group $B$ is Boolean, $\sigma$ may be written
  as $\sigma=\gamma_1\gamma_2\ldots \gamma_s$ where the elements
  $\gamma_1, \gamma_2,\ldots, \gamma_s$ are different generators of
  $B$, and this decomposition is unique up to reordering of the
  factors. Since $\sigma \in \xi(\Pi^x_I(X))$, and because the voltage
  of a semi-edge is always a generator, each $\gamma_i$ is also in
  $\xi(\Pi^x_I(X))$, and since $\sigma \in \xi(\Pi^x_J(X))$ each
  $\gamma_i$ is also in $\xi(\Pi^x_J(X))$. But, this implies that each $\gamma_i$ is in
  $\xi(\Pi^x_{I\cap J}(X))$, implying that
  $\sigma \in \xi(\Pi^x_{I\cap J}(X))$. Therefore,
  $\xi(\Pi^x_I) \cap \xi(\Pi^x_J) = \xi(\Pi^x_{I \cap J})$. \qed
\end{dem}

\begin{figure}%[h]
  \centering
  \includegraphics[width=7.5cm]{IntPropCat_caso1.pdf}
  \caption{If $x\in[x_i,x_j]$ then $(x,r)$ has voltage
    $\gamma\in \xi(\Pi^x_{I\cap J}(X))$.}
  \label{f:IntPropCat_caso1}
\end{figure}

\begin{figure}%[h]
  \centering
  \includegraphics[width=7.5cm]{IntPropCat_caso2.pdf}
  \caption{If $x_j\in[x_i,x]$ then $e'=(x_j,r)$ is in
    $X_{I\cap J}(x)$ and has voltage $\gamma$.}
  \label{f:IntPropCat_caso2}
\end{figure}

The flag graphs of the polytopes constructed in the proof of \cref{p:Caterpillars1} have some 4-cycles consisting of edges of consecutive colors. For this reason we say that they are \emph{degenerated}.

Proposition~\ref{p:Caterpillars1} is still true for infinite
caterpillars. Even if our algorithmic way of assigning voltages may
not be doable, the voltage assignment is still well defined as a
quotient of the Boolean group with one generator assigned to each
semi-edge.

Note that Proposition~\ref{p:Caterpillars1} says that every caterpillar $X$ is a symmetry type graph of a polytope $\p$ with respect to some group $B\leq \Aut(\p)$. 
However, $X$ is not necessarily the symmetry type graph of $\p$ with respect to the full automorphism group.
That is, $X^\xi$ might have ``extra'' symmetry.
Thus, we would want to investigate what could be the
symmetry type of $X^\xi$ with respect to its full automorphism group.

Let $X$ be a finite caterpillar and let $\xi:\Pi(X)\to B$ be the
voltage assignment constructed in the proof of
Proposition~\ref{p:Caterpillars1}. If $X$ is symmetric, its
non-trivial symmetry induces an automorphism of $B$ which is just a
reordering of the generators, moreover, if the generators are given
the natural order, it induces the reverse order on the
generators. Using~\cite[Theorem 7.1]{Voltajes}, we get that this symmetry induces a symmetry of the derived maniplex, so in this case the original caterpillar is
not the symmetry type of the derived polytope. But we will see in
Theorem~\ref{t:Caterpillars} that if $X$ is not symmetric, we can
almost be certain that the caterpillar is in fact the symmetry type
graph of the derived polytope by its full automorphism group. In this
case, by ``almost'' we mean that if this is not the case, the
caterpillar must have a very specific structure.

\begin{teo}\label{t:Caterpillars}
  Let $X$ be a finite caterpillar of length $k$ and rank $n$. Let
  $S=c_1c_2\ldots c_k$ be the underlying word of $X$. Then at
  least one of the following statements is true:
  \begin{enumerate}
  \item $X$ is symmetric.
  \item $X$ is the STG of a polytope with a Boolean automorphism
    group.
  \item $c_1$ is in $\{1,n-2\}$ and there exist $r\in
    \{1,2,\ldots,k-1\}$, and
    $a_1,a_2,\ldots,a_t \in \{0,1,\ldots,n-1\}$ where
    $t=(k+1)/(2r+2)$, such that
    $S=wa_1w^{-1}bwa_2w^{-1}b\ldots bwa_tw^{-1}$ where $w=c_1c_2\ldots
    c_r$ and %$(c_1,b) \in \{(1,0),(n-2,n-1)\}$.
    $b=0$ if $c_1=1$ and $b=n-1$ if $c_1=n-2$.
  \item There exist $r\in \{1,2,\ldots,k-1\}$ and
    $a,b \in \{0,n-1\}$ such that
    \[
      S=waw^{-1}bwaw^{-1}b\ldots bwaw^{-1}bw,
    \]
    where $w=c_1c_2\ldots c_r$. Also
    $(c_1,b), (c_r,a) \in \{(1,0),(n-2,n-1)\}$.
  \end{enumerate}
\end{teo}
\begin{dem}
  Suppose that $X$ is not symmetric and that it is not the STG of a
  polytope with a Boolean automorphism group. %% We want to prove that
  %% $(c_1,c_2)\in \{(1,0),(n-2,n-1)\}$ (for the pair $(c_k,c_{k-1})$ we
  %% would have a completely analogous proof).

  Consider the voltage
  assignment $\xi:\Pi(X)\to B$ previously discussed. We say that
  two vertices $x$ and $y$ of $X$ are equivalent ($x\sim y$) if there
  exist (or equivalently, for all) $\sigma,\tau \in B$ such that
  the flags $(x,\sigma)$ and $(y,\tau)$ of $X^\xi$ are in the same
  orbit under the action of the automorphism group of $X^\xi$. Then
  $\sim$ is an equivalence relation preserved by $i$-adjacency,
  that is $x\sim y \Rightarrow x^i\sim y^i$.
  Moreover,
  the natural function $h:X\to X/\sim$ is a premaniplex
  homomorphism, so by Proposition~\ref{p:CubsCat} there
  exists some $r$ such that $S$ can be written
  as $wa_1w^{-1}b_1wa_2w^{-1}b_2\ldots $ ending after an occurrence of
  either $w$ or $w^{-1}$, where $w=c_1c_2\ldots c_r$, $a_i\in
  \{c_r+1,c_r-1\}$ and $b_i\in \{c_1+1,c_1-1\}$ (see
  Figure~\ref{f:FoldedCat}).
  In fact, $X/\sim$ is isomorphic to the actual symmetry type graph of $X^\xi$ (mapping the orbit of $(x,\gamma)$ to the equivalence class of $x$ is an isomorphism).

  %AHORITA VEMOS QUE ONDA CON ESTO  The proof that there is a palindrome
  %segment $[x_i,x_k]$ is completely analogous.

  Note that since $X$
  is not symmetric nor the STG of $X^\xi$ with respect to $B$, at
  least $b_1$ exists. Let $j\in\{0,1\ldots,k-1\}$ be a number such
  that the segment $[x_0,x_{j+1}]$ has the underlying word
  $wa_1w^{-1}b_1wa_2w^-1b_2\ldots w^{-1}b_i$ for some $i$. We know in
  particular that $b_i$ differs from $c_1$ in exactly 1. We want to
  prove that $(c_1,b_i) \in \{(1,0),(n-2,n-1)\}$. We will assume this
  is not the case and arrive to a contradiction.

  Let $q$ be the {\em other} color that differs from
  $b_i$ in exactly 1 (that is $q = 2b_i - c_1$). Since $(c_1,b_i) \neq
  (1,0),(n-2,n-1)$ we know that $q\in \{0,1,\ldots,n-1\}$, and thus is
  the color of some edges of $X$. So there
  are semi-edges $e,e'$ incident
  to $x_0$ of colors $q$ and $b_i$ respectively. Let
  $\alpha:=\xi(e)$ and $\beta:=\xi(e')$. The voltage of the closed
  path $ee'ee'$ is $(\beta\alpha)^2 = 1$ because $B$ is Boolean. This
  means that its lift, (the path of length 4 that starts at $(x,1)$ in
  $X^\xi$ and  alternates colors between $q$ and $b_i$) must be closed.

  %Now let us check two cases:
  %
  % \noindent {\bf Case 1: The dart $(x_{j+1},r)$ is a link.} In
  % this case the path in $X$ of length 4 that alternates colors between
  % $r$ and $b_i$ and starts at  $x_j$ is not closed (after three steps
  % it is at $x_{j+2}$), so its lift cannot  be closed either.

  % \begin{figure}[h]
  %   \begin{center}
  %     \includegraphics[width=7cm]{CatCaso1.pdf}
  %     \caption{\label{f:CatCaso1} Case 1.}
  %   \end{center}
  % \end{figure}

  % \noindent {\bf Case 1: The dart $(x_{j+1},r)$ is a semi-edge.}
  By Theorem~\ref{p:CubsCat}, we know that $c_{j+1} = c_1 \neq q$, so
  we know that the darts $(x_{j+1},q)$ and $(x_j,q)$ are
  semi-edges. Let $\kappa := \xi(x_j,q)$ and
  $\lambda = \xi(x_{j+1},q)$. The path of length 4 that alternates
  colors between $r$ and $b_i$ and starts at $x_j$ is closed, and its
  voltage is $\lambda\kappa$. Note that since $|q-b_i|=1$ the
  definition of $\xi$ tells us that
  $\xi(x_j,q) \neq \xi(x_{j+1},q)$, that is $\lambda \neq \kappa$,
  which implies $\lambda\kappa \neq 1$. This means that the path of
  length 4 in $X^\xi$ starting at $(x_j,1)$ and alternating colors
  between $r$ and $b_i$ is not closed (it ends at
  $(x_j,\lambda\kappa)$).

    \begin{figure}%[h]
    \begin{center}
      \includegraphics[width=7cm]{CatCaso2.pdf}
      \caption{\label{f:CatCaso2} %Case2
        The voltage of the path that alternates colors between $q$ and
        $b_i$ starting at $x_j$ is $\lambda\kappa\neq 1$.}
    \end{center}
  \end{figure}

  % In both cases w
  We see that the path of length 4 in $X^\xi$ starting at $(x_j,1)$
  and alternating colors between $r$ and $c_{j+1}$ is not closed, but
  the one starting at $(x_0,1)$ is. This contradicts the fact that
  $(x_j,1)$ and $(x_0,1)$ are on the same orbit. The contradiction
  comes from the fact that there are edges of color
  $q = 2b_i -c_1 \in \{0,1,\ldots,n-1\}$, so to avoid this we must
  have that $(c_1,b_i) \in \{(1,0),(n-2,n-1)\}$. Since $c_1$ is fixed,
  every $b_i$ must be the same.

  % , so we have finished the proof.
  %The proof that $(c_k,c_i)\in\{(1,0),(n-2,n-1)\}$ is completely
  %analogous. \qed

  If the underlying word of $X$ ends after an occurrence of $w$ we
  may look at $X$ in the other direction. Then the previous result
  tells us that every $a_i$ is equal to some $a$ and that $(c_r,a)\in
  \{(1,0), (n-2,n-1)\}$. \qed
\end{dem}

 \begin{obs}
   If the third or fourth condition is the one holding in
   Theorem~\ref{t:Caterpillars}, the actual STG of $X^\xi$ might be the
   finite caterpillar with underlying word $w$.
 \end{obs}

By doing exactly the same proof, we obtain the following analogous
result for infinite caterpillars with one end-point (this would
  look like a ray or half-straight line):

\begin{teo}\label{t:Caterpillars1end}
  Let $X$ be an infinite caterpillar with one end-point. Let $S$ be
  the sequence of colors of the underlying path of $X$ starting at its
  end-point. Then one of the following statements is true:
  \begin{enumerate}
  \item $X$ is the STG of a polytope with a Boolean automorphism
    group.
  \item There exist some number $r$ and colors
    $b,a_1,a_2,\ldots \in \{0,1,\ldots,n-1\}$ such that
    $S=wa_1w^{-1}bwa_2w^{-1}bwa_3w^{-1}\ldots$ where $w=c_1c_2\ldots
    c_r$ and $(c_1,b) \in \{(1,0),(n-2,n-1)\}$.
  \end{enumerate}
\end{teo}

% OBSOBS GUSANOS SIN FINALES?

% Let us examine more deeply the structure of a caterpillar that is
% neigther symmetric nor the STG of a polytope with boolean automorphism
% group.

% Let $X$ be a caterpillar with at least one end-point (finite or infinite) and
% suppose that it is neigther symmetric or the STG of a polytope with a
% boolean group. According to Theorems~\ref{t:Caterpillars}
% and~\ref{t:Caterpillars1end}, the underlying path of $X$  must start
% with a
% palindrome segment $[x_0,x_j]$. Let $v = c_1c_2\ldots c_j$ be the
% palindrome word describing the colors of this segment. Since $v$ is a
% palindrome and it may not have the same color twice in a row, $j$ must
% be odd, say $j=2r+1$. %% Let $c := c_{r+1}$ be the color exactly in the
% %% middle of $v$.

% \begin{teo}\label{t:Caterpillars_f}
%   Let $X$ be a caterpillar with at least one end-point $x_0$. Let $P$ be the
%   underlying (possibly infinite) path starting at $x_0$ and let $S$ be
%   the word describing its sequence of colors. Then at least one of the
%   following statements is true:
%   \begin{enumerate}
%   \item $X$ is finite and symmetric.
%   \item $X$ is the STG of a polytope with boolean automorphism group.
%   \item $S$ is of the form $S =
%     wa_1w^{-1}bwa_2w^{-1}bwa_3w^{-1}b\ldots$, where $w=c_1c_2\ldots
%     c_r$ is a word on $\{0,1,\ldots,n-1\}, \; a_i = c_r\pm 1$ for all
%     $i$, and $(c_1,b) \in \{(1,0),(n-2,n-1)\}$. If $X$ is finite, $S$
%     must end right after an occurence of $w$ or $w^{-1}$. If $S$ ends
%     right after the $t$-th occurence of $w^{-1}$, then there exists
%     $i$ such that $a_i \neq a_{t+1-i}$. The inverse word $S^{-1}$,
%     must also have this same structure.
%   \end{enumerate}
% \end{teo}

 \begin{obs}
   If the second condition is the one holding, the actual STG of
   $X^\xi$ might be the finite caterpillar with underlying word $w$.
 \end{obs}

If $k\geq 3$, it is easy to construct a caterpillar of length $k-1$ (that is, with $k$ vertices and $k-1$ links) that does not satisfy properties $(1)$, $(3)$ and $(4)$ (simply let $c_1=0$ and then avoid the color $0$ for every other $c_i$).
Hence, we get the following corollary:

\begin{coro}\label{coro:k_orbit_exists}
    For every $n,k\geq 3$, there is an abstract $n$-polytope with Boolean automorphism group that has $k$ flag orbits.
\end{coro}


% We could have used a smaller boolean group to get a polytope: namely
% one with one generator for each color. The voltage of each
% semi-edge would be the generator corresponding to its color. This
% would not affect the proof of Proposition~\ref{p:Caterpillars1} (in
% fact it would have make it easier), but on
% Theorem~\ref{t:Caterpillars} We have used strongly the fact that some
% semi-edges of the same color have different voltages. It is a
% conjecture of the author of this thesis that if we use the smaller
% boolean group we would always get a polytope with extra symmetry,
% probably a regular one. OBSOBS CONJETURA LOCA, PENSAR MÁS

==> CoversCaterpillars.tex <==
\subsection{Caterpillar coverings}

We want to construct polytopes from caterpillars. 
As often when constructing maniplexes and polytopes via voltage assignments from a premaniplex $X$, the derived maniplex might not have $X$ as the symmetry type graph with respect to the full automorphism group.
However, the actual symmetry type graph is a quotient of $X$. 
For this reason, in this section we study quotients of caterpillars.
%The results of this section do not involve voltage assignments, but shall be use in the following section.


Given a caterpillar, let us call an {\em endpoint} a vertex incident to just one link (that is, an endpoint of the underlying path). 
Note that a caterpillar is finite if and only if it has exactly
two endpoints. 
Every symmetry of the caterpillar must map endpoints to endpoints. If a caterpillar is finite there is at most one non-trivial symmetry and its action on the vertices $x_0,x_1,\ldots,x_k$ is given by $x_j\mapsto x_{k-j}$. 
We call a finite caterpillar {\em symmetric} if it has a non-trivial symmetry.

A {\em word} $w$ in $\{0,1,\ldots,n-1\}$ is simply a finite sequence $w=a_1a_2\ldots a_t$, with $a_i\in \{0,1,\ldots,n-1\}$ for each $i=1,2,\ldots,t$. 
The {\em inverse} of a word $w$ is the word $w^{-1}$ that has the same colors as $w$ but written in reverse order. 
That is, if $w=a_1a_2\ldots a_t$ then $w^{-1} = a_ta_{t-1}\ldots a_1$. A word is said to be {\em reduced} if it has no occurrence of the same color twice in a row; in other words, $w=a_1a_2\ldots a_t$ is reduced if and only if $a_{i+1}\neq a_i$ for all $i=1,2,\ldots,t-1$. 
We shall work with reduced words from now on. 
A word $w=a_1a_2\ldots a_t$ is a {\em palindrome} if  $a_i = a_{t+1-i}$ for all $i\in \{1,2,\ldots,t\}$. 
A palindrome of even length can
be written as $vv^{-1}$ for some word $v$ and cannot be
reduced. 
A palindrome of odd length can always be written as
$w=vav^{-1}$ for some color $a$ and some word $v$.

Given a segment $[x,y]$ in a caterpillar, its {\em underlying word} is
the word $w$ consisting of the colors of the links in the path that
goes from $x$ to $y$. When we speak of the {\em underlying word} of a
caterpillar $X$ we are referring to the underlying word of its
underlying path in a fixed orientation.
Hence, we say that a segment $[x,y]$ is a {\em palindrome} if its underlying word
$v$ is a palindrome.

\begin{prop}\label{p:CubsCat}
  Let $X$ be a finite caterpillar and let $Y$ be a premaniplex not
  isomorphic to $X$ %with at least 2 vertices and
  such that there is a premaniplex homomorphism %(or covering)
  $h:X\to Y$. Then $Y$ is a caterpillar. Moreover, if $Y$ has at least
  2 vertices and $S=c_1c_2\ldots c_k$ is the underlying word of $X$,
  then there is some $r<k$ such that $w=c_1c_2\ldots c_r$ is the
  underlying word of $Y$ and one of the following statements is true:
  \begin{enumerate}
  \item There exist colors $a_1,a_2,\ldots,a_t \in \{c_r+1,c_r-1\}$ and
    $b_1,b_2\ldots,b_{t-1} \in \{c_1+1,c_1-1\}$ such that
    $S=wa_1w^{-1}b_1wa_2w^{-1}b_2\ldots b_{t-1}wa_tw^{-1}$.
  \item There exist colors $a_1,a_2,\ldots,a_t\in \{c_r+1,c_r-1\}$ and
    $b_1,b_2\ldots,b_t \in \{c_1+1,c_1-1\}$ such that
    $S=wa_1w^{-1}b_1wa_2w^{-1}b_2\ldots b_{t-1}wa_tw^{-1}b_tw$.
  \end{enumerate}

  In any case, if $i \equiv j \md 2r+2$ then $h(x_i) = h(x_j)$. Also
  if $i \equiv -j-1 \md 2r+2$ % and $\floor{\frac{i}{r+1}} \not\equiv
  % \floor{\frac{j}{r+1}} \md 2$
  then $h(x_i) = h(x_j)$% (here
  % $\floor{x}$ denotes the integer part of $x$)
  .
\end{prop}

Before proving Proposition~\ref{p:CubsCat} let us remark that it
simply means that the quotients of a caterpillar $X$ are those
caterpillars $Y$ such that $X$ can be ``folded'' into $Y$. We
illustrate this concept in Figure~\ref{f:FoldedCat}: the semi-edges
are not drawn and the names of the vertices have been omitted, but the
idea is that $X$ must be ``folded'' into ``layers'' of $r+1$ vertices
and then each vertex will be projected to the vertex on $Y$ in the
same horizontal coordinate. The layer $\ell$ consists of the vertices
$x_i$ where $\floor{\frac{i}{r+1}}=\ell$ ($\floor{x}$ denotes the
integer part of $x$). Even layers go from left to right, while odd
layers go from right to left, hence the underlying word of even layers
is $w=c_1c_2\ldots c_r$ while the underlying word of odd layers is
$w^{-1}=c_rc_{r-1}\ldots c_1$.

\begin{figure}%[h!]
  \centering
  \begin{subfigure}[t]{0.45\linewidth}
    \includegraphics[width=6cm]{FoldCat1.pdf}
    \caption{Case 1}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.45\linewidth}
    \includegraphics[width=6cm]{FoldCat2.pdf}
    \caption{Case 2}
  \end{subfigure}
  \caption{The caterpillar $X$ covers the caterpillar $Y$ if and only
    if it ``folds'' into it.}
  \label{f:FoldedCat}
\end{figure}

Now let us proceed with the proof.

\begin{dem} {\bf of Proposition~\ref{p:CubsCat}}
  Let us consider the equivalence relation $\sim_h$ on $X$ given by  $x\sim_hy$ if and only if $h(x)=h(y)$. 
  Recall that by the definition of a premaniplex homomorphism $x\sim_h y$ implies that $x^m\sim_h y^m$ for every monodromy $m$. 
  Therefore $Y$ is isomorphic to $X/\sim_h$.

  We already know that all premaniplex homomorphisms are surjective
  (see Section~\ref{sec:Polytopes-and-maniplexes}). By hypothesis $h$ is not an isomorphism,
  which implies it cannot be injective. Let $x$ and $y$ be two
  different vertices on $X$ such that $x\sim_h y$. Let
  $x_0,x_1,\ldots, x_k$ be the sequence of vertices in the underlying
  path of $X$. There is a monodromy $m$ such that $x^m=x_0$, and so
  $x_0\sim_h y^m$ and $y^m$ is different than $x_0$. Now let $q$ be
  the minimum positive number such that $x_q\sim_h x_0$. We know that
  $q$ exists because $x_0\sim_h y^m$. Note that if
  $q=1$ we would have that $x_0^i\sim_h x_0$ for all $i$, which would
  imply that the same is true for $x_1$ and in turn also for
  $x_2=x_1^{c_2}$ and so on. This would mean that all the vertices of
  $X$ are equivalent, meaning that $Y$ has only one vertex and the
  proposition follows. So we may assume that $q>1$.

  We know that $x_{q-1} = x_q^{c_q}$ is equivalent $x_0^{c_q}$. If
  $c_q \neq c_1$, we would have that $x_0^{c_q}=x_0$. This would imply
  that $x_{q-1}$ is equivalent to $x_0$, contradicting the minimality
  of $q$. So we have proven that $c_q = c_1$.

  Now note that if for some $\ell$ we have that $x_\ell\sim_h x_1$, then
  $x_\ell^{c_1}\sim_h x_1^{c_1}=x_0$. In particular this tells us that
  for $\ell<q-1$, $x_\ell$ cannot be equivalent to $x_1$. Now we can
  use the same argument we used to prove that $c_q=c_1$ to prove that
  $c_{q-1}=c_2$. Analogously we can prove that
  $c_3 = c_{q-2}, c_4=c_{q-3}$ and so on. In other words, $[x_0,x_q]$
  is a palindrome. Since for all $i$, $c_i$ and $c_{i+1}$ are
  different, then $q$ is odd, say $q=2r+1$. Let $v$ be the underlying
  word of the segment $[x_0,x_q]$. Then $v$ may be written as
  $v=wc_{r+1}w^{-1}$ for some word $w = c_1c_2\ldots c_r$. Let us call
  $a_1:=c_{r+1}$ and note that $a_1\in \{c_r+1,c_r-1\}$.

  For all $i=0,1,\ldots, k$, let us denote by $\widehat{i}$ the
  residue of dividing $i$ by $2r+2$. We will prove by induction on $i$
  that $x_i\sim_h x_{\widehat{i}}$ for all $i=0,1,\ldots, k$ and that
  $c_{i} = c_{\widehat{i}}$ when $i$ is not divisible by $r+1$,
  $c_i \in \{c_1+1,c_1-1\}$ if $i$ is an even multiple of $r+1$ and
  $c_i= \{c_r+1,c_r-1\}$ when $i$ is an odd multiple of $r+1$.

  Let our induction hypothesis be that $x_{\ell}\sim_h
  x_{\widehat{\ell}}$ for all $\ell<i$, and that
  $c_{\ell} = c_{\widehat{\ell}}$ if $\ell$ is not divisible by $r+1$.
  % This will prove
  % that  if $i\equiv j \md
  % 2r+2$ then $x_i\sim_h x_j$. Moreover, if $i \equiv -j-1 \md 2r+2$,
  % then $\widehat{i}= 2r+1 -\widehat{j}$. Note that since $v$ is
  % a palindrome, then $x_\ell\sim_h x_{2r+1-\ell}$ for
  % $\ell=0,1,\ldots,2r+1$, in particular $x_{\widehat{j}} \sim_h
  % x_{2r+1-\widehat{j}} = x_{\widehat{i}}$
  % and this
  % implies that if $i \equiv -j-1 \md 2r+2$ and
  % $\floor{\frac{i}{r+1}} \not\equiv \floor{\frac{j}{r+1}} \md 2$ then
  % $x_i\sim_h x_j$.

  % We will also
  % assume that $c_{i-1} = c_{\widehat{i-1}}$  but {\bf only}
  % when $\ell$ is not divisible by $r+1$. We will prove that
  % $c_i=c_{\,\widehat{i}}$ when $i$ is not divisible by $r+1$, that
  %  This would prove that $X$ has the structure suggested in the
  % statement of the theorem.

  Let us start with the case when $i\equiv 0 \md 2r+2$. In this case
  we want to prove that $x_i \sim_h x_{\widehat{i}}$ and that
  $c_i\in \{c_1+1,c_1-1\}$. By our induction hypothesis we know that
  $x_{i-1}\sim_hx_{2r+1} \sim_h x_0$ and $c_{i-1}=c_{2r+1}=c_1$. In
  particular $c_i\in \{c_1+1,c_1-1\}$.  This implies that
  $x_i=x_{i-1}^{c_i}\sim_h x_0^{c_i}=x_0=x_{\,\widehat{i}}$ (since
  $c_i\neq c_1$). Thus $i$ satisfies our claim.

  Now let us proceed with the case when $i$ is an odd multiple of
  $r+1$, that is $\widehat{i} = r+1$. In this case we want to prove
  that $x_i \sim_h x_{\widehat{i}}$ and that $c_i\in
  \{c_r+1,c_r-1\}$. Our induction hypothesis tells us that
  $x_{i-1}\sim_h x_r$ and that $c_{i-1}=c_r$. Hence
  $c_i \in \{c_r+1,c_r-1\}$. Note that one of the colors in
  $\{c_r+1,c_r-1\}$ is actually $c_{r+1}$, while the other is the
  color of a semi-edge incident to $x_r$. Since $x_{r+1}\sim_h x_r$ we
  have that
  $x_i=x_{i-1}^{c_i}\sim_h x_r^{c_i}\sim_h x_r\sim_h x_{r+1} =
  x_{\,\widehat{i}}$. Thus $i$ satisfies our claim.

  Finally let us prove our claim for the case when $i$ is not
  divisible by $r+1$. Our induction hypothesis tells us that
  $x_{i-1}\sim_h x_{\widehat{i-1}}$. Note that
  $\widehat{i} = \widehat{i-1}+1$. Since $i$ is not a multiple of
  $r+1$ we know that
  $x_{\,\widehat{i}}=x_{\widehat{i-1}}^{c_{\,\widehat{i}}}$ is not
  equivalent to $x_{\widehat{i-1}}$. This implies that
  $x_{i-1}^{c_{\,\widehat{i}}}$ is not equivalent to $x_{i-1}$, and
  since it is adjacent to $x_{i-1}$ it must be equal to either $x_i$
  or $x_{i-2}$. 
  \if
  If $i\equiv 1 \md r+1$, using our induction hypothesis we can see that $x_{i_2}\sim_h x_{i-1}$, so $x_{i-1}^{c_{\widehat{i}}}$ must be $x_i$, implying that $c_i=c_{\widehat{i}}$.
  \fi
  If $i\equiv 1 \md 2r+2$ then, by induction hypothesis,
  $x_{i-1}\sim_h x_0$, but recall that $x_0\sim_h x_{2r+1}=x_q$ by
  definition, and by induction hypothesis
  $x_{i-2}\sim_h x_{\widehat{i-2}} = x_{2r+1}$. This means that
  $x_{i-2}\sim_h x_{i-1}$, so $x_{i-1}^{c_{\,\widehat{i}}}$ must be
  $x_i$, implying that $ c_i=c_{\,\widehat{i}}$. 
  Similarly, if $i\equiv r+2\md 2r+2$, using our induction hypothesis we get that $x_{i-1}\sim_h x_{r+1}\sim_h x_r\sim_hx_{i-2}$, which implies that $x_{i-1}^{c_{\widehat{i}}}=x_i$ and again we get that $c_i=c_{\widehat{i}}$.
  If $i\not\equiv 1 \md r+1$ then our induction hypothesis tells us that
  $c_{i-1}=c_{\widehat{i-1}} \neq c_{\,\widehat{i}}$, and since
  $x_{i-2}=x_{i-1}^{c_{i-1}}=x_{i-1}^{c_{\widehat{i-1}}}$, the only
  possibility is that $x_{i-1}^{c_{\,\widehat{i}}} = x_i$, implying that
  $c_i=c_{\,\widehat{i}}$ and that $x_i\sim_h x_{\,\widehat{i}}$. Thus,
  $i$ satisfies our claim. Note that we have also proven that if $i$
  is not divisible by $r+1$ then $x_{i-1}$ cannot be an endpoint of
  $X$.

  We have proved that $x_i\sim_h x_{\,\widehat{i}}$ for all
  $i=0,1,\ldots, k$. This implies automatically that if $i\equiv j \md
  2r+2$ then $x_i\sim_h x_j$. Moreover, if $i\equiv -j-1 \md 2r+2$,
  then $\widehat{i} = 2r+1-\widehat{j}$. Now since $v$ is a
  palindrome, we know that $x_\ell \sim_h x_{2r+1-\ell}$ for all
  $\ell=0,1,\ldots, 2r+1$, in particular $x_{\,\widehat{i}} =
  x_{2r+1-\widehat{j}} \sim_h x_{\,\widehat{j}}$. This, together with the
  fact that $x_i \sim_h x_{\,\widehat{i}}$ and $x_j \sim_h
  x_{\,\widehat{j}}$, implies that $x_i \sim_h x_j$.

  We have already proved that $S=wa_1w^{-1}b_1wa_2w^{-1}\ldots$ and it
  ends after an occurrence of $w$ or $w^{-1}$. To end the proof note
  that since $h$ is surjective we already know exactly what
  premaniplex $Y$ is: It is a caterpillar with vertex sequence
  $h(x_0), h(x_1),\ldots, h(x_r)$. In fact, for $i=1,\ldots,r-1$ and
  $j=0,1,\ldots n-1$ we know that $h(x_i)$ is different from
  $h(x_i)^j=h(x_i^j)$ if and only if $j\in\{c_{i-1},c_i\}$; and if
  $i=0$ (resp. $r$) then $h(x_i)$ is different from $h(x_i)^j$ if and
  only if $j=c_1$ (resp. $c_r$). \qed


  % If $j=k$, that is, if $x_j$ is an endpoint of $X$, there is nothing
  % left to prove. Otherwise, let $b_1:=c_{j+1}$ and note that since
  % $c_j=c_1$ we have that $b_1\in \{c_1+1,c_1-1\}$. Note that since
  % $x_j\sim_h x_0$ and $(x_0,c_{j+1})$ is a semi-edge, we know that
  % $x_{j+1}=x_j^{c_{j+1}}\sim x_0^{c_{j+1}} = x_0$. On the other hand,
  % $x_1 = x_0^{c_1}\nsim_h x_0$ (unless $Y$ has only one vertex, in
  % which case there is nothing left to prove), which means that
  % $x_{j+1}^{c_1}\nsim_h x_{j+1}$. Then $c_{j+2} = c_1$ and
  % $x_{j+2}\sim_h x_1$. Repeating this argument we get that $c_{j+3} =
  % c_2$ and $x_{j+3}\sim x_2$; $c_{j+4} = c_3$ and $x_{j+4}\sim x_3$,
  % and so on; until we get to $c_{j+r+1} = c_r$ and $x_{j+r+1}\sim
  % x_r$. Now, since $x_{r+1} = x_r^{c_{r+1}}\sim x_r$, then
  % $x_{j+r+1}^{c_{r+1}}\sim x_{j+r+1}$, so this {\em might} be an end
  % point. Otherwise, it will be $a_2$-adjacent to $x_{j+r+2}$ for some
  % $a_2 \in \{c_r+1,c_r-1\}$ (since $c_{j+r+2} = c_r$).
  % % can also be $c_{r+1}$-adjacent to $x_{j+r+2}$,
  % % or even $(2c_r-c_{r+1})$-adjacent to $x_{j+r+2}$. These are the only
  % % options, since $c_{j+r+3}$ must differ from $c_{j+r+2} = c_r$ by
  % % exactly 1.
  % If we continue, we get to another vertex
  % ($x_{j+2r+2} = x_{2j+1}$) which is equivalent to $x_0$. %Now, since $X$
  % % is not symmetric this is not an end point, so
  % This vertex may be $b_2$-adjacent to $x_{2j+2}$ for some $b_2\in
  % \{c_1+1,c_1-1\}$ (since $c_{2j+2}=c_1$).

  % Proceeding with this logic we  get to the desired result. OBSOBS NO
  % SÉ CÓMO HACER QUE LA DEMOSTRACIÓN SE ENTIENDA BIEN Y A LA VEZ SEA
  % FORMAL. \qed
\end{dem}

%   see that if $S$ is the sequence of
%   colors of the path $P$ starting by the first endpoint, then $S$ must
%   be of the type $S = wa_1w^{-1}bwa_2w^{-1}bwa_3w^{-1}b\ldots$, where
%   $a_i = c_r\pm 1$ and $(c_1,b) \in \{(1,0),(n-2,n-1)\}$.

%   If $X$ is finite $S$ must end
% after an ocurrence of $w$ or $w^{-1}$. If $S$ ends after an
% occurrence of $w^{-1}$, say $S =
% wa_1w^{-1}bwa_2w^{-1}bwa_3w^{-1}b\ldots a_tw^{-1}$, then there must
% be at least one $i$ for which $a_i \neq a_{t+1-i}$, so that $S$ is not
% itself a palindrome (which would make the caterpillar symmetric). We
% should also consider that $S^{-1}$ must have the same structure, which
% is not automatic if $S$ ends after an occurence of $w$.

% In conclusion we get the following stronger theorem, which really
% restricts the structure of possible caterpillars that are not the STG
% of a polytope with a boolean automorphism group:

% \end{dem}

If we look closely at the proof of Proposition~\ref{p:CubsCat} we 
notice that we have not actually used the fact that $X$ is finite, but
only the fact that it has at least one endpoint. So the proposition
may be generalized as follows:

\begin{prop}\label{p:CubsCat1end}
    Let $X$ be a caterpillar with at least one endpoint and let $Y$ be a premaniplex
    such that there is a premaniplex homomorphism (or covering) $h:X\to
    Y$. Then $Y$ is a caterpillar. Moreover, if $Y$ has at least two vertices and $S=c_1c_2\ldots $ is
    the color sequence of $X$ starting at its endpoint, then there is some
    $r$ such that $w=c_1c_2\ldots c_r$ is the underlying word of $Y$
    and there exist colors $a_1,a_2,\ldots \in \{c_r+1,c_r-1\}$ and
    $b_1,b_2\ldots \in \{c_1+1,c_1-1\}$ such that
    $S=wa_1w^{-1}b_1wa_2w^{-1}b_2\ldots $. If $X$ is finite it ends
    after an occurrence of either $w$ or $w^{-1}$. If $i \equiv j \md
    2r+2$ then $h(x_i) = h(x_j)$. 
    If $i \equiv j$ or $-j-1 \md 2r+2$, then $h(x_i) = h(x_j)$.
\end{prop}

% OBSOBS  LOS GUSANOS SIN FINALES PARECEN COMPLICARSE POR LAS SIMETRÍAS
% DE TRASLACIÓN. ¿PONGO ALGO AL RESPECTO?

Let us look now at the degenerate cases. If $Y$ is only one vertex we
can think that the previous theorems still hold but with $w$ being the
empty word, and since $c_1$ and $c_r$ do not exist, we get rid of the
restrictions $a_i\in \{c_r+1,c_r-1\}$ and $b_i\in \{c_1+1,c_1-1\}$. In
Figure~\ref{f:FoldedCat} each layer of $X$ would have only one vertex and no links; essentially $X$ would be ``standing up'' instead of being
folded. If $Y$ is isomorphic to $X$ then $S=w$ and we do not have any $a_i$
or $b_i$. In Figure~\ref{f:FoldedCat} $X$ would have only one layer. 

If one would try to prove an analogous result as \cref{p:CubsCat1end} for caterpillars with no ends, there would be two additional cases to consider: One would be when $Y$ is a caterpillar with one endpoint with an underlying sequence of colors $S= c_1 c_2 c_3,\ldots$. In this case, the underlying infinite word of $X$ would be $S^{-1}aS$ for some color $a$, where $S^{-1}=\ldots c_3 c_2 c_1$. The other case would be that when $Y$ is not a caterpillar but a premaniplex consisting of a cycle with underlying word $w$ and all the edges not in the cycle are semiedges. In this case $X$ would have the underlying infinite word $\cdots w w w \cdots$.

==> IntPropTesis.tex <==
\section{Intersection properties and coset geometries}\label{sec:int prop}

%\elias{veo dos opciones. Resumir y quitar el ejemplo, o cambiarlo todo a que estamos citando el artículo de 3 órbitas.}

%\elias{Aquí debe introducirse un ejemplo de 3 órbitas en vez de citar el capítulo}

In order to prove the Main Theorem, we need to characterize, in terms of generators and relations, the 
%relations, inequalities, and mainly, intersection properties that a 
groups $\Gamma$ 
%need to satisfy to 
that act by automorphisms on a polytope $\p$ in such a way that the symmetry type graph $\T(\G(\p),\Gamma)$ is isomorphic to a given premaniplex $X$.
We shall do this in order to be able to recover the polytope $\p$ as a coset geometry using the group $\Gamma$. 

We start with the premaniplex $X$ and provide it with a %generic 
voltage assignment $\xi$. 
%Every (edge-colored) graph that regularly covers $X$ can be obtained as the derived graph $X^\xi$ of some voltage assignment, and the group of covering transformations coincides with the voltage group. In other words, 
Recall that if $(X,\xi)$ is a voltage graph with voltage group $\Gamma$, then $X^\xi/\Gamma$ is isomorphic to $X$; conversely, if $\M/\Gamma$ is isomorphic to $X$ then there is a voltage assignment $\xi$ on $X$ such that $X^\xi$ is isomorphic to $\M$. 
Hence, by characterizing the voltage assignments $\xi$  that satisfy that the derived graph $X^\xi$ is the flag graph of a polytope, we  determine the conditions that $\Gamma$ must satisfy to be the automorphism group of a polytope with symmetry type $X$.%\elias{probablemente esto debería estar más compacto aquí y con detalles en la sección anterior}



\subsection{Voltage graphs and the path intersection property}\label{s:IntProp}




We have figured out how to construct a maniplex from a premaniplex via voltage assignments. It is then natural to ask: when is the obtained maniplex the flag graph of a polytope?
The answer, as we shall see in this section, is closely related to Theorem~\ref{t:PolyMani}. In fact, translating Theorem~\ref{t:PolyMani} to the setting of voltage assignments will give us
%Now that we know which voltage assignments give maniplexes as derived graphs, we want to know when these maniplexes are polytopal, so that we obtain an abstract polytope with the base premaniplex as its symmetry type graph with respect to $\Gamma$. 
%We will see that the additional 
conditions that take the form of {\em intersection properties} that certain distinguished subgroups and some left cosets must satisfy. %\elias{sí quiero poner esto aquí?} To find these Intersection properties we use the characterization of polytopal maniplexes given in Theorem~\ref{t:PolyMani}.
%Recall that if $\xi:\Pi(X)\to \Gamma$ is a voltage assignment, then $\xi(\Pi^{x,y}_I(X)) $ denotes the set of voltages of all the paths of $X$ from $x$ to $y$ whose edges have colors in $I$.
Given two vertices $x,y$ in $X$ and a set of colors $I\in\{0,1,\ldots,n-1\}$, let us denote by $\Pi^{x,y}_I(X)$ the set of (homotopy classes of) paths from $x$ to $y$ in $X$ that only use darts with colors in the set $I$.
So $\xi(\Pi^{x,y}_I(X)) $ denotes the set of voltages of all the paths of $X$ from $x$ to $y$ whose edges have colors in $I$.

\begin{teo}\label{t:IntProp-w}
  Let $X$ be a premaniplex and let $\xi:\Pi(X)\to \Gamma$ be a voltage assignment such that $X^\xi$ is a maniplex. Then $X^\xi$ is the flag graph of a polytope if and only if
  \begin{equation}\label{VolPIP}
    \xi(\Pi^{x,y}_I(X)) \cap \xi(\Pi^{x,y}_J(X)) = \xi(\Pi^{x,y}_{I \cap J}(X)),    
  \end{equation}
  for all $I,J \subset \{0,\ldots,n-1\}$ and all vertices $x,y$ in $X$.
\end{teo}
\begin{dem}
  Start by assuming that $X^\xi$ is the flag graph of a polytope. 
 % Then, by Theorem~\ref{t:PolyMani}, it satisfies the SPIP.
  Let $x$ and $y$ be vertices of $X$ and let
  $I,J\subset\{0,1,\ldots,n-1\}$. 
  Consider two paths, $W\in \Pi^{x,y}_I(X)$ and $W'\in
  \Pi^{x,y}_J(X)$, with the same voltage, say $\alpha\in\Gamma$. 
  When lifting $W$ and $W'$ in $X^\xi$, they lift to 
  paths $\os{W}$ and $\os{W}'$, respectively, that go from $(x,1)$ to $(y,\alpha)$ (here 1 is the identity element of $\Gamma$) and satisfying that $\os{W}$ uses edges with colors in $I$ while $\os{W}'$ uses edges with colors in $J$.  
  In fact, one would define $\os{W}$ and $\os{W}'$ as the paths that start at $(x,1)$ and follow the same sequence of colors as $W$ and $W'$ respectively.
  By Theorem~\ref{t:PolyMani} $X^\xi$ satisfies the
  SPIP, which implies that there is a path
  $\os{W}''$ from $(x,1)$ to $(y,\alpha)$ that uses only colors in $I \cap J$. 
  Then, its projection $W'':= p(\os{W}'')$ is a path in $X$
  that goes from $x$ to $y$ that uses only colors in $I \cap J$ and
  has voltage $\alpha$. 
  This proves that $\xi(\Pi^{x,y}_I(X)) \cap
  \xi(\Pi^{x,y}_J(X)) \subset \xi(\Pi^{x,y}_{I \cap J}(X))$. Since the other
  contention is given, equality~(\ref{VolPIP}) must hold.

  Now let us assume that equality~(\ref{VolPIP}) holds for all $I,J\subset
  \{0,1,\ldots,n-1\}$ and all vertices $x$ and $y$. 
  Let $\os{W}$ and
  $\os{W}'$ be paths in
  $X^\xi$ from a vertex $(x,\gamma)$ to a vertex $(y,\tau)$. Let $I$ and $J$
  be the sets of colors of darts of $\os{W}$ and $\os{W}'$, respectively, and let $W:=p(\os{W})$
  and $W':=p(\os{W'})$ be the projections of the paths to $X$. 
  Then, both $W$ and $W'$ go from $x$ to $y$, and $W$ is a path with colors in $I$, while $W'$ is a path with colors in $J$, that is, $W\in \Pi^{x,y}_I(X)$ and $W'\in
  \Pi^{x,y}_J(X)$.
  Furthermore, since $\os{W}$ and $\os{W}'$ start at $(x,\gamma)$ and finish at $(y,\tau)$, they both have voltage
  $\alpha:=\tau\gamma^{-1}$. 
  By hypothesis, there exists a path $W''\in \Pi^{x,y}_{I \cap J}(X)$ that also has  voltage $\alpha$. 
  Then $W''$ has a unique lift $\os{W}''$ in $X^\xi$  starting at $(x,\gamma)$. The path $\os{W}''$ ends in $(y,\tau)$ and it uses darts
  of colors in $I \cap J$. This  proves that $X^\xi$ satisfies the
  SPIP and therefore, by Theorem~\ref{t:PolyMani}, it is the flag graph of a polytope. \qed
\end{dem}

Note that when $x=y$ the set $\xi(\Pi^{x,y}_I(X)) = \xi(\Pi^x_I(X))$ is a group,
since it is the image of a group under a groupoid
antimorphism. Actually, we shall find a set of distinguished generators
for the group $\xi(\Pi^x_I(X))$ in a similar way as  the distinguished
generators of the automorphism group of a polytope are found in
\cite{SymType}. 
Recall that $X_I$ is the subgraph of
$X$ induced by the edges with colors in $I$. Let $X_I(x)$ be the
connected component of $X_I$ containing the vertex $x$. 
To find a set of generators of $\xi(\Pi^x_I(X))$, fix a spanning
tree $T^x_I$ for $X_I(x)$. % (usually we would try to have as big an intersection with the spanning tree $T$ of $X$ as possible, but this
%is only for convenience). 
For each dart $d$ in $X_I(x)$ but not in
$T^x_I$
we get a cycle $C_d$ of the form $WdV$ where $W$ is the unique path
contained in $T^x_I$ from $x$ to the initial vertex of $d$, and $V$ is
the unique path contained in $T^x_I$ from the terminal vertex of $d$
to $x$. 
Then, the set $\{C_d\}$, where $d$ runs among
the darts in $X_I(x)$ not in $T^x_I$, is a generating set for
$\Pi^x_I(X)$. 
This imples that $\{\xi(C_d)\}$, where $d$ runs among the darts of $X_I(x)$ not in $T^x_I$, is a set of generators for
$\xi(\Pi^x_I(X))$. 
%We call these generators the \emph{distinguished generators of $\xi(\Pi^x_I(X))$ (with respect to $T$)}.

Since $\xi$ is a voltage assignment, we might consider only one dart $d$ for each edge. By denoting by $W_y$ the unique path
contained in $T^x_I$ from $x$ to $y$, we can see that $\Pi_I^{x,y}(X) = \Pi_I^x(X)W_y$ (that is, a path from $x$ to $y$ can be written as a closed path starting and finishing at $x$, concatenated with $W_y$), which implies that $\xi(\Pi^{x,y}_I(X)) =
\xi(W_y)\xi(\Pi^x_I(X))$.
Therefore, all the
intersection properties can be given in terms of left cosets of the groups $\xi(\Pi^x_I)$, whose generators we already know.

Theorem~\ref{t:IntProp-w} gives an intersection property for each pair
of vertices $(x,y)$ and each two sets of colors $I,J \subset
\{0,1,\ldots,n-1\}$. If we prove an intersection property for the pair
$(x,y)$, by taking the inverse on both sides we get the corresponding
property for the pair $(y,x)$, so we can consider only unordered pairs
$\{x,y\}$, and this reduces the number of intersection properties to
verify by a factor of 2. Still, the total number of intersection
properties is quadratic on the number of vertices %(since there are $v(v+1)/2$ unordered pairs of vertices, where $v$ is the number of vertices) 
and exponential
on the number of colors. %(since there are $2^{n-1}(2^n+1)$ pairs of sets of colors, where $n$ is the rank). 
This number gets too big
too quickly; however, many of these properties are redundant,
either because they are true for any group (for example, the
intersection of a group and one of its subgroups is the smaller
subgroup) or because they are a consequence of other intersection
properties.

Fortunately we may reduce the number of intersection properties to
check by following the same proof but using the {\em weak} path
intersection property instead of the strong one. Doing this we get
the following refinement of the previous theorem.

\begin{teo}\label{t:IntProp}
  Given a premaniplex $X$ and a voltage assignment $\xi$ such that
  $X^\xi$ is a maniplex, $X^\xi$ is the flag graph of a polytope if
  and only if
  \begin{equation}\label{eq:IntPropIntervalos}
    \xi(\Pi^{x,y}_{[0,m]}(X)) \cap \xi(\Pi^{x,y}_{[k,n-1]}(X)) =
    \xi(\Pi^{x,y}_{[k,m]}(X)),
  \end{equation}
  for all $k,m \in \{0,\ldots,n-1\}$ and all $x,y\in \F$.
\end{teo}

With Theorem~\ref{t:IntProp} the number of intersection properties to
check is now quadratic on the number of vertices and also quadratic on
the rank. We can still refine this theorem a little more with the following observations: 
\begin{itemize}
    \item The cases $k=0$ and $m=n-1$ say that the intersection of the whole voltage group with some subset is the subset itself, so they are trivially true for every voltage assignment.
    
    \item %\elias{Ésta es la que podemos quitar y poner en la def de WPIP. Habría también que modificar el teorema} 
    In Theorem~\ref{t:IntProp} one has to consider the cases when $k>m$.
    In such case, $\xi(\Pi^{x,y}_{[k,m]}(X))$ is the trivial group when $x=y$ and the empty set when $x \neq y$.
    However, if the intersection property holds for $k=m+1$, that is, if $\xi(\Pi^{x,y}_{[0,m]}(X)) \cap \xi(\Pi^{x,y}_{[m+1,n-1]}(X)) =
    \xi(\Pi^{x,y}_{\emptyset}(X))$, then it also holds for $k>m+1$. So one may only verify the intersection property for $k\leq m+1$.
    
    \item If $y$ and $y'$ are in the same connected component of $X_{[k,m]}$ and ~(\ref{eq:IntPropIntervalos}) is satisfied for the pair $(x,y)$, then it is also satisfied for the pair $(x,y')$.
    To see this, let $W$ be a path from $y$ to $y'$ with colors in $[k,m]$ and notice that $\Pi^{x,y'}_I(X) = \Pi^{x,y}_I(X)W$ whenever $I$ contains $[k,m]$. By taking voltages we get that $\xi(\Pi^{x,y'}_I(X)) = \xi(W)\xi(\Pi^{x,y}_I(X))$. 
    This means that we can get the intersection property for the pair $(x,y')$ by multiplying the one for pair $(x,y)$ by $\xi(W)$ on the left.
    So for each pair of numbers $(k,m)$ we only need to verify one intersection property for each pair of connected components of $X_{[k,m]}$.
\end{itemize}

Taking the previous observations into consideration, the maximum amount of necessary intersection properties to check is $v(v+1)/2\sum_{m=0}^{n-2} (m+1) =  v(v+1)n(n-1)/4$. 
But to reach this bound we need for every vertex to be in a different connected component of $X_{[k,m]}$ for every pair $(k,m)$ with $0<k\leq m+1$, which is only possible when every link has color 0 or $n-1$. This implies that every example where this bound is tight has at most 4 vertices (as for $n\geq 3$ the colors $0$ and $n-1$ are not consecutive).
%But to reach this bound we need for every vertex to be in a different connected component of $X_{[k,m]}$ for every pair $(k,m)$ with $0<k\leq m+1$, which is only possible when $v=1$. In other words, this bound is not tight for symmetry type graphs with more than one vertex.%Quitar esta línea, pues es falsa (ver WhatsApp)!

\ifEjemploPropsTresOrb
Using Theorem~\ref{t:IntProp} on the premaniplex $3^1$ we get the following
intersection properties (in parenthesis the values of $k$ and $m$ and
a choice endpoints for each property):

\begin{eqnarray}\label{IntProp3^1s}
    \begin{aligned}
        \gen{\alpha_1, \beta_0} \cap \gen{\alpha_1,\beta_2^{\alpha_{02}}} &=& \gen{\alpha_1}\quad (k=1, m=1, x\to x)\nonumber\\
        \gen{\alpha_1, \beta_0} \cap \gen{\alpha_1^{\alpha_{02}}, \beta_2} &=& 1\quad (k=1, m=1, y\to y)\nonumber\\
        \gen{\alpha_1,\beta_0} \cap \alpha_{02}\gen{\alpha_1,\beta_2^{\alpha_{02}}} &=& \emptyset\quad  (k=1, m=1, x\to y)\nonumber\\
        \gen{\alpha_1,\beta_0} \cap \{\alpha_{02}\} &=& \emptyset\quad (k=2, m=1, x\to y)\nonumber\\
        \gen{\beta_0} \cap \gen{\alpha_1^{\alpha_{02}},\beta_2} &=& 1\quad (k=1, m=0, z\to z).
  \end{aligned}
\end{eqnarray}\elias{arreglar para que quede bien la referencia}
We have omitted the properties that are redundant or that hold trivially for any voltage assignment.

Applying Theorem~\ref{t:IntProp} to the premaniplex $3^1$ and using  Corollary~\ref{c:Mani3^1} we get the following result:

\begin{teo}\label{t:3^1}
  A group $\Gamma$ acts on a polytope with symmetry type graph $3^1$ if and only if it is generated by 4 involutions $\alpha_1,\alpha_{02}, \beta_0$ and $\beta_2$ such that $\beta_0$ commutes with $\beta_2$ and the intersection properties~(\ref{IntProp:3^1s} hold.
\end{teo}

A previous characterization for the automorphism groups of polytopes with symmetry type graph $3^1$ was given in~\missingref[el de 3 óbitas], however in that paper 7 intersection properties need to be checked, in contrast to the 5 presented here.
We can get the 7 conditions in~\missingref[el de 3 óbitas] if we use Theorem~\ref{t:IntProp-w} instead and make some choices for $I$
 and $J$. In this case, using Theorem~\ref{t:IntProp} only saves us 2 intersection properties, but in higher rank the difference would be way more significant.
\fi

\subsection{Constructing a polytope from the voltage
  group}\label{s:Construction}

%\elias{tal vez queremos refrasear esta introducción para que suene más llamativo. Algo tipo "Ahora usamos los resultados de lasección anterior para construir politopos con cualquier tipo de simetría como coset geometries} 
We have seen how to recover a polytope from its flag graph (see
Theorem~\ref{t:GrafBand}) and when
$X^\xi$ is the flag graph of a polytope for a given premaniplex $X$
and a voltage assignment $\xi$ (see Theorem~\ref{t:IntProp}). By
concatenating the construction of $X^\xi$ from $X$ and $\xi$, and the
construction of a polytope $\p$ from $X^\xi$ we get a construction of
a polytope from $X$ and $\xi$. 
In this section, we translate this to give a
construction only in terms of subgroups of $\Gamma$ and their
cosets. This will give the proof of the Main Theorem.

%Let $<$ be an arbitrary well order relation\elias{si queremos podemos cambiarlo por una función de selección} on the vertices of $X$. 
Let $f$ be a choice function on the connected subgraphs of $X$, that is, a function that assigns a base vertex to each such subgraph.
Let $C$
be a connected component of $X_I$ for some
$I\subset \{0,1,\ldots,n-1\}$ and let $x=f(C)$. 
Let $\ol{C}:=(X^\xi)_I(x,1)$, that is, the connected
component of $(X^\xi)_I$ containing $(x,1)$.
Thus, if
$(x,\gamma) \in \ol{C}$, then there is a path $\os{W}$ from $(x,1)$ to
$(x,\gamma)$ which uses only colors in $I$, which implies that its projection is a
closed path $W$ in $\Pi^x_I(X)$ with voltage $\gamma$. This means that
when considering the action of $\Gamma$ on $X^\xi$, the stabilizer of
$\ol{C}$ coincides with $\xi(\Pi^x_I(X))$. If we now consider a coset
$\xi(\Pi^x_I(X)) \sigma$, this would be the set of elements of
$\Gamma$ that map $\ol{C}$ to $(X^\xi)_I(x,\sigma)$.

We know that the $i$-faces of the polytope that has $X^\xi$ as its
flag graph correspond to the connected components of
$(X^\xi)_{\ol{i}}$. 
This makes natural the following construction:

Given $X$ and $\xi$ satisfying Theorem~\ref{t:IntProp} and %an order
%$<$ on the vertices of $X$,
a choice function $f$ on the connected subgraphs of $X$, 
we  will construct a
partially ordered set $\p(X,\xi)$. 
We will start by defining the underlying set and a rank function and define the order relation later.
Let us define the elements of rank $i$ of $\p(X,\xi)$ 
as the right cosets of groups of the type
$\xi(\Pi^x_{\ol{i}}(X))$ where 
\[
x \in \{f(C)|C\ {\rm is\ a\ connected\
  component\ of}\ X_{\ol{i}}\}.
 \] 
  We have to consider these groups as formal copies, that is, if $x$ and $x'$ are on different connected components we consider $\xi(\Pi^x_{\ol{i}}(X))$ to be different than $\xi(\Pi^{x'}_{\ol{i}}(X))$, even if, as groups, they might be equal. 
  Likewise, if $j\neq i$ but $\xi(\Pi^x_{\ol{i}}(X))$ coincides with $\xi(\Pi^{x'}_{\ol{j}}(X))$ we consider them to be different in $\p(X,\xi)$.
  We could formalize this by saying that the elements of rank $i$ in $\p(X,\xi)$ are pairs $(C,\xi(\Pi^x_{\ol{i}})\gamma)$ with $C$ a connected component of $X_{\ol{i}}$, $x=f(C)$ and $\gamma \in \Gamma$, but since $x$ and $i$ already appear in the notation, we may assume that $\xi(\Pi^x_{\ol{i}}(X))\gamma$ stands for the pair $(X_{\ol{i}}(x),\xi(\Pi^x_{\ol{i}}(X))\gamma)$.
  
 % Here we have used the order relation $<$ to have a natural representative for each component where we will base a fundamental group.
 % We could also have used any other choice function.\elias{tal vez quitar este párrafo?}
%
%We still need to define the order on $\p(X,\xi)$, and we do this as
%follows.\elias{no me encanta esta forma de decirlo}

Now we shall define the order on $\p(X,\xi)$ as follows.
First, for all $i\in\{0,1,\ldots,n-1\}$ and every vertex $y$
in $X$ we look at the connected component $X_{\ol{i}}(y)$ and fix a
path going from its base vertex $x=f(X_{\ol{i}}(y))$ to $y$. We call
this path $W^y_i$ and we denote its voltage by
$\alpha_i^y:=\xi(W^y_i)$.

\begin{Def}[Order in $\p(X,\xi)$]\label{d:p(X,xi)}
  %{\em Order in $\p(X,\xi)$:} 
  Given $0\leq i<j \leq n-1$, let $C$ be a
  connected component of $X_{\ol{i}}$ and $C'$ be a connected
  component of $X_{\ol{j}}$, and let $x$ and $x'$ be their respective
  base flags.  Given $\gamma, \gamma' \in \Gamma$, we say that
  \begin{eqnarray}
  \xi(\Pi^x_{\ol{i}}(X))\gamma < \xi(\Pi^{x'}_{\ol{j}}(X))\gamma'\ \mathrm{if} \ \mathrm{
  and}\ \mathrm{ only}\ \mathrm{ if} \
 \alpha^y_i \xi(\Pi^x_{\ol{i}}(X))\gamma \cap
  \alpha^y_j\xi(\Pi^{x'}_{\ol{j}}(X))\gamma' \neq \emptyset, \nonumber
    \end{eqnarray}
    for some $y \in C \cap C'$.
  % where $\alpha_i$ and $\alpha_j$ are the voltages of
  % fixed paths $W \in \Pi^{x,y}_{\ol{i}}$ and $W' \in
  % \Pi^{x',y}_{\ol{j}}$ respectively.
\end{Def}

%For the next Theorem, keep in mind that $\Gamma$ might not be the full automorphism group of $\p(X,\xi)$.

\begin{teo}\label{t:Recons}
  Let $X$ be a premaniplex and $\xi:\Pi(X)\to \Gamma$ a voltage
  assignment satisfying Theorem~\ref{t:IntProp}. Let
  \[
  \begin{split}
  \p(X,\xi) := \{\xi(\Pi^x(C))\tau:&\ C {\rm \ is\ a\ connected\ component
   \ of\ }
  X_{\ol{i}} \\ 
  &{\rm \ for\ some\ } i\in[0,n-1], x=f(C), \tau \in \Gamma\},
  \end{split}
  \]
  together with the order given in Definition~\ref{d:p(X,xi)}. Then
  $\p(X,\xi)$ is a polytope in which $\Gamma$ acts by right multiplication with symmetry type
  graph $X$.
\end{teo}

Note that $\Gamma$ might not be the full automorphism group of $\p(X,\xi)$, and thus $X$ might not be the symmetry type graph of $\p(X,\xi)$ with respect to its full automorphism group.

% To get a polytope from $X^\xi$
\begin{dem}

% We say that a component $\os{C}$ of
% $(X^\xi)_{\ol{i}}$ and a component $\os{C}'$ of $(X^\xi)_{\ol{j}}$ are
% incident if and only if they have non-empty intersection.

% We know that the faces of $X^\xi$ as a maniplex correspond to cosets
% of subgroups of $\Gamma$. Now we want to know when two of these faces
% are incident in terms of these cosets, so that we can use this to
% define an order in $\p(X,\xi)$.
%
%  In Section~\ref{sec:voltage} we saw that
  
 % $\xi:X\to \Gamma$ is a voltage assignment, then $p:X^\xi\to X$ is a
 % covering with covering transformations group $CT(p)=\Gamma$. In other
%  words, 
Let us denote $\p(X^\xi)$ as $\p$ and $\p(X,\xi)$ as $\Q$. 
  Note that Theorem~\ref{t:IntProp} implies that $\p$ is a polytope, and we want to show that $\Q$ is also a polytope (such that $\Q / \Gamma \cong X$).
  
  By the discussion in Section~\ref{s:VoltMani},  $\T(\p,\Gamma)\cong X$, since, by construction of $X^\xi$, we have that $X^\xi/\Gamma \cong X$.
 So in order to settle the theorem it is enough to find a poset isomorphism
  $\varphi:\p\to \Q$ such that it commutes with the action of
  $\Gamma$, that is, such that $\os{C}\sigma\varphi = \os{C}\varphi\sigma$ for all
  faces $\os{C}$ in $\Q$ and all $\sigma\in\Gamma$.


  Let $\os{C}$ be a face of $\p$. Hence,
  $\os{C}$ is a connected component of $X^\xi_{\ol{i}}$ for some color
  $i$. Let $C:=p(\os{C})$ and let $x:=f(C)$. This implies that $\os{C}$ has a flag $(x,\gamma)$ for some $\gamma \in \Gamma$. Let $\os{K}$ be
  the connected component of $X^\xi_{\ol{i}}$
  that contains $(x,1)$. 
Then, the set of elements of $\Gamma$
  that map $\os{K}$ to $\os{C}$  is
  $\xi(\Pi^x_{\ol{i}}(X))\gamma$. We want to identify $\os{C}$ with this
  coset, so we define $\os{C}\varphi:=\xi(\Pi^x_{\ol{i}}(X))\gamma$. Note that $\varphi:\p\to\Q$ is well defined, since if $(x,\gamma')$ is in $\os{C}$ then $\gamma'\gamma^{-1}$ stabilizes $\os{K}$, implying that $\gamma'\gamma^{-1} \in \xi(\Pi^x_{\ol{i}}(X))$.
  We want to prove that $\varphi$ is a poset isomorphism and that it
  commutes with $\Gamma$.

  Let us show first that $\varphi$ commutes with the action of
  $\Gamma$. 
  Let $\os{C}$ be a face in $\p$ and let $\sigma\in
  \Gamma$. By the definition of $\varphi$ we know that $\os{C}\varphi
  = \xi(\Pi^x_{\ol{i}}(X))\gamma$ where $i$ is the rank of $\os{C}$,
  $x=f(p(\os{C}))$ and $\gamma\in\Gamma$ is any element such that
  $(x,\gamma)\in \os{C}$. On the other hand $(\os{C}\sigma)\varphi =
  \xi(\Pi^{x'}_{\ol{i}}(X))\gamma'$ where $x'=f(p(\os{C}\sigma))$
  and $(x',\gamma')\in \os{C}\sigma$. Also note that since $\os{C}$
  and $\os{C}\sigma$ are in the same orbit, then
  $p(\os{C})=p(\os{C}\sigma)$, and thus $x=x'$. Furthermore, the flag
  $(x,\gamma\sigma) = (x,\gamma)\sigma$ is in $\os{C}\sigma$. This
  proves that $(\os{C}\sigma)\varphi =
  \xi(\Pi^x_{\ol{i}}(X))\gamma\sigma = (\os{C}\varphi)\sigma$.

  Now let us prove that $\varphi$ is an isomorphism of posets. Let
  $\os{C}$ and $\os{C}'$ be incident faces of $\p$ of ranks $i$ and
  $j$, respectively, with $i<j$ (therefore,
  $\os{C}<\os{C}'$). Hence, there is a flag $(y,\tau)$ in $\os{C} \cap
  \os{C}'$, which in turn implies that its first entry, $y$, must be in $C \cap C'$ where
  $C=p(\os{C})$ and $C'=p(\os{C}')$.

  Let $x=f(C)$ and $x'=f(C')$. Note that the path $W^y_i$ from $x$ to $y$ is contained in $C$, while
  $W^y_j$ from $x'$ to $y$ is contained in $C'$. Then, these paths have lifts
  $\os{W}^y_i$ and $\os{W}^y_j$ respectively, that go from
  $(x,(\alpha^y_i)^{-1}\tau)$ and $(x',(\alpha^y_j)^{-1}\tau)$,
  respectively, to $(y,\tau)$. Observe that $\os{W}^y_i$ is contained in
  $\os{C}$ and $\os{W}^y_j$
  is contained in $\os{C}'$. Thus, $(\alpha^y_i)^{-1}\tau \in
  \xi(\Pi^x_{\ol{i}}(X))\gamma$ and $(\alpha^y_j)^{-1}\tau \in
  \xi(\Pi^{x'}_{\ol{j}}(X))\gamma'$. Therefore
  \[
    \tau \in \alpha^y_i \xi(\Pi^x_{\ol{i}}(X))\gamma \cap
    \alpha^y_j \xi(\Pi^{x'}_{\ol{j}}(X))\gamma' = \alpha^y_i
    (\os{C}\varphi) \cap \alpha^y_j (\os{C}'\varphi);
  \]
  but this means that $\os{C}\varphi<\os{C}'\varphi$ in $\Q$.

  Conversely, suppose that $\os{C}\varphi<\os{C}'\varphi$ in
  $\Q$. We want to
  show that $\os{C}<\os{C}'$ in $X^\xi$. Let us write $\os{C}\varphi =
  \xi(\Pi^x_{\ol{i}}(X))\gamma$, where $i$ is the rank of $\os{C}$, $x:=f(p(\os{C}))$ and $\gamma$ is an element of
  the voltage group such that $(x,\gamma)\in \os{C}$. Similarly, we
  write $\os{C}'\varphi =
  \xi(\Pi^{x'}_{\ol{j}}(X))\gamma'$, where $j$ is the rank of $\os{C}'$,
  $x:=f(p(\os{C}'))$ and $\gamma'$ is an
  element of the voltage group such that $(x',\gamma')\in \os{C}'$.

  By hypothesis $\alpha^y_i \xi(\Pi^x_{\ol{i}}(X))\gamma$ and $\alpha^y_j
  \xi(\Pi^{x'}_{\ol{j}}(X))\gamma'$ have non-empty intersection for some
  $y\in C\cap C'$. Let $\tau$
  be an element in such intersection. Then $(\alpha^y_i)^{-1}\tau \in
  \xi(\Pi^x_{\ol{i}}(X))\gamma$. This implies that
  $(x,(\alpha^y_i)^{-1}\tau)$ is in the same connected component of
  $(X^\xi)_{\ol{i}}$ as $(x,\gamma)$, that is $(x,(\alpha^y_i)^{-1}\tau)
  \in \os{C}$. 
  But at the same time, there is a
  lift of $W^y_i$ that connects $(x,(\alpha^y_j)^{-1}\tau)$ with
  $(y,\tau)$, and since $W^y_i$ does not use the color $i$, its lift is
  contained in $\os{C}$, which proves that
  $(y,\tau)\in\os{C}$. Similarly, the fact that
  $(\alpha^y_j)^{-1}\tau \in \xi(\Pi^{x'}_{\ol{j}}(X))\gamma'$ implies
  that $(y,\tau)\in \os{C}'$. Thus, we have proved that $\os{C}\cap
  \os{C}'$ is not empty, or in other words $\os{C}<\os{C}'$ in
  $\p$.

  Therefore, $\varphi$ is an isomorphism and the theorem follows. \qed

\end{dem}

\input{Caterpillars2}


%\end{document}


==> IntroV1.tex <==
In the 1970s several ideas extend the geometric study of convex polytopes to study and generalize them from different points of view. 
While Tits studies incidence systems, Coxeter focuses on tessellations of manifolds and Gr\"unbaum proposes to move away from spherical tiles.
In the early 1980s Danzer and Schulte put several of these ideas together to start the study of {\em incidence polytopes}, now called {\em abstract polytopes}.
%Thus, abstract polytopes generalize the classical notion of convex polytopes to more general combinatorial structures: 
An abstract polytope is a ranked, partially ordered set which generalizes the face lattice of a convex polytope. Thus, abstract generalize the classical notion of convex polytopes to more general combinatorial structures.

\elias{párrafo de Isa que hay que conciliar con el párrafo anterior} 
Abstract polytopes can be classified in terms of their so-called symmetry type graph (\cite{SymType}), which encodes all the information of the local configuration of flags (maximal chains of the partial order) with respect to the automorphism group.
It is well-known that regular and chiral polytopes can be seen as coset geometries (\cite{EgonPhd}, \cite{QuiralesEgonAsia}); this characterization of their automorphism groups constitute the more important tool to study them. In particular, regular polytopes are in one to one correspondence with the so called string C-groups, which are smooth quotients of Coxeter groups.

Incidence and coset geometries were first studied by Tits (\cite{Tits61}). The ideas behind these concepts are to construct incidence structures using groups, and in particular were developed by Tits in connection to Coxeter groups.

In this paper we show that not only regular and chiral polytopes can be seen as coset geometries, but that in fact any abstract polytope can be constructed as a coset geometry. To show this, we characterize the automorphism group with a given symmetry type graph, in terms of generators and relations.

The degree of symmetry of an abstract polytope is measured by counting the number of flag
orbits under the action of its automorphism group.


A {\em flag} in a polytope consists of one face of each rank all
incident to each other. 
A good way of
measuring % ``how symmetric is a polytope''
the degree of symmetry of a polytope is by counting the number of flag
orbits under the action of its automorphism group
(that is, its group of symmetries). Polytopes with only 1 flag-orbit
are called {\em regular} and they are by far the most studied. The
book~\cite{ARP} is the standard reference and is dedicated exclusively
to abstract regular polytopes.

More recently the study of 2-orbit polytopes and maniplexes (abstract
polytopes or maniplexes with 2 flag-orbits) has become more popular
(see~\cite{2OrbPol1}, for example). When studying 2-orbit polytopes,
one realizes that there are many different types of them, depending of
which symmetries can occur or not. For example, {\em chiral} polytopes
(the most studied non-regular polytopes) are 2-orbit polytopes where
there are no ``reflections' but there are all ``rotations''. In the
context of maps, {\em rotary} maps, i.e. those with all the possible
rotational symmetry, are extensively studied; many authors even use the
word {\em regular} to refer to them
(see~\cite{JonesSingerman_1978_TheoryMapsOrientable}, for example).


% , that is,
% every two flags differing exactly in one face are in different orbits.

Certain types of 2-orbit polytopes are much more elusive than regular
ones. In 1991~\cite{QuiralesEgonAsia}, Schulte and Weiss study chiral
polytopes and classify their automorphism groups in terms of
generators and relations. Chiral 3-polytopes had been studied as maps
on surfaces, while Schulte and Weiss~\cite{ProjQuir} give examples of
infinite families of finite and infinite chiral 4-polytopes. They also
construct examples of (locally) infinite 5-polytopes and post the
question of the existence of higher rank (finite and infinite) chiral
polytopes~\cite{EgonAsiaFree}. In 2008, Conder, Hubard and Pisanski
use algebraic methods to construct the first examples of finite chiral
polytopes of rank 5~\cite{QuiralesConstruct}, and it is until 2010,
almost 20 years after Schulte and Weiss's first paper, that Pellicer
finally proves that chiral polytopes exist in any rank higher than
2~\cite{Quirales}. However, the automorphism groups of the constructed
polytopes are too big to be understood.

The general theory of 2-orbit polyhedra
was studied by Hubard in~\cite{2OrbPol1} in 2010, where she uses a
similar approach to that of chiral polytopes to find conditions on a
set of generators of a group to be the automorphism group of a 2-orbit
polyhedron. In 2016 Matteo classifies 2-orbit convex polytopes and
finds that they only exist in dimensions 2 and 3
(geometrically)~\cite{Matteo}. More recently, Pellicer, Poto\v{c}nik
and Toledo show that there are 2-orbit maniplexes of any type with
rank higher than 2, but they might not necessarily be flag graphs of
polytopes~\cite{2OrbMani}.

In~\cite{AsiaDaniel} Orbanić, Pellicer and Weiss study 3-orbit maps
and they also divide them by types according to what kind of
symmetries are allowed or not.

The literature on $k$-orbit polytopes with $k\geq 3$ is far less
abundant. In~\cite{k-orb} Cunningham and Pellicer give a list of open
problems (at the time) about $k$-orbit polytopes for arbitrary $k$.

In order to study $k$-orbit polytopes one needs a certain method to
find all the different types that might exists. To do this,
in~\cite{SymType} the concept of {\em symmetry type graph} of a
maniplex is introduced as a generalization of the Delaney-Dress symbol
previously used for maps and described in~\cite{Dress2}
and~\cite{Dress1}. The symmetry type graph of a polytope or maniplex
is a graph that not only tells us how many orbits the polytope or
maniplex has, but also how these orbits are connected and what kinds of
symmetries the object has. Essentially, it summarizes the
information about the symmetric structure of the polytope or maniplex.



The problem of finding polytopes with a given symmetry type graph is
in general very difficult, as one can note, for example, by looking
at the history of chiral polytopes. There are some necessary
conditions a graph must satisfy to be the symmetry type graph of a
maniplex or polytope. Graphs satisfying these conditions are called
{\em multi-maniplexes} in this thesis. At the time this thesis is
being written, it is not known if every multi-maniplex with rank
$n\geq 3$ is the symmetry type graph of a polytope or a
maniplex. This is in fact Problem 12 in~\cite{k-orb}.

Previously we mentioned that it is known that all multi-maniplexes
with 2 vertices are symmetry type graphs of a
maniplex~\cite{2OrbMani}, but it is not known if they are polytopal
(i.e. the flag graph of a polytope). It is known that every
multi-maniplex with 3 vertices with rank $n\geq 3$ is the symmetry
type graph of a polytope~\cite{SymType}.

By using {\em
  voltage assignments} one can construct a maniplex $\M$ from
a multi-maniplex $X$ and a group $G$ (satisfying some
conditions). Then $G$ will act on $\M$ by automorphisms and the
quotient of $\M$ by the action of $G$ will be $X$. This means that
$\M$ will have symmetry type graph $X$ if and only if every
automorphism of $\M$ is represented by the action of an element of
$G$. In this thesis we give an algebraic test to $G$ that tells us if
the constructed maniplex $\M$ is polytopal or not, thus translating
the problem of finding polytopes with a given symmetry type graph to a
group-theoretic one.

The main methods for studying regular polytopes (see~\cite{ARP}) and
2-orbit polyhedra (see~\cite{2OrbPol1}) have been algebraic. The
automorphism groups of these polytopes are characterized as groups
generated by a certain amount of elements satisfying certain relations
and intersection properties that depend on the symmetry
type. In~\cite{k-orb} Cunningham and Pellicer ask the following
question for $k$-orbit polytopes:

\begin{preg}\label{preg:IntProp}
  Given a distinguished generating set for the automorphism
  group of a $k$-orbit polytope, what analogue of the intersection
  condition holds?
\end{preg}

We shall give a complete answer to this question in this
thesis in terms of the symmetry type graph. Moreover, given the
symmetry type graph we will also answer its follow-up question, which
asks how to rebuild a $k$-orbit polytope from its automorphism
group. More concretely, the question asks:

\begin{preg}\label{preg:Recons}
  Describe a way to build a general polytope as a coset geometry of
  its automorphism group, given a distinguished set of generators.
\end{preg}

% Given the symmetry type and the automorphism group there is a way to
% rebuild the polytope as a coset geometry. In this work we will show
% how to do this for $k$-orbit polytopes with an arbitrary given
% symmetry type graph. This gives an answer to Problems 1 and 2
% from~\cite{k-orb}.

Questions~\ref{preg:IntProp} and~\ref{preg:Recons} are Problems 1 and
2 in~\cite{k-orb}, respectively.

==> IntroV2.tex <==
In the 1970s several ideas extended the geometric study of convex polytopes to  generalize them from different points of view: 
while Tits studied incidence systems, Coxeter focused on tessellations of manifolds and Gr\"unbaum proposed to move away from spherical tiles.
In the early 1980s Danzer and Schulte put several of these ideas together to start the study of {\em incidence polytopes}, now called {\em abstract polytopes}.
%Thus, abstract polytopes generalize the classical notion of convex polytopes to more general combinatorial structures: 
An abstract polytope is a ranked, partially ordered set which generalizes the face lattice of convex polytopes and tessellations. Thus, abstract polytopes generalize the classical notion of convex polytopes and tessellations to more general combinatorial structures.


The degree of symmetry of an abstract polytope is measured by counting the number of flag
orbits under the action of its automorphism group, where a flag is a maximal chain of the partial order.
Abstract polytopes can then be classified in terms of their so-called symmetry type graph (\cite{SymType}), which encodes all the information of the local configuration of flags with respect to the automorphism group. 

Polytopes with only one flag-orbit
are called {\em regular} and  are  the most studied ones. 
Regular polytopes have maximal degree of symmetry and in particular their automorphism groups are generated by involutions, often called ``(abstract) reflections''.
The
book Abstract Regular Polytopes~\cite{ARP} by McMullen and Schulte is the standard reference and it is devoted exclusively
to the study of abstract regular polytopes.
%
There are $2^{n}-1$ classes of n-polytopes with 2 flag orbits, each of them corresponding to one symmetry type graph. 
Among them is the class of {\em chiral} polytopes (\cite{QuiralesEgonAsia}), which have no ``reflectional'' symmetry, but have maximal ``rotational'' one.

The study of coset geometries goes back to Tits (\cite{Tits61}). 
The ideas behind this concept are to construct incidence structures using groups, and in particular were developed by Tits in connection to Coxeter groups.
It is well-known that regular and chiral polytopes, as well as two-orbit polyhedra can be seen as coset geometries (see \cite{EgonPhd},\cite{2OrbPol1} and \cite{QuiralesEgonAsia}); this characterization of their automorphism groups 
constitute the most important tool to study them. 
In a recent paper (\cite{3Orb}), the authors showed that 3-orbit polyhedra, as well, can be seen as coset geometries, and this fact is used to construct 3-orbit polyhedra from symmetric groups.
%In particular, regular polytopes are in one to one correspondence with the so called string C-groups, which are smooth quotients of Coxeter groups.
%

The purpose of this paper is to prove the following theorem.
\begin{Mteo}
Every abstract polytope can be constructed as a coset geometry.
\end{Mteo}
 To show this, we characterize the automorphism group of an abstract polytope with a given symmetry type graph, in terms of generators and relations, as well as some intersection conditions on some subgroups and cosets.

 
Throughout the paper, we work with the flag graph of a polytope, as opposed to  the partial order. In fact, we shall often work with {\em maniplexes}, that is, colored graphs that generalize flag graphs of polytopes (\cite{Maniplexes}).
%In particular, we also explicitly show that every maniplex can be constructed as a coset geometry, fact that follows from \cite{SymType} and \cite{Voltajes}.

As pointed out before, symmetry type graphs are a great tool to classify polytopes (and maniplexes) in terms of their automorphism groups.
We will rely on them heavily in our study.
There are some (necessary)
conditions a graph must satisfy to be the symmetry type graph of a
maniplex or polytope. 
Graphs satisfying such conditions are called
{\em premaniplexes} (or admissible graphs) and will be properly defined in Section~\ref{s:STG}.
We believe our main theorem will shed light to the study of $k$-orbit polytopes; in particular, it opens the gate to study one of the main problems in the area (listed as Problem 12 in~\cite{k-orb}):

\begin{preg}\label{q:premaniplexasSTG}
  Given a premaniplex, does it exist a polytope (or maniplex) having such premaniplex as its symmetry type graph?
\end{preg}

The problem of finding polytopes or maniplexes with a given symmetry type graph is
in general very difficult, as one can note, for example, by looking
at the history of chiral polytopes:
although it was back in 1991~\cite{QuiralesEgonAsia}, when Schulte and Weiss studied chiral
polytopes and classified their automorphism groups in terms of
generators and relations, it took almost $20$ years to have a construction showing that such polytopes existed for all ranks $n>3$ (see \cite{Quirales}).


%At the time this paper is
%being written, it is not known if every premaniplex with rank
%$n\geq 3$ is the symmetry type graph of a polytope or a maniplex. %This is in fact Problem 12 in~\cite{k-orb}.


Very little is know about other particular instances of Question~\ref{q:premaniplexasSTG}. 
It is known~\cite{SymType} that every
premaniplex with 3 vertices with rank $n\geq 3$ is the symmetry
type graph of a polytope,
and in~\cite{2OrbMani} Pellicer, Potočnik and Toledo proved that every premaniplex of rank $n\geq 3$ with 2 vertices is the symmetry type graph of a maniplex, but it is not known if the constructed maniplexes are polytopal
(i.e. the flag graph of a polytope). 
%The results of this paper can help to determine the polytopality of such maniplexes.


This paper is organized as follows. In Section~\ref{sec:Polytopes-and-maniplexes} we give the basic concepts from the theory of abstract polytopes as well as maniplexes, and formally introduce the concepts of symmetry type graphs and premaniplexes. We also state a relaxed version of Question~\ref{q:premaniplexasSTG}, that we answer later, in Section~\ref{s:IntProp}.
We start Section~\ref{sec:voltage} by going over the main tool used in this paper: voltage graphs. Then,
by using them, in Section~\ref{s:VoltMani} we construct a maniplex $\M$ from
a premaniplex $X$ and a group $G$ (satisfying some
conditions). 
Then $G$ will act on $\M$ as a group of automorphisms and the
quotient of $\M$ by the action of $G$ will be $X$. 
This means that $\M$ will have symmetry type graph $X$ if and only if every automorphism of $\M$ is represented by the action of an element of $G$. 

In Section~\ref{s:IntProp}, we use the construction of Section~\ref{sec:voltage}, as well as the results from \cite{PolyMani}, to characterize in terms of generators and relations the groups that are automorphism groups of a polytope with a given symmetry type graph. We do so by showing that automorphism groups of polytopes must satisfy certain ``intersection conditions'' for some subgroups and cosets, that depend on the symmetry type graph.
In other words, we give an algebraic test for the group $G$ of Section~\ref{s:VoltMani}  that tells us if
the constructed maniplex $\M$ is polytopal or not, thus translating
the problem of finding polytopes with a given symmetry type graph to a
group-theoretic one.
This gives an answer to Problem 1 of \cite{k-orb}. 
In Section~\ref{s:Construction} we give the proof to the Main Theorem by constructing a polytope as a coset geometry from a voltage group.
This gives an answer to Problem 2 of \cite{k-orb}.

We finish the paper in Section~\ref{s:Caterpillars} by using the above result to construct $k$-orbit $n$-polytopes with Boolean automorphism groups, (that is, elementary Abelian $2$-groups), 
for all $k, n\geq 3$. 
For this, we define {\em caterpillars} as premaniplexes having exactly one generating tree, and study their coverings in order to avoid the possible extra symmetry that might happen when one uses our construction to obtain polytopes from groups.

==> STG.tex <==
A \emph{$k$-orbit maniplex} is one with exactly $k$ flag orbits under its automorphism group.
When studying $k$-orbit maniplexes with $k>1$ one finds that it is convenient  to classify them in terms of the local structure of the flags. 
For this reason, in~\cite{SymType}, Cunningham et al. introduce the concept of \emph{symmetry type graph}.

Given a maniplex $\M$ and a subgroup $G$ of the automorphism group of $\M$, the \emph{symmetry type graph of $\M$ with respect to $G$}, denoted either by $\T(\M,G)$ or by $\M/G$, is constructed as follows: 
The vertex set of $\T(\M,G)$ is the set of flag orbits of $\M$ under the group $G$, and if $\Phi$ and $\Psi$ are $i$-adjacent in $\M$ we draw an edge of color $i$ between their orbits.
If $\Phi$ and $\Phi^i$ are in the same orbit under $G$, we draw a semi-edge of color $i$ at the vertex corresponding to that orbit. 
Note that a semi-edge is different from a loop in that it consists of an edge with only one endpoint, rather than an with two equal endpoints; that is, a semi-edge is incident to its vertex once, while a loop is incident to its vertex two times.

%of only one dart which is inverse to itself, rather than two darts starting at the same vertex; less formally, a semi-edge is incident to the vertex once, while a loop is incident to the vertex two times.

When we speak about \emph{the symmetry type graph of $\M$}, we mean it with respect to $\Gamma(\M)$ and we simply write $\T(\M)$ instead of $\T(\M,\Gamma(\M))$.

If $\p$ is a polytope, \emph{the symmetry type graph of $\p$ (with respect to $G$)}  is defined as the symmetry type graph (with respect to $G$) of its flag graph.

If $X$ is the symmetry type graph of an $n$-maniplex, then it is a connected graph in which every vertex is incident to exactly one edge of each color in $\{0,1,\ldots,n-1\}$ and it satisfies that if $|i-j|>1$, the paths of length 4 that alternate between the colors $i$ and $j$ are closed. 
However, it might not be a maniplex as it is not necessarily simple. 
We will call such a graph a \emph{$n$-premaniplex}.

If $X$ is a premaniplex and $i,j\in\{0,1,\ldots,n-1\}$ are non-consecutive, the connected components of the subgraph of $X$ induced by the edges of colors $i$ and $j$ are not necessarily 4-cycles. In fact they can be any quotient of a 4-cycle, as illustrated in Figure~\ref{f:ijComponentes}.

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{ijComponentes.pdf}
    \caption{Components of two non-consecutive colors in a premaniplex.}
    \label{f:ijComponentes}
\end{figure}

The notions of \emph{homomorphism, isomorphism, automorphism} and \emph{monodromy group} from maniplexes can all be easily extended to premaniplexes as well.

The natural projection $p:\M\to\T(\M,G)$ is, of course, a homomorphism (of premaniplexes). 
%In fact, it is a covering projection with covering group $G$.

When studying polytopes (or maniplexes) and their symmetry type graphs two natural questions occur:
\begin{itemize}

\item     Given a premaniplex $X$, is there a polytope (or maniplex) whose symmetry type graph is $X$? (see \cref{q:premaniplexasSTG})
%\end{preg}

\item
%\begin{preg}\label{q:IntProp}
    Given a premaniplex $X$, what conditions must a group $G$ satisfy so that there is a polytope (or maniplex) $\p$ such that $\T(\p,G)\cong X$?
    % If there is such $\p$, can we determine wether $G$ is the full automorphism group of $\p$ or a proper subgroup?
%\end{preg}

\end{itemize}

%Questions~\ref{q:SymType} and~\ref{q:IntProp} appear as questions 12 and 1 in~\cite{k-orb}, respectively.

In \cref{s:IntProp} we give a complete answer to the latter.  \cref{q:premaniplexasSTG}
 remains as a hard question, as even if we find a polytope $\p$ and a group $G$ such that $\T(\p,G)\cong X$, it may still happen that $G$ is a proper subgroup of $\Gamma(\p)$.
However, in \cref{s:Caterpillars} we give an infinite family of premaniplexes that are in fact symmetry type graphs of polytopes.

==> VoltMan.tex <==
\subsection{Voltage graphs that give maniplexes as derived graphs}\label{s:VoltMani}

 
Of course, we want to use voltage graphs to obtain maniplexes (and polytopes). In this section we shall give necessary and sufficient conditions on a voltage assignment $\xi$ on a premaniplex $X$ so that $X^\xi$ is a maniplex.

Let $\M$ be a maniplex, $\Gamma$ a group of automorphisms of $\M$ and $X=\T(\M,\Gamma)$.
Let $T$ be a spanning tree of $X$. As mentioned before, there is a voltage assignment $\xi:\Pi(X)\to \Gamma$ such that $X^\xi$ is isomorphic to $\M$ and $\xi(d)=1$ for every dart $d$ in $T$.
The set of non-trivial voltages of darts in $X$ then gives a generating set for the group $\Gamma$. In fact, if we keep only one element from each pair of inverse generators, what we get is the set of \emph{distinguished generators of $\Gamma$}, as defined in  \cite[Section 5]{SymType}.
%However, not every voltage assignment on $X$ will give a maniplex as the derived graph. 

\if
In \cite[Section 5]{SymType} the authors find a set of distinguished generators for the automorphism group of a maniplex $\M$ with a given symmetry type graph $X$. 
It is easy to see that there is a spanning tree on $X$ and a voltage assignment $\xi:\Pi(X)\to \Gamma(\M)$ such that $X^\xi\cong \M$ and the distinguished generators are exactly the voltages of the darts of $X$ not in $T$ (excluding inverses and neutral elements).
%can be thought of as voltages assigned to $X$ (or more precisely to $\Pi(X)$) so that the derived graph is $\M$.
%To do this, one must choose a spanning tree $T$ on $X$ and assign trivial voltage to all its darts. %All the darts that are not in $T$ will have a non-trivial voltage. NO ES VERDAD NECESARIAMENTE
If we want to start with a premaniplex $X$, we need to be careful with the way we assign voltages so that the derived graph is indeed a maniplex.
\fi

\if
If the STG of $\M$ is $X$, there is a method to assign voltages to the remaining darts in such a way that the derived graph is isomorphic to $\M$.
It is known (\cite{SymType}\missingref{agregar resultado exacto}) that
the voltages of these darts have to generate the whole voltage group for the derived graph to be connected. So we call the non-trivial voltages of the darts
\fi

Conversely, given a premaniplex $X$ with fundamental groupoid $\Pi(X)$, let $T$ be a spanning tree of $X$ and let $\xi:\Pi(X)\to \Gamma$ be a voltage assignment, for some group $\Gamma$ such that $\xi(d)=1$ for every dart $d$ in $T$.
In what follows, we find the conditions on $\Gamma$ and $\xi$ that ensure that $X^\xi$ is actually a maniplex.
%, but before doing so, let us assume that there is a spanning tree $T$ of $X$ with trivial voltage in all its darts. 

First we want $X^\xi$ to be connected.
It is known (see~\cite{Voltajes}) that in order for $X^\xi$ to be connected, $\xi(D)$ must generate $\Gamma$, where $D$ denotes the set of darts of $X$.

Next, $X^\xi$ must be a simple graph. 
Thus, it must not have semi-edges or multiple edges.
Note that a semi-edge of $X^\xi$ that starts at a vertex $(x,\gamma)$ ends in
$(x,\xi(e)\gamma) = (x,\gamma)$, where $e$ is a semi-edge of $X$.
This implies that if the voltage of every semi-edge of $X$ is not trivial, we avoid semi-edges in $X^\xi$.
Since $\xi$ is an antimorphism we should have that $\xi(e)=\xi(e^{-1}) = \xi(e)^{-1}$, implying that the voltage of a semi-edge must have order two.

%\elias{nuevo párrafo} 
%
To avoid multiple edges, we need to avoid different darts with the same initial and terminal vertices;
%If $X^\xi$ had parallel darts, their images under the covering projection $X^\xi\to X$ would also be parallel darts, %, since parallel darts are mapped to either parallel darts or to the same dart, but since homomorphism of premaniplexes preserve color, they cannot be  mapped to the same dart.
suppose $X^\xi$ has two parallel darts
$(d,\sigma)$ and $(d',\tau)$. 
Since both darts start at the same
vertex, we have that $(I(d),\sigma)=(I(d'),\tau)$, so $I(d)=I(d')$ and $\sigma =
\tau$. The common end-point of $(d,\sigma)$ and $(d',\tau)$ could be
written as $(y,\xi(d)\sigma)$
or $(z,\xi(d')\sigma)$, where $y$ is the end-point of $d$ and $z$ the
end-point of $d'$. The fact that these two are the same means
that $y=z$ and $\xi(d) = \xi(d')$. So $(d,\sigma)$ and
$(d',\sigma)$ are parallel darts in $X^\xi$ if and only if $d$ and $d'$ are
parallel darts in $X$ with the same voltage. Thus, $X^\xi$ has no parallel
darts if and only if no pair of parallel darts in $X$ has equal voltages.

Finally, we want to ensure that if $|i-j|>1$, the paths of length 4 in
$X^\xi$ that alternate colors between $i$ and $j$ are closed. Let
$\os{W}$
be one of these paths. 
Projecting $\os{W}$ to $X$ we get a path $W$ in
$X$ of length 4 that alternates colors between $i$ and $j$, and
since $X$ is a premaniplex we know that $W$ is closed. 
Suppose $W$ starts at a vertex $x$. 
Then $\os{W}$ goes from a vertex of the form
$(x,\gamma)$ to $(x,\xi(W)\gamma)$. So $\os{W}$ is closed if and only
if $\xi(W)\gamma = \gamma$, or in other words, if $W$ has trivial
voltage.
Summarizing this discussion, we arrive to the following lemma:

\begin{lema}\label{l:VoltMani}
  Let $X$ be a premaniplex and let $\xi:\Pi(X) \to \Gamma$ be a
  voltage assignment with a spanning tree $T$ of trivial voltage on all
  its darts. Then $X^\xi$ is a maniplex if and only if
  \begin{enumerate}
    % \item $X$ is a premaniplex,
  \item The set $\xi(D)$ generates $\Gamma$, where $D$ is the set of
    darts of $X$,
  \item  $\xi(d)$ has order exactly 2 when $d$ is a semi-edge,
  \item $\xi(d) \neq \xi(d')$ when $d$ and $d'$ are
    parallel darts, and
  \item if $|i-j|>1$ every (closed) path $W$ of length 4 that alternates between
    the colors $i$ and $j$ has trivial voltage.
    %% $\xi(W)=1$ when $W$ is a (closed) path of length 4 that
    %% alternates between colors $i$ and $j$ with $|i-j|>1$.
  \end{enumerate}
\end{lema}

In Section~\ref{sec:int prop} we shall translate the conditions in Lemma~\ref{l:VoltMani} to relations and inequalities that the generators of a group $\Gamma$ need to satisfy to act on a maniplex with given symmetry type graph $X$. 
%If we look at a particular premaniplex $X$, the 4 conditions in Lemma~\ref{l:VoltMani} translate to relations and inequalities that the generators of a group $\Gamma$ need to satisfy to act on a maniplex with symmetry type graph $X$. 
Before doing so, 
let us now take a closer look at the consequences of condition 4 of the above Lemma.

Condition 4 of Lemma~\ref{l:VoltMani} invites us to introduce a new concept of homotopy:
we say that two paths $W$ and $W'$  are \emph{maniplex-homotopic} if we can transform one into the other by a finite sequence of inserting or deleting pairs of inverse darts, as well as switching the colors of two consecutive darts with non-consecutive colors, that is $$d_1d_2\ldots d_i d_{i+1}\ldots d_k\mapsto d_1d_2\ldots d'_i d'_{i+1}\ldots d_k,$$ where, if $c(d)$ denotes the color of $d$, we have that $|c(d_i)-c(d_{i+1})|>1,$ $c(d'_i)=c(d_{i+1})$, $c(d'_{i+1})=c(d_i)$, $I(d'_i)=I(d_i)$ and $I(d'_{i+1})=T(d'_i)$.
Hence, a voltage assignment $\xi$ is well defined when applied to the maniplex-homotopy class of paths if and only if it satisfies Condition 4 of Lemma~\ref{l:VoltMani}. 
From this point on, whenever we speak about homotopy, homotopy class, fundamental groupoid, etc. we will be thinking in terms of maniplex-homotopy.

One could use the group $\Gamma:=\gen{S\mid R}$ as the voltage group where
$S$ has a generator $\alpha_e$ for each edge $e$ not in the spanning
tree of $X$ and $R$ has one element $\alpha_e^2$ per each semi-edge $e$ and one element $\alpha_{e_4}\alpha_{e_3}\alpha_{e_2}\alpha_{e_1}$ for each path of length four alternating between two non-consecutive colors.
In fact every voltage
group that gives a maniplex should be a quotient of this group, or in
other words $\Gamma$ is the ``most general'' group we can use as a
voltage group to get a maniplex as the derived graph. 
The ideas of the proof of Theorem 5.2 of \cite{Hartley_AllPtpsAreQuotients} show that
%We know (see~\cite[Theorem 5.2]{Hartley_AllPtpsAreQuotients}) that
$X=\T(\U,G)$ where $\U$ is the
universal polytope of rank $n$ and $G$ is some group. This means that
there is some voltage assignment $\xi$ on $X$ with voltage group $G$
such that $X^\xi$ is isomorphic to the flag graph of $\U$. Because of
the universality of $\U$ we get that $G$ and $\Gamma$ in fact are the
same. 
In other words, if we use the most general group as our voltage
group we will always get the flag graph of the universal polytope as
the derived graph.

==> VoltManB4.tex <==
\subsection{Voltage graphs that give maniplexes as derived graphs}\label{s:VoltMani}

%\ifDetallesGeneradores
%First we turn our attention to the relations between the generators. 

In \cite[Section 5]{SymType} the authors find a set of distinguished generators for a maniplex $\M$ with a given symmetry type graph $X$. 
It is easy to see that such distinguished generators can be though as voltages assigned to $X$ (or more precisely to $\Pi(X)$) so that the derived graph is $\M$.
To do this one must choose a spanning tree $T$ on $X$ and assigning trivial voltage to all its darts. All the darts that are not in $T$ will have a non-trivial voltage. 
Of course, if we want to start with a premaniplex $X$, we need to be careful with the way we assign voltages so that the derived graph is indeed a maniplex.

\if
If the STG of $\M$ is $X$, there is a method to assign voltages to the remaining darts in such a way that the derived graph is isomorphic to $\M$.
%To do this, we chose a base flag $\Phi$ in $\M$, 
It is known (\cite{SymType}\missingref{agregar resultado exacto}) that
the voltages of these darts have to generate the whole voltage group for the derived graph to be connected. So we call the non-trivial voltages of the darts
\fi

Let $X$ be a premaniplex with fundamental groupoid $\Pi(X)$, and let $\xi:\Pi(X)\to \Gamma$ be a voltage assignment, for some group $\Gamma$.
We want to find the conditions on these generators that ensure that $X^\xi$ is actually a maniplex, but before doing so, let us assume that there is a spanning tree $T$ of $X$ with trivial voltage in all its darts. 

Recall from Section~\ref{sec:voltage} that in order for $X^\xi$ to be connected, then $\xi(D)$ must generate $\Gamma$, where $D$ denoted the set of darts of $D$.





\if
It is known (see \missingref{})  that
the set $\xi(D)$, where $D$ is the set of darts of $X$, must be a
generating set of $\Gamma$ for $X^\xi$ to be connected. We can get a
more refined set of generators by choosing a subset $D' \subset D$
satisfying that no dart in $D'$ has trivial voltage and that $D'$ has
at most one dart on each edge. Once we have chosen $D'$ we call
$\xi(D')$ the {\em distinguished generators of $\Gamma$}. 
%This way of finding generators for the automorphism group of a maniplex with given symmetry type graph appears in~\cite{SymType}\missingref{agregar resultado exacto}.

Now we want to
find the conditions on these generators that ensure that $X^\xi$ is
actually a maniplex.
\fi

Next, $X^\xi$ must be a simple graph. 
This, it must not have semi-edges nor multiple edges.
%
Note that a semi-edge of $X^\xi$ would have to start at a vertex $(x,\gamma)$ and end in
$(x,\xi(e)\gamma)$, where $e$ is a semi-edge of $X$.
This implies that if the voltage of every semi-edge of $X$ is not trivial, we avoid semi-edges in $X^\xi$.
Recall further that we should have that $\xi(e)=\xi(e^{-1}) = \xi(e)^{-1}$, implying that the voltage of a semi-edge must have order two.
\if
We want $X^\xi$ to be simple. So first, we want $X^\xi$ to not have
semi-edges. We know that $X^\xi$ covers $X$ and that the image of a
semi-edge under a covering must be a semi-edge. The pre-image of a
semi-edge $e$ based on a vertex $v$ in $X$ consists of the edges of the
form $(e,\gamma)$, that start at the vertex $(x,\gamma)$ and end in
$(x,\xi(e)\gamma)$, so $(e,\gamma)$ is a semi-edge if and only if
$\xi(e) \neq 1$. We also know that the voltage of a semi-edge must
have order at
most 2 (remember that $\xi(e^{-1}) = \xi(e)^{-1}$), so we conclude that
the voltage of any semi-edge must have order exactly 2.
\fi
To avoid multiple edges, we need to avoid different darts with the same initial and terminal vertices;
%If $X^\xi$ had parallel darts, their images under the covering projection $X^\xi\to X$ would also be parallel darts, %, since parallel darts are mapped to either parallel darts or to the same dart, but since homomorphism of premaniplexes preserve color, they cannot be  mapped to the same dart.
suppose $X^\xi$ has two parallel darts
$(d,\sigma)$ and $(d',\tau)$. 
Since both darts start at the same
vertex, we have that $(I(d),\sigma)=(I(d'),\tau)$, so $I(d)=I(d')$ and $\sigma =
\tau$. The common end-point of $(d,\sigma)$ and $(d',\tau)$ could be
written as $(y,\xi(d)\sigma)$
or $(z,\xi(d')\sigma)$, where $y$ is the end-point of $d$ and $z$ the
end-point of $d'$. The fact that these two are the same means
that $y=z$ and $\xi(d) = \xi(d')$. So $(d,\sigma)$ and
$(d',\sigma)$ are parallel darts in $X^\xi$ if and only if $d$ and $d'$ are
parallel darts in $X$ with the same voltage. Thus, $X^\xi$ has no parallel
darts if and only if all pairs of parallel darts in $X$ have different
voltages.

Finally, we want to ensure that if $|i-j|>1$, the paths of length 4 in
$X^\xi$ that alternate colors between $i$ and $j$ are closed. Let
$\os{W}$
be one of these paths. 
Projecting $\os{W}$ to $X$ we get a path $W$ in
$X$ of length 4 that alternates colors between $i$ and $j$, and
since $X$ is a premaniplex we know that $W$ is closed. 
Let us base $W$
at a vertex $x$. 
Then $\os{W}$ goes from a vertex of the form
$(x,\gamma)$ to $(x,\xi(W)\gamma)$. So $\os{W}$ is closed if and only
if $\xi(W)\gamma = \gamma$, or in other words, $W$ has trivial
voltage.
Summarizing this discussion, we arrive to the following lemma:

\begin{lema}\label{l:VoltMani}
  Let $X$ be a premaniplex and let $\xi:\Pi(X) \to \Gamma$ be a
  voltage assignment with a spanning tree $T$ of trivial voltage on all
  its darts. Then $X^\xi$ is a maniplex if and only if
  \begin{enumerate}
    % \item $X$ is a premaniplex,
  \item The set $\xi(D)$ generates $\Gamma$, where $D$ is the set of
    darts of $X$,
  \item  $\xi(d)$ has order exactly 2 when $d$ is a semi-edge,
  \item $\xi(d) \neq \xi(d')$ when $d$ and $d'$ are
    parallel darts, and
  \item if $|i-j|>1$ every (closed) path $W$ that alternates between
    the colors $i$ and $j$ has trivial voltage.
    %% $\xi(W)=1$ when $W$ is a (closed) path of length 4 that
    %% alternates between colors $i$ and $j$ with $|i-j|>1$.
  \end{enumerate}
\end{lema}

If we look at a particular premaniplex $X$, the 4 conditions in Lemma~\ref{l:VoltMani} translate to relations and inequalities that the generators of a group $\Gamma$ need to satisfy to act on a maniplex with symmetry type graph $X$. Before doing so (in the next section), let us take a closer look at the consequences of condition 4 of the above Lemma.

Condition 4 of Lemma~\ref{l:VoltMani} invites us to introduce a new concept of homotopy:
we say that two paths $W$ and $W'$  are \emph{maniplex-homotopic} if we can transform one into the other by a finite sequence of inserting or deleting pairs of inverse darts, as well as switching the colors of two consecutive darts with non-consecutive colors, that is $$d_1d_2\ldots d_i d_{i+1}\ldots d_k\mapsto d_1d_2\ldots d'_i d'_{i+1}\ldots d_k,$$ where $|c(d_i)-c(d_{i+1})|>1,$ $c(d'_i)=c(d_{i+1})$, $c(d'_{i+1})=d(d_i)$, $I(d'_i)=I(d_i)$ and $I(d'_{i+1})=T(d'_i)$.
Hence, the voltage assignment $\xi$ is well defined when applied to the maniplex-homotopy class of paths. From this point on, whenever we speak about homotopy, homotopy class, fundamental groupoid, etc. we will be thinking in terms of maniplex-homotopy.

\ifEjemploManiplex
For example, if $X$ is the premaniplex $3^1$ in Figure~\ref{c:Mani3^1}, by chosing the spanning tree $T$ that includes the edge of color 0 as the tree with trivial voltage we get the following corollary:

\begin{coro}\label{c:Mani3^1}
    A group $\Gamma$ acts in a 3-maniplex (a map) with symmetry type graph $3^1$ if and only if, there are four elements $\alpha_1, \alpha_{02}, \beta_0,\beta_2$ satisfying the following conditions:
    \begin{enumerate}
        \item $\alpha_1, \alpha_{02}, \beta_0$ and $\beta_2$ generate $\Gamma$.
        \item $\alpha_1,\beta_0$ and $\beta_2$ have order 2, or in other words $\alpha_1^2=\beta_0^2=\beta_2^2=1$, $\alpha_1\neq 1$, $\beta_0\neq 1$ and $\beta_2\neq 1$.
        \item $\alpha_{02}\neq 1$ and $\beta_0\neq \beta_2$.
        \item $\alpha_{02}^2=(\beta_0\beta_2)^2=1$
    \end{enumerate}
\end{coro}

Corollary~\ref{c:Mani3^1} has been written in such a way that the items correspond to the ones with the same index in Lemma~\ref{l:VoltMani}.
In Figure~ We can see what generator corresponds to the voltage of which edge. Note that since $\alpha_{02}$ has order two, both darts of the link of color 0 have the same voltage (otherwise we would specify which is the dart with the assigned voltage by drawing it as an arrow).

\begin{figure}%[hb]
  \begin{center}
    \includegraphics[width=0.7\linewidth]{Volt02l.pdf}
    \caption{\label{f:Volt02l} The premaniplex $3^1$ with a voltage assignment.}
  \end{center}
\end{figure}


\ifCondsOrdenRaro

The fourth condition in the above lemma can be expressed as a set of
relations between the distinguished generators of $\Gamma$, one
relation for each path of length 4 satisfying the condition (we may
get some redundancy). Some of
these relations may say that two generators are the same.
%, as it was the case for $\delta_2$ and $\alpha_2$ in Section~\ref{s:3OrbGenerators}.
The second condition also gives some relations, and they are of the type
$\alpha^2=1$ where $\alpha$ is the voltage of a semi-edge, but in
addition it also gives the inequalities
$\alpha\neq 1$ when $\alpha$
is the voltage of a semi-edge. The third condition also gives inequalities, and they are of the type
$\alpha \neq \beta$, when $\alpha$ and $\beta$ are the voltages of
parallel darts.
\fi
\fi

One could use the group $\Gamma:=\gen{S|R}$ as the voltage group where
$S$ has a generator for each edge not in the spanning
tree of $X$ and $R$ has one element per each semi-edge and one element for each path of length four alternating between two non-consecutive colors. In fact every voltage
group that gives a maniplex should be a quotient of this group, or in
other words $\Gamma$ is the ``most general'' group we can use as a
voltage group to get a maniplex as the derived graph. 
We
know (see\missingref[alguna referencia externa o ponerlo antes]) that $X=\T(\U,G)$ where $\U$ is the
universal polytope of rank $n$ and $G$ is some group. This means that
there is some voltage assignment $\xi$ on $X$ with voltage group $G$
such that $X^\xi$ is isomorphic to the flag graph of $\U$. Because of
the universality of $\U$ we get that $G$ and $\Gamma$ must be the
same\isa{el universal con respecto a cualquier X es regular}. In other words, if we use the most general group as our voltage
group we will always get the flag graph of the universal polytope as
the derived graph.

==> VoltageGraphs.tex <==
%If $G$ is a group of automorphisms of a graph $X$ that acts regularly on its vertices and darts, and $Y$ is the graph... we say that \emph{$X$ covers $Y$ regularly}

The projection $p:\M\to\T(\M,G)$ is an example of what is called a \emph{regular covering projection} in graph theory (see~\cite{VoltsOrig} or~\cite{Voltajes} for more details).
Given a regular covering projection $p:\os{X}\to X$, one may recover the graph $\os{X}$ from the graph $X$ using what is known as a \emph{voltage assignment}.

We shall refer to a directed edge as a {\em dart}. The {\em inverse} of a dart $d$ is the dart $d^{-1}$ with the same edge, but different orientation. Hence, loops and links (edges between two different vertices) have two darts inverse to each other. In contrast, semi-edges have only one dart, inverse to itself.
Given an edge $e$ with vertices $v$ and $u$, if a dart $d$ of $e$ has direction from $v$ to $u$, we shall say that $v$ is the initial vertex of $d$ (and denote it by $I(d)$) and $u$ is the terminal vertex of $d$ (and denote it by $T(d)$).


A \emph{path} in a graph is a finite sequence of darts $W=d_1d_2\ldots,d_k$ such that the dart $d_{i+1}$ starts at the endpoint of the dart $d_i$. 
The \emph{start-point of $W$} is $I(d_1)$, and the \emph{endpoint of $W$} is $T(d_k)$. 
If $x$ and $y$ are the start-point  and endpoint of $W$, respectively, we say that $W$ \emph{goes from $x$ to $y$} and we write this as $W:x\to y$.
%The number $k$ is the \emph{length} of $W$ \elias{creo que sólo usamos longitud en los caminos de long. 4 que alternan colores. Tal vez se puede quitar esto}.
If the endpoint and start-point of a path $W$ are the same vertex $x$ we say that $W$ is a \emph{closed path based at $x$}.
We also consider that for every vertex $x$ there is an empty closed path %of length 0 
based at $x$.
%, and we may abuse notation and write this path as $x$ as well.

If a path $W$ ends at the start-point of a path $V$, we may define the product $WV$ as their concatenation.

Two paths $W$ and $W'$ with the same start-point and endpoint are said to be \emph{homotopic} if one can transform $W$ into $W'$ by a finite sequence of the following operations:
\begin{itemize}
    \item Inserting two consecutive inverse darts at any point, that is $$d_1d_2\ldots d_i d_{i+1}\ldots d_k\mapsto d_1\ldots d_i d d^{-1} d_{i+1}\ldots d_k,$$ where $I(d)=T(d_i)$;
    \item Deleting two consecutive inverse darts at any point, that is $$d_1\ldots d_i d d^{-1} d_{i+1}\ldots d_k \mapsto d_1d_2\ldots d_i d_{i+1}\ldots d_k;$$
\end{itemize}   
In this case we write $W\sim W'$.
 
 It is easy to see that homotopy is an equivalence relation and that if $W\sim W'$, $V\sim V'$, and $W$ ends at the start-point of $V$, then $WV\sim W'V'$.
 Therefore, we can think of the product of two homotopy classes of paths. 
 The set of all homotopy classes of paths in a graph $X$ with this operation is called \emph{the fundamental groupoid of $X$} and it is denoted by $\Pi(X)$.
 We will often speak of a "path $W$ in $\Pi(X)$", but the reader should keep in mind that we are actually referring to its homotopy class. 
 
 The subset of $\Pi(X)$ consisting of all the (homotopy classes of) closed paths based at a vertex $x$ forms a group known as \emph{the fundamental group of $X$ based at $x$} and it is denoted by $\Pi^x(X)$. 
 
 A \emph{voltage graph} is a pair $(X,\xi)$ where $X$ is a graph and $\xi$ is a groupoid antimorphism from $\Pi(X)$ to a group $G$. In this case we say that $\xi$ is a \emph{voltage assignment (on $X$)} and we call $G$ the \emph{voltage group (of $\xi$)}.
 The element $\xi(W)$ is called \emph{the voltage of $W$}.
 
 Note that a voltage assignment is completely determined by the voltages of the darts of the graph, as the voltage $\xi(W)$ of a path $W=d_1d_2\ldots d_{k-1}d_k$ is simply $\xi(d_k)\xi(d_{k-1})\ldots \xi(d_1)$.
 In fact, if $D$ is the set of darts of a graph $X$, any function $\xi:D\to G$ can be extended to a voltage assignment as long as $\xi(d^{-1})=\xi(d)^{-1}$ for every dart $d\in D$.
 
 Given a voltage graph $(X,\xi)$ with voltage group $G$, we can construct the \emph{derived graph} $X^\xi$ as follows:
 \begin{itemize}
     \item The vertex set is $V\times G$ where $V$ is the vertex set of $X$.
     \item The dart set is is $D\times G$ where $D$ is the dart set of $X$.
     \item If the dart $d$ goes from $x$ to $y$, the dart $(d,g)$ goes from the vertex $(x,g)$ to $(y,\xi(d)g)$.
 \end{itemize}
 This is an undirected graph, as the inverse of the dart $(d,g)$ is the dart $(d^{-1},\xi(d)g)$.
 Note that for every $h\in G$, the mapping $(x,g) \mapsto (x,gh)$ is an automorphism of $X^\xi$. That is, $G$ can be regarded as a group of automorphisms of $X^\xi$.
 
 Given a path $W$ of a graph $X$ starting at a vertex $x$ and given an element $g$ in the voltage group, there is a unique path $\os{W}$ in $X^\xi$ that starts at $(x,g)$ that projects to $W$.
 The path $\os{W}$ is called a \emph{lift of $W$} and it is easy to see that it ends at $(y,\xi(W)g)$ where $y$ is the endpoint of $W$ (for details see~\cite{Voltajes}).
 
 In our case, we will work with graphs that have a coloring of its edges (and therefore, darts), so we will define that the color of the dart $(d,g)$ is the same as the color of $d$.
 
 It is known (see~\cite{VoltsOrig} or ~\cite{Voltajes}) that if $p:\os{X}\to X$ is a regular covering, there is a voltage assignment $\xi$ such that $\os{X}$ is isomorphic to $X^\xi$.
 Moreover, given a spanning tree $T$ of $X$, there is a voltage assignment $\xi$ such that $\os{X}\cong X^\xi$ and $\xi(d)=1$ for every dart $d$ in $T$.
